On Average-Case Error Bounds for Kernel-Based Bayesian Quadrature

In this paper, we study error bounds for {\em Bayesian quadrature} (BQ), with an emphasis on noisy settings, randomized algorithms, and average-case performance measures. We seek to approximate the integral of functions in a {\em Reproducing Kernel Hilbert Space} (RKHS), particularly focusing on the Mat\'ern-$\nu$ and squared exponential (SE) kernels, with samples from the function potentially being corrupted by Gaussian noise. We provide a two-step meta-algorithm that serves as a general tool for relating the average-case quadrature error with the $L^2$-function approximation error. When specialized to the Mat\'ern kernel, we recover an existing near-optimal error rate while avoiding the existing method of repeatedly sampling points. When specialized to other settings, we obtain new average-case results for settings including the SE kernel with noise and the Mat\'ern kernel with misspecification. Finally, we present algorithm-independent lower bounds that have greater generality and/or give distinct proofs compared to existing ones.

==> On Average-Case Error Bounds for Kernel-Based Bayesian Quadrature/abstract.tex <==
\begin{abstract}

In this paper, we study error bounds for {\em Bayesian quadrature} (BQ), with an emphasis on noisy settings, randomized algorithms, and average-case performance measures.  We seek to approximate the integral of functions in a {\em Reproducing Kernel Hilbert Space} (RKHS), particularly focusing on the Mat\'ern-$\nu$ and squared exponential (SE) kernels, with samples from the function potentially being corrupted by Gaussian noise.  We provide a two-step meta-algorithm that serves as a general tool for relating the average-case quadrature error with the $L^2$-function approximation error. 
When specialized to the Mat\'ern kernel, we recover an existing near-optimal error rate while avoiding the existing method of repeatedly sampling points.  When specialized to other settings, we obtain new average-case results for settings including the SE kernel with noise and the Mat\'ern kernel with misspecification.  Finally, we present algorithm-independent lower bounds that have greater generality and/or give distinct proofs compared to existing ones.

% In particular, by greedily optimizing the posterior variance, the meta algorithm recovers the optimal bound of noisy Mat\'ern functions, while being more practical than an earlier result which relied on repetitive sampling.  Our algorithm has the advantage of being non-adaptive compared to existing adaptive GP-based algorithms, but also establishing that there is no adaptivity gap against the known lower bound, where such results are re-proven by us in a kernel-focused manner together with a new unified proof technique in the noisy setting, and most importantly, are generalized from integer-order function smoothness to fractional-order.  Finally, we present a connection between BQ and {\em Bayesian optimization} (BO), by analyzing the convergence of the posterior variance of the first step of our algorithm using BO techniques, resulting new upper bounds for SE kernel.


\end{abstract}

==> On Average-Case Error Bounds for Kernel-Based Bayesian Quadrature/main.tex <==
\section{Introduction} \label{sec:intro}

The integration of black-box functions is a fundamental problem with numerous applications, with Bayesian inference being a prominent example. The method of {\em Bayesian Quadrature} (BQ) \citep{Oha91, Ras03} has particularly gained popularity, adopting Bayesian modeling techniques to model the unknown function and reduce the required number of function evaluations.  Mathematically, the goal is to approximate the quantity
\begin{equation}
    I(f) = \int f(\xv)p(\xv)d\xv, \label{eq:integral0}
\end{equation}
where $p(\xv)$ is a known weighting function, but we only have black-box access to $f(\xv)$. 
%
It is common to study this problem for worst-case functions in a given class, and with noiseless function queries and deterministic algorithms (e.g., see \citep{Nov88,Kan16,Kan19}).  However, this is also substantial motivation to understand average-case performance measures, noisy queries, and randomized algorithms (e.g., see \citep{Nov88,Pla96,Nov16}).  

As an example motivating noisy settings, when performing integrals in Bayesian inference, function evaluations themselves may be implemented using a randomized subroutine whose variations can be modeled by introducing noise terms.  As a rather different example, in the same way that noisy Bayesian optimization (BO) can be used to find maximal sensor readings in a sensor network (e.g., see \citep{Kra11}), noisy BQ methods could be used to find average (or weighted average) readings.   

\subsection{Overview of Contributions}

In this paper, our focus is on kernel-based BQ methods, corresponding to functions lying in a {\em Reproducing Kernel Hilbert Space} (RKHS). 
 We focus on the widely-used Mat\'ern and Squared Exponential (SE) kernels, given by \citep{Ras06}
\begin{align}
    \knu(\xv,\xv') &= \frac{2^{1-\nu}}{\Gamma(\nu)}
    \bigg(\frac{\sqrt{2\nu}\,\|\xv - \xv'\|}{l}\bigg)^{\nu}  J_{\nu}\bigg(\frac{\sqrt{2 \nu}\,\|\xv - \xv'\|}{l} \bigg), \label{eq:kMat} \\
    \kse(\xv,\xv') &= \exp\bigg(-\frac{\|\xv-\xv'\|^2}{2l^2}\bigg), \label{eq:kSE} 
\end{align}
where $J_{\nu}$ is the modified Bessel function, $\Gamma$ is the gamma function, $l
$ is the length-scale, $\nu$ is the Mat\'ern smoothness parameter, and $\|\cdot\|$ denotes the Euclidean norm.  Our main contributions are outlined as follows.

% In such a setting, we have established a conceptually stretchable algorithm that estimates the average-case BQ error from a function approximation point of view.  There are several kernel-based function approximation estimators, such as the kernel interpolation estimator (also known as kernel ridge regression) and the Gaussian process (GP) estimator, where we are particularly interested in the later since it fits the Bayesian paradigm of being able to model the posterior uncertainty.  In-depth relationships of these two estimators can be found, for example, in a recent survey \citep{Kan18}.  

{\bf Meta-Algorithm.} Our main algorithm is a ``meta-algorithm'' that builds on an idea originally used for Sobolev (and other) functions in noiseless settings (e.g., \citep[Sec.~2]{Nov88}).  The meta-algorithm runs any algorithm for estimating the function in $L^2$-norm using the first half of the samples, runs a Monte Carlo method using the remaining samples to estimate the residual, and then combines the two.  We give a general theorem relating the $L^2$-error of the first step with the overall integration error, and show that this has broad implications beyond the settings for which the idea was used previously, as outlined below.

{\bf Resulting Upper Bounds.} Some specific applications of our general theorem are as follows:
\begin{itemize}
    % \setlength\itemsep{1em}
    \item By using a maximxum-variance algorithm from \citep{Vak21} in the first part, we establish that for the Mat\'ern-$\nu$ kernel, one attains an order-optimal error bound of $\Theta(T^{-\frac{\nu}{d}-1} + \sigma T^{-\frac{1}{2}})$ (with time horizon $T$, noise variance $\sigma^2$, Mat\'ern smoothness $\nu$, and dimension $d$).  This scaling was previously derived in \citep{Pla96}, but used a method based on repeatedly re-sampling a carefully-chosen set of points many times to reduce noise, which may be undesirable in practice.
    % When applied to $d$-dimensional Mat\'ern-$\nu$ RKHS functions, our algorithm establishes that, by greedily selecting points according to minimizing the GP posterior variance, one can achieve the averaged optimal order with no adaptive gap.  While both order-optimal lower and upper bounds in the noisy setting, in the order of $\Theta(T^{-\frac{\nu}{d}-1} + \sigma T^{-\frac{1}{2}})$, has once obtained by \citep{Pla96}, their analysis of the upper bound was built on repeatedly sampling from a fixed set of points in a deterministic manner, whereas the randomization is only reflected through observation noise.  As shown in their analysis, the deterministic approach relies heavily on carefully designed sub-domain/point sets,  which is significantly less practical than purely non-adaptive randomized algorithms. 
    \item We additionally provide corollaries of our main theorem providing results that appear to be new (though related results with other settings or criteria do exist), including for the Mat\'ern kernel with misspecified smoothness, and average-case performance for the SE kernel in both the noiseless and noisy settings.
    % Other evidence of the practicality of our algorithm is that it can be easily extended to the recent prevalent mis-specified setting with the presence of kernel hyperparameter selection \citep{Kan16,Tec20,Wyn21}, or even to the average-case SE kernel quadrature, where such results are considerably less explored.
    % \item In a certain manner, the second step can be detached from the first step, reducing to a pure exploration policy, usually referred to as maximum variance reduction in BO-related works (see e.g. \citep{Vak21}).  This allows us to analyze the BQ error using BO techniques, which is rarely seen in BQ literature.  This yields several new average-case upper bounds for both kernels in Section \ref{sec:upper}, where the noiseless SE upper bound converges rapidly.  
\end{itemize}

{\bf Algorithm-Independent Lower Bounds.} While our main contributions are those outlined above, we also provide some results regarding algorithm-independent lower bounds.  For the Mat\'ern kernel with noise, we provide an alternative proof of the $\Omega(T^{-\frac{\nu}{d}-1} + \sigma T^{-\frac{1}{2}})$ lower bound from \citep{Pla96} that establishes a single source of difficulty for both terms in the bound (which were previously handled separately), and we slightly generalize to Mat\'ern parameters such that $\nu+\frac{d}{2}$ may be non-integer.  Moreover, we establish that the $\Omega( \sigma T^{-\frac{1}{2}} )$ lower bound holds much more generally in noisy settings, including for the SE kernel.

% We have also extended the noisy lower bound in \citep{Pla96} from integer-valued $\nu+\frac{d}{2}$ to fractional order, in parallel with the noiseless lower bounds that have been comprehensively studied by \citep{Nov88,Nov16}.  We provide two distinct proofs for the noisy lower bound.
% \begin{itemize}
%     \item The first combines a noiseless average-case $\Omega(T^{-\frac{\nu}{d}-1})$ lower bound \citep{Nov88} with a simple $\Omega(\sigma T^{-\frac{1}{2}})$ lower bound that arises from considering constant-valued functions.  This proof, although being trivial, benefits from reproducing properties of RKHS functions, readily extends to obtain a noisy SE lower bound, where only near-constant functions are available.  
%     \item  The second proof considers a single subset of functions consisting of ``bumps'' whose signs are difficult to determine, and simultaneously attains both terms in a unified manner.   This approach is more technically challenging, but is useful for identifying a single source of difficulty, and may be more suitable when generalizing to other RKHS function classes.
% \end{itemize}

Our results are summarized in Table \ref{tab:compare}, along with various existing results that we discuss in the following subsection.

\subsection{Related Work}\label{sec:relate}
\begin{table*}[t!]
\renewcommand{\arraystretch}{1.3}
    \begin{centering}
    \resizebox{0.75\linewidth}{!}{
        \begin{tabular}{|>{\centering}m{3cm}|>{\centering}m{3.5cm}|>{\centering}m{3.5cm}|>{\centering}m{4.5cm}|}
            \hline 
            \textbf{Summarized Results} & {\small \bf Noiseless Worst} & {\small \bf Noiseless Average } & {\small \bf Noisy Average }
            \tabularnewline
            \hline
            
            {\small \bf Mat\'ern Lower} &  $\underline{\Omega\big(T^{-\frac{\nu}{d}-\frac{1}{2}}\big)}$  \\ \citep{Nov88} &  $\underline{\Omega\big(T^{-\frac{\nu}{d}-1}\big)}$ \\ \citep{Nov88} &  $\underline{\Omega\big(T^{-\frac{\nu}{d}-1}+\sigma T^{-\frac{1}{2}}\big)}$ \\ \citep{Pla96} \tabularnewline
            \hline
            
            
            {\small \bf Mat\'ern Upper}  & $O\big(T^{-\frac{\nu}{d}-\frac{1}{2}}\big)$ \\ \citep{Nov88}& $\underline{O\big(T^{-\frac{\nu}{d}-1}\big)}$ \\ \citep{Nov88} &  $\underline{O\big(T^{-\frac{\nu}{d}-1}+\sigma T^{-\frac{1}{2}}\big)}$ \\ \citep{Pla96}
            \tabularnewline
            \hline 
            
            {\small \bf SE Lower}  & $\Omega(T^{-C T^{\frac{1}{d}}})$ \\ \citep{Kuo17} (Linear algs.~only) & N/A &  $\doubleunderline{\Omega\big(\sigma T^{-\frac{1}{2}}\big)}$  \tabularnewline
            \hline 
            
            {\small \bf SE Upper} & $O\big(e^{-C T^{\frac{1}{d}}}\big)$ \\ \citep{Kan19} & $\doubleunderline{O\big(e^{-\frac{d}{2} T^{\frac{1}{d}}}\big) T^{-\frac{1}{2}}}$ & $\doubleunderline{O\big(e^{-C (\frac{T}{\log T})^{\frac{1}{d}}}T^{-\frac{1}{2}} + \sigma T^{-\frac{1}{2}}\big)}$
            \tabularnewline
            \hline 
        \end{tabular}
    }
    \par\end{centering}
        
    \caption{Summary of some of the most related existing results and our results.  Results with an underline were partially or fully existing but are extended or re-derived in our work (e.g., results extended to fractional $\nu+\frac{d}{2}$, upper bounds based on distinct algorithms, or lower bounds via alternative proof techniques).  Results with double underlines are new to this paper, to our knowledge. \label{tab:compare}}
\end{table*}

{\bf Numerical Integration and Bayesian Quadrature.} Extensive early work on numerical integration appeared in the literature on information-based complexity, e.g., see \citep{Bak59,Nov88,tra03,Nov08} and the references therein. Function classes considered included Sobolev, H\"older, and others, with the Sobolev class being particularly related to the Mat\'ern RKHS (see Appendix \ref{sec:sobolev}). 
%
More explicit use of kernel-based methods appeared in \citep{Nar02,Wen04,Wen05,Rie10}, and 
%In particular, \citep{Wen04} proved that Mat\'ern RKHS functions are norm-equivalent to Sobolev functions, which brought convince for using earlier obtained mathematical results.  Among these kernel-based methods, 
Bayesian quadrature from a probabilistic perspective \citep{Ras06,Kan16,Kan18,Wyn21} has gained particular popularity due to its role in statistical machine learning.  
% As a consequence, this motivated us to re-prove lower bounds in \citep{Nov88,Pla96}, by treating Sobolev functions as Mat\'ern RKHS functions from a kernel-centric point of view.  

% From Table \ref{tab:compare}.  We see that, the noiseless worst-case setting is generally well-studied for both kernels, whereas more challenges are left for the average-case setting, especially for SE functions.

{\bf Upper Bounds Under the Mat\'ern Kernel.}  For $d$-dimensional Mat\'ern-$\nu$ RKHS functions with query budget $T$, early literature such as \citep{Bak59, Nov88} proved that in the noiseless setting, the best possible worst-case (deterministic) error is $\Theta(T^{-\frac{\nu}{d}-\frac{1}{2}})$, whereas by considering the average-case error of a randomized algorithm, this can be reduced to $\Theta(T^{-\frac{\nu}{d}-1})$.  An extensive survey of the noiseless setting can be found in \citep{Nov88}, where it is also noted that basic Monte Carlo sampling attains $O(T^{-\frac{1}{2}})$ error; this observation also extends immediately to the noisy setting with $\sigma = O(1)$ \citep{Pla96}.  

As we hinted above, the $L^2$-error bounds for the Mat\'ern kernel with noise in \citep{Wyn21} will be particularly useful for our purposes, including in misspecified settings.  Some implications of these results for noisy BQ were also noted in \citep{Wyn21}, but they resulted in worse scaling (namely, $\Theta(T^{-\frac{s}{2s+d}})$ with $s = \nu+\frac{d}{2}$) than that shown in Table \ref{tab:compare}.  In fairness, however, several of the results in \citep{Wyn21} can also be applied to settings with non-stochastic noise, whereas we only handle i.i.d.~random noise.

% As discussed earlier, all these results are recovered and further extended by us from kernel-based analysis and GP-based randomized algorithms, where the analysis of the noisy upper bounds are particularly related to the work of \citep{Wyn21}, since they considered estimating the function in $L^2$-norm.

% We note that our noisy Mat\'ern upper bound also shares the same notable feature of considering mis-specification as in \citep{Wyn21} (as well as the earlier work of \citep{Kan16}), where the $\nu$ value is assumed to be different to the true one.  This is a quite useful setting for some scenarios where it is difficult to identify the smoothness of the target function, and one has to perform maximum marginal likelihood estimation (see \citep{Ras06}), or similar, to choose suitable kernel hyperparameters.

{\bf Upper Bounds Under the SE Kernel.}  For functions in the SE RKHS, we observe in Table \ref{tab:compare} that there are non-minor gaps between lower and upper bounds.
%mainly due to the difficulty of not being able to use the bounded-support bump functions (as it has infinite RKHS norm) in proving the lower bound.  This hardness increases in the average-case setting, as such lower bound is currently missing from the field.  
For a different setting in $\RR^d$ with $p(\xv)$ in \eqref{eq:integral0} being a Gaussian distribution, \citep{Kuo17} gives a worst-case lower bound for \emph{linear algorithms}, by decomposing SE functions using an orthogonal basis in the $L^2$ space.  This lower bound has been further improved in \citep{Kar21} using another orthogonal basis in the native RKHS space, but it only applies to (linear) Gauss-Hermite rules.  Overall, research on the SE kernel appears to have mainly focused on noiseless worst-case upper bounds. 

A notable work related to ours is the adaptive BQ (ABQ) algorithm from \citep{Kan19}.  While their algorithm is adaptive, we see in Table \ref{tab:compare} that our non-adaptive algorithm yields a slight improvement over theirs, albeit with a weaker average-case guarantee.  Similar observations also apply to Mat\'ern functions, where the ABQ algorithm only achieves $O(T^{-\frac{\nu}{d}})$ scaling \citep[Cor.~C.4]{Kan19}.

% {\color{red} The above same algorithm is not applicable to noisy SE functions, where the difficulty is caused by the key ingredient, the $L^2$ function approximation error, is not robust to noisy observations.  This has first been observed by \citep{Mar10} through a quantity called Lebesgue constant, where for infinite smooth kernels (such as SE), this quantity tends to grow with the number of samples, in the meanwhile, will shrink for finite smoothness kernels (such as Mat\'ern).  Further discussions will be made in Section \ref{sec:upper} with a subsequent work \citep{Son13} with theoretical justifications.  Nevertheless, we might only perform the first batch of our algorithm to obtain a sub-optimal bound, but there exist techniques other than GP regression to give optimal bounds for noisy SE quadrature.} 

{\bf Equivalence between Random Features and Bayesian Quadrature.}  An interesting equivalence between worst-case kernel-based quadrature and random feature based function approximation in $L^2$ norm has once established in \citep{Bac17}.  While the main focus in \citep{Bac17} is the worst-case noiseless setting, it is noticed in Sec.~3.1 therein that their methods are have a certain tolerance to noise.  Noisy error bounds can be obtained via this fact, but they are higher than ours, with the first of the two terms (e.g., see \eqref{eq:matern_final} below) typically being a factor $\frac{1}{\sqrt T}$ smaller in our work, and being order-optimal in several cases of interest.  We crucially rely on randomization to achieve this, whereas the proposed algorithm in \citep{Bac17} is deterministic.  We note that for the SE kernel, one of our results (Corollary \ref{cor:avg_se_sig}) uses a result from \citep{Bac17} as an intermediate step.

% {\color{red} It has to be pointed out that, such an equivalence does not hold in our setting nor affect our previously obtain results, since (i) we are more interested in GP-based algorithms, (ii) the random noise naturally lends itself to an average-case criterion, and (iii) we are also interested in general choices of $p(\xv)$, and our hardness results will consider $p(\xv)=1$ (the equivalence in \citep{Bac17} does not apply under this choice).   Therefore, in a rather different setting, the GP-based selection rule in our two-batch algorithm can be replaced by a random feature selection algorithm to obtain the desired noisy upper bound.}

{\bf Relationship with Bayesian Optimization.}  The extensive literature on {\em Bayesian Optimization} (BO) is also related to our work in the sense of iterating acquisition functions.  However, BO turns out to be a strictly harder problem.  As surveyed in detail in the noiseless setting in \citep{Nov88}, noiseless BO is closely related to estimating the function in $L^{\infty}$ norm, and noiseless BQ is closely related to estimating it in $L^2$ norm, with the former being strictly harder.  Viewed differently, a key difficulty in BO is identifying a single short and narrow ``bump'' \citep{Bul11,Sca17a}, whereas in BQ the same bump contributes a negligible amount to the integral.  We elaborate on this connection in Appendix \ref{app:alt_bo}, showing that BO-type techniques yield suboptimal BQ bounds for the Mat\'ern kernel.  On the other hand, in Section \ref{sec:upper}, we will see that this approach gives a fairly good result for the SE kernel in the noiseless (but not noisy) setting.

% To further connect the two problems, in Appendix \ref{app:alt_bo}, we analyze the error of maximum variance sampling algorithm using techniques from BO literature, which are extensively studied and convenient to use.   We obtain orders of $O\big(T^{-\frac{\nu}{d}}\big)$ and $O\big(T^{-\frac{\nu}{2\nu+d}}\big)$ (see Theorem \ref{thm:alt_upper}) for noiseless and noisy Mat\'ern functions respectively, which are significantly weaker than our main upper bound results.  Thus, while BO techniques can indeed be adapted to BQ, doing so would sometimes gives highly sub-optimal bounds.  We again observe that, the non-adaptive average-case upper $O\big(T^{-\frac{\nu}{d}}\big)$ actually matches ABQ in the worst case setting.   The SE kernel results are also readily to obtain, in Theorem \ref{thm:alt_upper}, we obtain orders of $O\big(e^{-\frac{d}{2} T^{\frac{1}{d}}} \big)$ and $O\big((\log T)^{\frac{d+1}{2}} T^{-\frac{1}{2}}\big)$ for noiseless and noisy SE functions respectively.  While the noisy result is considerably sub-optimal, the noiseless bound achieves the promising exponential convergence, which is comparable to the convergence of ABQ in the worst-case setting, however, is non-adaptive.

{\bf Other Variants of BQ.} Finally, various works on BQ have explored more sophisticated techniques and variations such as adaptive sampling \citep{Kan19}, active area search \citep{Ma14}, and settings with multiple related functions \citep{Ges19} (among many others).  We are not aware of any (beyond those outlined above) that are directly related to our study of theoretical error bounds in relatively standard settings.

\section{Problem Setup} \label{sec:setup}

Let $f:D\rightarrow\RR$ be a real-valued function on the compact domain $D=[0,1]^d$.  By shifting and scaling, our results readily extend to arbitrary rectangular domains.  In addition, our upper bounds easily extend to general compact domains.  

We consider the class $\Hk(B)$ of functions whose RKHS norm $\|\cdot\|_{\Hk}$ is upper bounded by some constant $B>0$.  We focus in particular on the Mat\'ern-$\nu$ kernel (see \eqref{eq:kMat}), whose function class $\mat(B)$ is norm-equivalent to the Sobolev class (see Appendix \ref{sec:sobolev} for details).  We also derive results for the SE kernel (see \eqref{eq:kSE}), where the function class is denoted as $\se(B)$.

Let $p(\xv)$ be a known and bounded density function, i.e., $p(\xv) \in [0,p_{\max}]$ for some $p_{\max} > 0$, and $\int p(\xv)d\xv=1$.  We define $\Pc(p_{\max})$ to be the set of all functions satisfying these conditions. Our goal is to estimate the integral of an RKHS function $f:D\rightarrow \RR$ weighted by $p(\xv)$, defined in \eqref{eq:integral0}.  Before forming an approximation of this integral, the algorithm takes $T$ observations: At time step $t$, select $\xv_t\in D$, and observe $y_t=f(\xv_t)+\epsilon_t$, where $\epsilon_t \sim \Nc(0,\sigma^2)$ is Gaussian noise.  The final approximate integral is denoted by $\Ihat$.

As is commonly done for RKHS functions, we will use Bayesian methods based on a GP prior ${\rm GP}(0,k)$ and a Gaussian noise model.  After observing $t$ noisy samples, the posterior distribution is also a GP with the following posterior mean and variance:
\begin{align}
    \mu_{t}(\xv) &= \kv_t(\xv)^T\big(\Kv_t + \lambda \mathbf{I}_t \big)^{-1} y_t,  \label{eq:posterior_mean} \\ 
    \sigma_{t}^2(\xv) &= k(\xv,\xv) - \kv_t(\xv)^T \big(\Kv_t + \lambda \mathbf{I}_t \big)^{-1} \kv_t(\xv), \label{eq:posterior_variance}
\end{align}
where $y_t = [y_1,\ldots,y_t]^T$, $\kv_t(\xv) = \big[k(\xv_i,\xv)\big]_{i=1}^t$, $\Kv_t = \big[k(\xv_t,\xv_{t'})\big]_{t,t'}$ is the kernel matrix, $\mathbf{I}_t$ is the identity matrix of dimension $t$, and $\lambda>0$ is a hyperparameter.

We consider both adaptive algorithms (i.e., the algorithm observes $y_1,\dotsc,y_{t-1}$ before choosing $\xv_t$) and non-adaptive algorithms (i.e., all $\xv_1,\dotsc,\xv_T$ are chosen in advance).  In fact, we will prove our lower bound for adaptive algorithms and upper bounds for non-adaptive algorithms, thus establishing the stronger type of result in both cases.

Using the shorthands $\Hk = \Hk(B)$ (as well as $\mat$ or $\se$ when the kernel $k$ is specialized as Mat\'ern or SE) and $\Pc = \Pc(p_{\max})$, the settings in Table \ref{tab:compare} are summarized as follows, the last of which is the one we primarily focus on:
\begin{itemize}
    \item {\bf Noiseless Worst-Case Error:} $\rwst = \sup_{p \in \Pc, f\in \Hk} |I -\Ihat|$.
    \item {\bf Noiseless Average-Case Error:} $\ravg = \sup_{p \in \Pc, f\in \Hk} \EE\big[ |I - \Ihat| \big]$, where the expectation is over the randomized algorithm.
    \item {\bf Noisy Average-Case Error:} $\ravgsig = \sup_{p \in \Pc, f\in \Hk} \EE\big[ |I - \Ihat| \big]$, where the expectation is over the randomized algorithm and the noise.
\end{itemize}
We have omitted a notion of worst-case error for the noisy setting, since there are subtle issues in posing such a setting in a meaningful manner (e.g., see \citep{Pla96}).  For instance, even if the algorithm is deterministic given the noisy observations, it can still obtain randomness by taking digits after the 1000th decimal point (say) of the observed values $y_t$.  That is, the randomness from the noise alone could still give the same effect as using a randomized algorithm.


\section{Lower Bounds}
Our lower bounds for the noisy setting are stated as follows; note that we allow $\sigma$ to vary with $T$.

\begin{thm}\label{thm:noisy_lower}
    {\em (Average-Case Noisy Lower Bounds)}
    Consider our problem setup with constant parameters $(B,\nu,d,l)$, noise variance $\sigma^2$, and query budget $T$.  Then, for any algorithm (possibly adaptive and/or randomized) for estimating $I$, we have the following lower bounds on the average-case error:
    \begin{enumerate}
        \item For Mat\'ern kernel with $\nu+\frac{d}{2}\ge 1$, we have
        \begin{equation}\label{eq:mat_lb_sig}
            \ravgsigmat = \Omega\big(T^{-\frac{\nu}{d}-1} + \sigma T^{-\frac{1}{2}}\big).
        \end{equation}
        \item For any kernel such that $\max_{\xv} k(\xv,\xv) < \infty$ and $\int_{[0,1]^d} k(\xv,\xv^\natural) d\xv \ne 0$ for some $\xv^\natural$ (e.g., the SE or Mat\'ern kernel with $\xv^\natural = \bzero$), we have:
        \begin{equation}\label{eq:se_lb_sig}
            \ravgsig = \Omega\big(\sigma T^{-\frac{1}{2}} \big).
        \end{equation}
        % where ${\rm LB}(\ravgse)$ represents the average-case lower bound for SE kernel quadrature.
    \end{enumerate}
    Moreover, these lower bounds hold even under the fixed weight function $p(\xv) = 1$.
\end{thm}

\subsection{Proof of Theorem \ref{thm:noisy_lower}}

The first term in \eqref{eq:mat_lb_sig} follows directly from noiseless average-case error bounds (see Appendix \ref{app:existing}).  The second term can also be established by considering constant-valued functions \citep{Pla96}, or as a special case of \eqref{eq:se_lb_sig} (which is proved below).  On the other hand, it is also of interest to establish a single hard subset of functions that yields both terms in \eqref{eq:mat_lb_sig} in a unified manner, thus establishing a single source of difficulty for both terms.  We provide such an approach in  Appendix \ref{app:lowerboundproof}, considering functions composed of several small ``bumps''.  The idea is that with too few samples the algorithm cannot reliably determine which bumps are positive and which are negative, and if too many of these are uncertain, then a certain level of error is unavoidable.

It remains to prove \eqref{eq:se_lb_sig}.  To do so, we consider the function $f(\xv) = k(\xv,\xv^\natural)$, which is bounded and has a non-zero integral by assumption.  Moreover, since $k(\cdot,\xv^\natural)$ is trivially in the RKHS class, we have that the scaled function $f_c(\xv) = c f(\xv)$ has RKHS norm at most $B$ for all $c > 0$ below a suitably-chosen threshold.

We consider the sub-class of functions $f_c$ with RKHS norm at most $B$, and show that $\Omega(\sigma T^{-\frac{1}{2}})$ queries are needed even for this sub-class.  To see this, we note that sampling any point $\xv$ corresponds to observing $c$, scaled by $f(\xv)$, with $N(0,\sigma^2)$ noise.  Without loss of optimality, we can assume that the algorithm only samples at the point(s) where $|f(\xv)|$ is largest (so that $c$ is maximally scaled while the noise level is fixed), and by assumption we have $|f(\xv)| < \infty$.  Then, the noisy integration problem on this sub-class reduces to the noisy estimation of $c$ with Gaussian noise, which is well known to incur $\Theta(\sigma T^{-\frac{1}{2}})$ error (even when $c$ is known to be below an arbitrarily small constant threshold), e.g., see \citep{Pla96}.

\section{Upper Bounds}\label{sec:upper}
% \subsection{Worst-case SE Upper Bounds}

% \subsection{Upper Bounds}
\begin{algorithm}[t]
	\caption{Two-batch integral estimation meta-algorithm}  \label{alg:two-phase-bq}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:}  Function $f$, domain $D$, time horizon $T$, function estimation algorithm \textsc{EstimateFunc}
		\STATE Use \textsc{EstimateFunc} with $\frac{T}{2}$ samples to produce a function estimate $\fhat$ 
		\FOR{$t=\frac{T}{2}+1,\dots,T$}
			\STATE Sample $\xv_t \sim p(\xv)$ independently
			\STATE Observe $y_t=f(\xv_t)+\epsilon_t$
		\ENDFOR
		\STATE Compute the approximate integral $\Ihat_1=\int_D p(\xv) \fhat(\xv)d\xv$
		\STATE Compute the residual $\Rhat=\frac{2}{T}\sum_{t=T/2 + 1}^{T} (y_t-\fhat(\xv_t))$
		\STATE Output $\Ihat = \Ihat_1+\Rhat$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
	\caption{Maximum variance sampling; can be used as \textsc{EstimateFunc} in Algorithm \ref{alg:two-phase-bq}}  \label{alg:max-var}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} Function $f$, domain $D$, GP prior ($\mu_0$, $k_0$), GP noise variance $\lambda$, time horizon $\frac{T}{2}$
		\FOR{$t=1,\dots,\frac{T}{2}$}
			\STATE Select $\xv_t=\argmax_{\xv\in D}\sigma_{t-1}(\xv)$
			\STATE Receive $y_t=f(\xv_t)+\epsilon_t$
			\STATE Update $\sigma_t$ using $\xv_1,\dotsc,\xv_t$
		\ENDFOR
		\STATE Update $\mu_{T/2}(\xv)$ using $\xv_1,\dots,\xv_{T/2},y_1,\dots,y_{T/2}$
		\STATE Output $\mu_{T/2}$
	\end{algorithmic}
\end{algorithm}
In this section, we introduce our main meta-algorithm and derive upper bounds on the average-case error.  We follow the high-level idea of combining function estimation methods with Monte Carlo estimation on the residual, previously proposed for the noiseless setting \citep{Nov88}, but with different details to account for the noise.
The meta-algorithm is shown in Algorithm \ref{alg:two-phase-bq}, and is described as follows.  The samples are performed in two batches, but still in a non-adaptive manner (i.e., the second batch can be chosen without knowing the first batch).\footnote{Our main theorem remains true when the first batch consists of adaptive sampling, but all of our corollaries will be based on non-adaptive sampling.}  The first batch uses $T/2$ samples to construct an approximation $\fhat$ of $f$, which forms an initial estimate $\Ihat_1=\int_D p(\xv) \fhat(\xv) d\xv$.  The subroutine \textsc{EstimateFunc} for doing so is kept general for now, but by default, we will use maximum variance sampling\footnote{We focus on maximum variance sampling for concreteness, but our analysis and results are unchanged when, at time $t$, an arbitrary point satisfying $\sigma_{t-1}(\xv)\geq \gamma\|\sigma_{t-1}\|_{L^\infty}$ is found for some $\gamma \in (0,1)$ (e.g., $\gamma = \frac{1}{2}$).  This requirement is potentially much easier to attain in practice, instead of insisting on the global maximum.} as shown in Algorithm \ref{alg:max-var}, with the estimated $\fhat$ being given by the GP posterior mean $\mu_{T/2}$.  Note that these $T/2$ samples are non-adaptive because the posterior variance of a GP does not depend on any observations.  The remaining $T/2$ samples estimates the residual $R$ between the difference of the true integral $I$ and this value $\Ihat_1$:
\begin{equation*}
    R=I-\Ihat_1=\int_D p(\xv) (f(\xv)-\fhat(\xv))d\xv.
\end{equation*}
Having fixed $\fhat$ and hence $\Ihat_1$, we can refine our overall estimate of $I$ by estimating the residual $R$. To do so, we use the last $T/2$ samples to construct a Monte Carlo estimator $\Rhat$ of $R$, i.e., 
\begin{equation*}
\Rhat=\frac{2}{T}\sum_{t=T/2+1}^{T} (y_t-\fhat(\xv_t)),
\end{equation*}
in which each $\xv_t$ is sampled from $p(\xv)$.  Hence, the approximated integral is simply $\Ihat = \Ihat_1 + \Rhat$. 

In the following theorem, we establish the upper bound of the average-case integration error of Algorithm \ref{alg:two-phase-bq} in terms of the noisy $L^2$ distance between $f$ and $\fhat$, with an extra noise term.  This theorem is general and can be applied to a variety of kernel choices, noise settings, misspecified settings, etc., as we will see below.  In the following, all omitted proofs are deferred to Appendix \ref{app:proof-avg-upper}.

\begin{thm} \label{thm:avg_int_l2}
    {\em (Quadrature-$L^2$ Relationship)} 
     For any fixed $f\in\Hk$ and $p\in \Pc(p_{\max})$, consider running Algorithm \ref{alg:two-phase-bq} with $T$ observations being corrupted by Gaussian independent noises $\Nc(0,\sigma^2)$, and obtain the estimates $\fhat$ and $\Ihat$.  Then, the average error satisfies
    \begin{equation}
        \EE\big[|I-\Ihat|\big] \le 2\sqrt{p_{\max}} T^{-\frac{1}{2}} \EE\big[ \| f - \fhat \|_{L^2} \big] + 2\sigma T^{-\frac{1}{2}} ,
    \end{equation}
    where the expectation is averaged over the randomness of the points queried and the noise.
\end{thm}
For the Mat\'ern kernel, building on the results of \citep[Thm.~4]{Wyn21}, we obtain the following two corollaries. 

\begin{cor} \label{cor:avg_mat_sig}
    {\em (Average-Case Noisy Mat\'ern Upper Bound)} 
     For $f\in \mat$, consider the setup of Theorem \ref{thm:avg_int_l2}, where the subroutine \textsc{EstimateFunc} for producing $\fhat$ is maximum-variance sampling (Algorithm \ref{alg:max-var}) with parameter $\lambda=\Theta(T^{-\frac{\nu}{d}})$.  Then, the average-case integration error is upper bounded by
    \begin{equation}
        \ravgsigmat = O\Big(T^{-\frac{\nu}{d}-1} + \sigma T^{-\frac{1}{2}}\Big). \label{eq:matern_final}
    \end{equation}
\end{cor}

As discussed in Section \ref{sec:relate}, Corollary \ref{cor:avg_mat_sig} matches the lower bound (Theorem \ref{thm:noisy_lower}) up to constant factors, and shows that the overall difficulty of noisy BQ is as roughly hard as either noiseless BQ or univariate Gaussian mean estimation with variance $\sigma^2$ (whichever is harder).  Since the algorithm used is non-adaptive but the lower bound applies even to adaptive algorithms, we conclude that there is no adaptivity gap in terms of scaling laws in this case.

Similarly to prior works such as \citep{Kan16,Tec20,Wyn21}, we now consider the setting in which the smoothness hyperparameter $\nu$ is unknown, and Algorithm \ref{alg:max-var} is accordingly modified as follows:
\begin{itemize}
    \item Instead of assuming that $\nu$ is given (via the prior $k_0$), we assume that the algorithm is given a sequence of estimates $\{\nuhat_t\}_{t=1}^{T}$.  These are kept generic, but could correspond to estimates that are iteratively updated as more data is collected.
    \item When forming the GP posterior at time $t$, the parameter $\nuhat_t$ is used.
\end{itemize}
Following \citep{Wyn21}, given the time horizon $T$, we define $\num = \inf_{t\le T}\nuhat_t$ and $\nup = \sup_{t\le T}\nuhat_t$,\footnote{This can be generalized so that these definitions also restrict $t \ge N$ for some finite $N$, but we simply take $N=1$ to reduce notation.} and we assume that the number of distinct values in $\{\nuhat_t\}_{t=1}^{T}$ is upper bounded by fixed constant.

% and one has to estimate $\nu$ through a sequence of estimates $\{\nuhat_t\}_{t=1}^{\infty}$, so that the $t$-th node is observed with the presence of $\nuhat_t$.  For some $T\in \NN$, define $\num = \inf_{t\ge T}\nuhat_t$ and $\nup = \sup_{t\ge T}\nuhat_t$.  In this sense, the well-specified smoothness is that $\nu\ge\nup$, whereas the mis-specified smoothness is that $\nu<\nup$.  
% We use $x\vee y$ to denote $\max(x,y)$, and $x\wedge y$ to denote $\min(x,y)$

\begin{cor} \label{cor:avg_mat_sig_mis}
    {\em (Average-Case Noisy Mat\'ern Upper Bound -- Misspecified Setting)} 
     For $f\in \mat$, consider the setup of Theorem \ref{thm:avg_int_l2}, where the subroutine \textsc{EstimateFunc} for producing $\fhat$ is the above-described modification of maximum-variance sampling with parameters $\{\nuhat_t\}_{t=1}^{T}$ satisfying $\nup > \nu$, and with $\lambda=\Theta(T^{-\frac{\num}{d}})$.  Then, the average-case integration error is upper bounded by
    \begin{equation}
        \ravgsigmat = O\Big(T^{-\frac{\min(\num,\nu)}{d}-1} + T^{-\frac{\nu+\num-\nup}{d}-1} + \sigma T^{-\frac{1}{2}}\Big). \label{eq:misspec_final}
    \end{equation}
\end{cor}

As a special case of this result, when $\num = \nup$ (and both are greater than $\nu$, in accordance with the assumption $\nup > \nu$), the scaling precisely reduces to that of Corollary \ref{cor:avg_mat_sig}.  Thus, interestingly, over-estimating the smoothness parameter is not harmful in terms of scaling laws; similar observations were made in prior works such as \citep{Kan16} (Remark 2 therein).  More broadly, Theorem \ref{thm:avg_int_l2} can be used to convert other $L^2$ guarantees from \citep{Wyn21} (or from other works) to BQ guarantees, but for brevity we only formally state Corollary \ref{cor:avg_mat_sig_mis}.

% Our Theorem \ref{thm:avg_int_l2} suggests that, the scaling of the average quadrature error will be improved over the average $L^2$ function estimation error by a factor of $O(T^{-\frac{1}{2}})$, with an additional $\sigma T^{-\frac{1}{2}}$ noise term.  As can be seen that, such an error scaling has simultaneously manifested in the above two corollaries, further details can be found in Appendix \ref{app:proof_mat_cor}.
% \begin{cor} \label{cor:avg_se_nosig}
%     {\em (Average-Case Noiseless SE Upper Bound)} For $f\in\se$, under the setup of Theorem \ref{thm:avg_int_l2}, where the samples are selected with maximum variance sampling using Algorithms \ref{alg:two-phase-bq} and \ref{alg:max-var} with noise-free observations. Then, there exist constants $C_g,\Ctil_g >0$ depending only on $d$, such that we can set the GP noise variance $\lambda = \Theta(T^{-2C_gT^{\frac{1}{d}}} e^{-2\Ctil_g T^{\frac{1}{d}}})$, and get an average-case error bounded by
%     \begin{equation*}
%         \ravgse = O\Big(T^{- C_g T^{\frac{1}{d}}-\frac{1}{2}}\Big).
%     \end{equation*}
% \end{cor}

% We remark that the above used Algorithms \ref{alg:two-phase-bq} and \ref{alg:max-var}, in the noisy setting, are not applicable to the SE case.  This is since the essential quantity $\Lc=\|\kv(\xv_{T+1})^T(\Kv_T+\lambda\Iv)^{-1}\|_{L^1}$, $\forall \xv_{T+1}\notin \{\xv_t\}_{t=1}^T$, will not shrink for band-unlimited kernels such as SE.  In other words, $\|\kv(\xv)^T(\Kv_t+\lambda\Iv)^{-1}\beps\|_{L^2}$ that ambient in $\EE\big[ \| f - \mu_{T/2} \|_{L^2}^2 \big]$ is unbounded for the SE kernel with the growth of $T$.  Despite that, one may still use Algorithms \ref{alg:two-phase-bq} and \ref{alg:max-var} for one-dimensional SE kernel  functions, and get
% \begin{equation*}
%         \ravgsigse = O\Big(T^{-C_g T - \frac{1}{2}} + \sigma T^{-\frac{1}{2}}\Big), \quad d=1,
%     \end{equation*}n sdas
% since $1$-D SE kernel yields uniformly bounded $\Lc$ ($\Lc\le 1$), see \citep{Son13}.

%We remark that the above used Algorithms \ref{alg:two-phase-bq} and \ref{alg:max-var}, in the noisy setting, are not applicable to the SE case.  This is since the essential quantity $\Lc=\|\kv(\xv_{T+1})^T(\Kv_T+\lambda\Iv)^{-1}\|_{L^1}$, $\forall \xv_{T+1}\notin \{\xv_t\}_{t=1}^T$, will not shrink for band-unlimited kernels such as SE.  In other words, $\|\kv(\xv)^T(\Kv_t+\lambda\Iv)^{-1}\beps\|_{L^2}$ that ambient in $\EE\big[ \| f - \mu_{T/2} \|_{L^2}^2 \big]$ is unbounded for the SE kernel with the growth of $T$.   

We now turn to the SE kernel with noise, for which we follow the use of random features \citep{Rah07}.  we specifically build on \citep{Bac17}, which analyzes weighted random Fourier features from a function approximation point of view.  The approximation requires sampling from a leverage function distribution based on an infinite-dimensional integral operator.  With the help of their analysis, we  obtain the following corollary.

\begin{cor} \label{cor:avg_se_sig}
    {\em (Average-Case Noisy SE Upper Bound)} 
      For $f\in\se$, under the setup of Theorem \ref{thm:avg_int_l2}, there exists a random feature sampling algorithm that produces an approximation $\fhat$ in Algorithm \ref{alg:two-phase-bq} such that the average-case error is 
    \begin{equation*}
        \ravgsigse = O\Big(e^{-C_r (\frac{T}{\log T})^{\frac{1}{d}}}T^{-\frac{1}{2}} + \sigma T^{-\frac{1}{2}} \Big)
    \end{equation*}
    for some constant $C_r > 0$.
\end{cor}

In Section \ref{sec:intro}, we highlighted that BQ is related to RKHS-based optimization problems.  We briefly note that that the techniques from such works can also be used to obtain BQ bounds via Algorithm \ref{alg:max-var} (using it for $T$ observations rather than only the first half) or sampling on a uniform grid, but the resulting scaling is typically highly suboptimal.  Specifically, in Appendix \ref{app:alt_bo}, we show that this approach leads to the following:
\begin{align}
    &\ravgsigmat = O\Big(T^{-\frac{\nu}{2\nu+d}} (\log{T})^{\frac{4\nu+d}{4\nu+2d}}\Big),  \label{eq:mat_boup_sig}\\
    &\ravgmat = O\Big(T^{-\frac{\nu}{d}}\Big),  \label{eq:mat_boup_nosig}\\
    &\ravgsigse = O\Big((\log T)^{\frac{d+1}{2}} T^{-\frac{1}{2}}\Big),  \label{eq:se_boup_sig}\\
    &\ravgse = O\Big(e^{-\frac{d}{2} T^{\frac{1}{d}}} \Big), \label{eq:se_boup_nosig}
\end{align}
where \eqref{eq:mat_boup_sig} and \eqref{eq:se_boup_sig} hold under the assumption that $\sigma = \Theta(1)$.  These four results correspond to the Mat\'ern noisy/noiseless and SE noisy/noiseless settings respectively.  Algorithm \ref{alg:max-var} can be used directly to obtain the first three results, whereas \eqref{eq:se_boup_nosig} is based on sampling on a uniform grid.

While the first three bounds above are weaker than our earlier results, \eqref{eq:se_boup_nosig} gives fast decay to zero for the noiseless SE case.  Moreover, in Appendix \ref{app:alt_bo} we additionally show that \eqref{eq:se_boup_nosig} can be slightly reduced by a $T^{-\frac{1}{2}}$ factor using Algorithm \ref{alg:two-phase-bq}, as summarized in the following corollary.

\begin{cor} \label{cor:avg_se_nosig}
    {\em (Average-Case Noiseless SE Upper Bound)} 
      For $f\in\se$, consider the setup of Theorem \ref{thm:avg_int_l2}, where \textsc{EstimateFunc} is chosen to take samples on a uniformly-spaced grid and return $\mu_{T/2}$ with $\lambda = 0$.  Then, the average-case error is upper bounded by
    \begin{equation}\label{eq:avg_se_nosig}
        \ravgse = O\Big(e^{-\frac{d}{2} T^{\frac{1}{d}}} T^{-\frac{1}{2}}\Big).
    \end{equation}
\end{cor}

\section{Experiments} \label{sec:experiments}

In this section, we conduct simulation studies to compare our two-batch algorithm with its component parts, maximum variance sampling (MVS) and Monte Carlo sampling (MC).  These experiments serve to verify that Algorithm \ref{alg:two-phase-bq} can be effective in practice, but we will also discuss some potential gaps between the theory and practice.  In particular, our goal is \emph{not} to establish state-of-the-art practical performance.

We refer to Algorithm \ref{alg:max-var} as MVS-MAT or MVS-SE when the kernel is Mat\'ern or SE, and similarly for Algorithm \ref{alg:two-phase-bq} with MVS-MC-MAT or MVS-MC-SE.  
% our theory by comparing the two-batch method in Algorithm \ref{alg:two-phase-bq} (MVS-MC) to the individual components that make up its batches: Maximum-variance sampling (MVS) (see Algorithm \ref{alg:max-var-sampling} in Appendix \ref{app:max_var}), and Monte Carlo sampling (MC).
%
To attain a better understanding of how MVS-MC performs with respect to time, we modify it to {\em alternate} between MVS samples and MC samples, instead of doing all of one followed by all of the other.  Mathematically, this does not change the behavior at the {\em final} time step.

\subsection{Setup}
{\bf \noindent GP model.}  We adopt the common choice $\nu = 3/2$ for Mat\'ern-$\nu$ kernel, and the GP noise hyperparameter $\lambda$ is fixed as $10^{-4}$ for both kernels \footnote{Our theory uses choices such as $\lambda = \Theta(T^{-\frac{\nu}{d}})$ with unspecified implied constants, which makes it difficult to choose the parameter in a way that exactly matches the theory. 
 However, since the theory dictates choosing $\lambda$ to be small, we set it to be small here accordingly.}. 
 The lengthscale is left as a free parameter, as is an additional scale parameter that we introduce (multiplying \eqref{eq:kMat}) to permit functions with varying ranges.  Except where stated otherwise, these two parameters are learned by maximizing the data log-likelihood \citep{Ras06} using the  built-in SciPy optimizer based on L-BFGS-B, which is also used for finding the maximum variance point.  We seek to solve the BQ problem with a constant weight function, i.e., $p(\xv) = 1$.

{\bf \noindent Evaluation.}  We compare MVS-MC against its two components, MVS and Monte Carlo. For MVS and MVS-MC, we perform 100 trials, with each trial using a distinct set of 3 random initial points (but these are common to both methods).  For MC, since every round is already randomized, we simply run 100 trials without initial points.  For all functions, we consider a time horizon of $T = 250$, and evaluate the performance using the mean absolute error, with the ground truth value (and also $\Ihat_1$ at Line 7 of Algorithm \ref{alg:two-phase-bq}) being determined by 
% the SciPy \textsc{nquad} function 
trapezoidal rule with $10^5$ uniformly-spaced grid points (without noise).  Error bars in our plots indicate $\pm 0.5$ standard deviation with respect to the 100 trials.
% or exhaustive MC (in case {\em nquad} fails to give a fairly correct answer).

% {\bf \noindent Other details.}  We compute the approximate integral $\Ihat_1$ (see Line 7 of Algorithm \ref{alg:two-phase-bq}) using 
% the SciPy \textsc{nquad} function if the dimension is one.  For higher dimensions, we approximate it using 
% $10^5$ Monte Carlo iterations
% to avoid the potentially slow behavior of \textsc{nquad}.

{\bf \noindent Varying the split size.} In our theoretical analysis, we let MVS-MC use half of the samples for each component (MVS and MC).  However, in practice, it may be beneficial to allow different splits.  In our experiments, we additionally explore the effect of the split fraction, i.e., the fraction allocated to the MVS part, and plot the final error with respect to that fraction.  A split of 0 corresponds to MC, and a split of 1 corresponds to MVS.

\subsection{Results} \label{sec:results}
\begin{figure}[t]
\centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\sizecustom]{figs/synthetic/mat_syn4-0.5.pdf}
        \includegraphics[width=\sizecustom]{figs/splits/syn/split-mat_syn4-0.5.pdf}
        \includegraphics[width=\sizecustom]{figs/synthetic/se_syn4-0.1.pdf}
        \includegraphics[width=\sizecustom]{figs/splits/syn/split-se_syn4-0.1.pdf}
    \end{subfigure}
    
    % \vskip 0.1in
    % \begin{subfigure}{\columnwidth}
    % \centering
    % \end{subfigure}

    \caption{Results for synthetic functions. \label{fig:synthetic}}
    \vspace*{-1.5ex}
\end{figure}

We provide a selection of our results here, and give additional results in Appendix \ref{app:addexp}.   

\subsubsection{Synthetic Kernel-Based Functions}
We first simulate on a set of synthetic functions following the method of \citep{Jan20}, where each function is constructed by sampling $m=30d$ points, $\xvhat_1\ldots\xvhat_m$, uniformly on $[0,1]^d$, and $\ahat_1\ldots\ahat_m$ uniformly on $[-1,1]$.  The function is then defined as $f(\xv) = \sum_{i=1}^{m} \ahat_i k(\xvhat_i, \xv)$.  The length-scale and $\nu$ (in the case of the Mat\'ern kernel) are set to be fixed as $0.2$ and $3/2$ respectively.

We let MVS and MVS-MC know the kernel hyperparameters exactly (i.e., they match the ones used to produce the functions).  Some results for $d =4$ and $\sigma \in \{0.1,0.5\}$ are shown in Figure \ref{fig:synthetic}, and further $(d,\sigma)$ pairs are shown in Appendix \ref{app:addexp}.   We observe that MC performs well at the higher noise level, but performs poorly at the lower noise level, which aligns with the theory.  At the final time step, MVS in fact performs well in both cases, though it can perform poorly in the low-query regime (e.g., Mat\'ern 4D).  While MVS-MC is not universally best, it is generally able to capture the benefits of both MVS and MC in this experiment.


\subsubsection{Benchmark Functions and Sensor Measurement Function}
\begin{figure}[t]
\centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\sizecustom]{figs/benchmark/1d/ack1-0.5.pdf}
        \includegraphics[width=\sizecustom]{figs/benchmark/2d/keane-0.1.pdf}
        \includegraphics[width=\sizecustom]{figs/benchmark/2d/alp2-0.pdf}
        \includegraphics[width=\sizecustom]{figs/realworld/energy-0.1.pdf}
    \end{subfigure}
    
    \vskip 0.1in
    
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\sizecustom]{figs/splits/1d/split-ack1-0.5.pdf}
        \includegraphics[width=\sizecustom]{figs/splits/2d/split-keane-0.1.pdf}
        \includegraphics[width=\sizecustom]{figs/splits/2d/split-alp2-0.pdf}
        \includegraphics[width=\sizecustom]{figs/splits/split-energy-0.1.pdf}
    \end{subfigure}
    
    \caption{Results for benchmark and real data functions. \label{fig:benchmark}}
    % \vspace*{-1.5ex}
\end{figure}

We consider a variety of well-known benchmark functions, namely, Ackley, Alpine, Gramacy-Lee, Griewank and Keane; see \citep{SFU_Funcs} for the descriptions.  We also consider an experiment for sensor measurement data, which is described in Appendix \ref{app:addexp}. 
A small selection of the results are shown in Figure \ref{fig:benchmark}, and the rest are shown in Appendix \ref{app:addexp}.

These results again indicate that MC is better suited to higher noise levels, but they provide a somewhat less clear picture for MVS and the ideal MVS-MC split.  In general, the error as a function of the split fraction can increase, decrease, or exhibit ``U-shaped'' behavior, though we again found the choice of 0.5 to usually be a good one (even if not always optimal). 

Notably, in both the synthetic and benchmark experiments, the error can drop suddenly at $1.0$, as this is where the MC component is no longer used and MVS-MC simply becomes MVS.  This indicates that the theoretical benefits of MVS-MC over MVS may not always be observed in practice (e.g., because the theory hides important constant factors, or only captures the behavior for very large $T$).  It may be of interest to seek refined theory addressing these findings in future work.

% Here we see a clear trend of Monte Carlo suffering at low noise, MVS suffering at high noise, and MVS-MC performing well in both cases, consistent with our theory.  Thus, while MVS-MC does not perform best in each individual plot, it is generally able to attain the benefits of both MVS and MC, at least in these examples.



% \begin{figure}[!t]
% \centering
%     \begin{subfigure}{\columnwidth}
%     \centering
%     \end{subfigure}
    
%     \vskip 0.1in
        
%     \begin{subfigure}{\columnwidth}
%     \centering
%     \end{subfigure}
    
%     \caption{Comparison of different MVS-MC splits, i.e., the fraction of rounds for which MVS is used. \label{fig:split-1}}
% \end{figure}

% \subsection{Effect of Stochastic $\lambda$ for Mat\'ern Kernel}
% In theory, see Corollary \ref{cor:avg_mat_sig} for example, we need $\lambda=\Theta(T^{-\frac{\nu}{d}})$.  While all the previous experiments are conducted with $\lambda=10^{-5}$ to avoid heavy computation (since each trial has to be executed $T$ times), we would like to see the effect when $\lambda$ is exactly $T^{-\frac{\nu}{d}}$.  In Appendix \ref{app:sto_lambda}, we see that there is nearly no benefit to vary $\lambda$ for different $T$, since the convergence will be slower more erratic.

% \subsection{Effect of Grid Samples for SE Kernel}1


\section{Conclusion}

We have developed a framework for relating average-case quadrature error with $L^2$-function approximation error, allowing us to derive a number of both existing and new results.  In addition, we explored algorithm-independent lower bounds with greater generality and/or distinct proofs compared to existing ones.  In future work, it may be of interest to address some of the remaining gaps, such as those between the upper and lower bounds for the SE kernel (see Table \ref{tab:compare}).

% We have established tight scaling laws on the mean absolute error of noisy Bayesian quadrature for functions in an RKHS with Mat\'ern-$\nu$ kernel, showing a lower bound of $\Omega(T^{-\frac{\nu}{d}-1}+\sigma T^{-\frac{1}{2}})$ for any adaptive algorithm, and there exists a non-adaptive algorithm with a matching upper bound $O(T^{-\frac{\nu}{d}-1}+\sigma T^{-\frac{1}{2}})$. Thus, there is no adaptivity gap in terms of scaling laws.  

% Perhaps the most immediate direction for future work is to extend our results to other kernels, notably including (i) the Mat\'ern kernel with non-integer values of $\nu + d/2$, and (ii) the squared exponential kernel.  The former has the added difficulty of not being able to use the equivalence with the Sobolev class, and the latter has the added difficulty of not being able to use the bounded-support bump function (as it has infinite RKHS norm under the SE kernel).

% RKHS of squared exponential (SE) kernel. Our analysis requires that $\nu+d/2$ is an integer in order to establish an equivalence between RKHS of Mat\'ern kernel with Sobolev spaces. Another interesting direction would be to extend our analysis to the case where $\nu+d/2$ is not required to be an integer.

==> On Average-Case Error Bounds for Kernel-Based Bayesian Quadrature/preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{dsfont}
% \usepackage{cite}
\usepackage{amsmath}
\usepackage{array}
\usepackage{multirow}
\usepackage{caption}
\usepackage{color}
\usepackage{cancel}

\usepackage{multicol}

\theoremstyle{plain}
\newtheorem{claim}{\protect\claimname}
\theoremstyle{plain}
\newtheorem{prop}{\protect\propositionname}
\theoremstyle{plain}
\newtheorem{lem}{\protect\lemmaname}
\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\theoremstyle{plain}
\newtheorem{cor}{\protect\corollaryname}  
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\theoremstyle{definition}
\newtheorem{assump}{\protect\assumptionname}
\theoremstyle{definition}
\newtheorem{rem}{\protect\remarkname}

\renewenvironment{proof}{{\bf Proof. }}{\qed}

\makeatother
  
\usepackage{babel} 

\providecommand{\claimname}{Claim}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}
\providecommand{\corollaryname}{Corollary} 
\providecommand{\definitionname}{Definition}
\providecommand{\assumptionname}{Assumption}
\providecommand{\remarkname}{Remark}

\newcommand{\overbar}[1]{\mkern 1.25mu\overline{\mkern-1.25mu#1\mkern-0.25mu}\mkern 0.25mu}
\newcommand{\overbarr}[1]{\mkern 3.5mu\overline{\mkern-3.5mu#1\mkern-0.75mu}\mkern 0.75mu}
\newcommand{\mytilde}[1]{\mkern 0.5mu\widetilde{\mkern-0.5mu#1\mkern-0mu}\mkern 0mu}
\newcommand{\mytildee}[1]{\mkern 1.5mu\widetilde{\mkern-1.5mu#1\mkern-0mu}\mkern 0mu}
\newcommand{\mywidehat}[1]{\mkern 1.5mu\widehat{\mkern-1.5mu#1\mkern-0mu}\mkern 0mu}
  
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize} 
\newcommand{\openone}{\mathds{1}}

\newcommand{\todo}[1]{{\bf \color{red} [TODO: #1]}}

\newcommand{\alert}[1]{{\bf \color{red} [#1]}}

% BQ
\newcommand{\RMSE}{{\rm RMSE}}
% \newcommand{\Sv}{\mathbf{S}}
\newcommand{\Svhat}{\mywidehat{\mathbf{S}}}
\newcommand{\Shat}{\mywidehat{S}}

% Robust GP
\newcommand{\Dbar}{\overbar{D}}
\newcommand{\Rbar}{\overbar{R}}
\newcommand{\Runder}{\underline{R}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\kSE}{k_{\text{SE}}}
\newcommand{\kMat}{k_{\text{Mat\'ern}}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\Otil}{\tilde{O}}

% Other
\newcommand{\GP}{{\rm GP}}
\newcommand{\gv}{\mathbf{g}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\zvbar}{\overbar{\mathbf{z}}}

% Ranking and bandits
\newcommand{\thetamin}{\theta_{\mathrm{min}}}
\newcommand{\thetamax}{\theta_{\mathrm{max}}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\jworst}{j_{\mathrm{worst}}}
\newcommand{\Actil}{\widetilde{\mathcal{A}}}
% \newcommand{\Stil}{\widetilde{S}}
\newcommand{\mab}{\texttt{mab}}
\newcommand{\cmp}{\texttt{btl}}
\newcommand{\pemab}{P_{\mathrm{e},\texttt{mab}}}
\newcommand{\pecmp}{P_{\mathrm{e},\texttt{btl}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\Alg}{\mathrm{ALG}}
\newcommand{\Geometric}{\mathrm{Geometric}}
\newcommand{\Ttotal}{T_{\mathrm{total}}}
\newcommand{\jsec}{j_{\mathrm{sec}}}

% NoisyDD
\newcommand{\NDhat}{\widehat{\mathrm{ND}}}
\newcommand{\PDhat}{\widehat{\mathrm{PD}}}
% \newcommand{\Dhat}{\widehat{\mathrm{D}}}
% \newcommand{\Shat}{\widehat{S}}
\newcommand{\Ehat}{\widehat{E}}
\newcommand{\peid}{P_{\mathrm{e},1}^{(\mathrm{D})}}
\newcommand{\peind}{P_{\mathrm{e},1}^{(\mathrm{ND})}}
\newcommand{\peiid}{P_{\mathrm{e},2}^{(\mathrm{D})}}
\newcommand{\peiind}{P_{\mathrm{e},2}^{(\mathrm{ND})}}
\newcommand{\epsid}{\epsilon_{1}^{(\mathrm{D})}}
\newcommand{\epsind}{\epsilon_{1}^{(\mathrm{ND})}}
\newcommand{\epsiid}{\epsilon_{2}^{(\mathrm{D})}}
\newcommand{\epsiind}{\epsilon_{2}^{(\mathrm{ND})}}
\newcommand{\nid}{n_1^{(\mathrm{D})}}
\newcommand{\nind}{n_1^{(\mathrm{ND})}}
\newcommand{\niid}{n_2^{(\mathrm{D})}}
\newcommand{\niind}{n_2^{(\mathrm{ND})}}
\newcommand{\Npd}{N_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\Npnd}{N_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npd}{n_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\npnd}{n_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npos}{n_{\mathrm{pos}}}
\newcommand{\nneg}{n_{\mathrm{neg}}}
\newcommand{\Ntilpos}{\widetilde{N}_{\mathrm{pos}}}
% \newcommand{\Npos}{N_{\mathrm{pos}}}
% \newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Aid}{\mathcal{A}_{1,i}^{(\mathrm{D})}}
\newcommand{\Aind}{\mathcal{A}_{1,i}^{(\mathrm{ND})}}
\newcommand{\mutild}{\tilde{\mu}^{(\mathrm{D})}}
\newcommand{\mutilnd}{\tilde{\mu}^{(\mathrm{ND})}}

% OneDimBO

\newcommand{\diag}{\mathrm{diag}}
\newcommand{\cunder}{\underline{c}}
\newcommand{\cbar}{\overline{c}}
\newcommand{\bunder}{\underline{b}}
\newcommand{\bbar}{\overline{b}}
\newcommand{\aunder}{\underline{a}}
\newcommand{\abar}{\overline{a}}
\newcommand{\mutil}{\widetilde{\mu}}
\newcommand{\sigmatil}{\widetilde{\sigma}}
\newcommand{\Tearly}{T_{\mathrm{early}}}
\newcommand{\Tlate}{T_{\mathrm{late}}}
\newcommand{\Rearly}{R_{\mathrm{early}}}
\newcommand{\Rlate}{R_{\mathrm{late}}}
\newcommand{\Ctil}{\widetilde{C}}
\newcommand{\ctil}{\widetilde{c}}
\newcommand{\ftil}{\widetilde{f}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\LCB}{\mathrm{LCB}}
\newcommand{\UCBtil}{\widetilde{\mathrm{UCB}}}
\newcommand{\LCBtil}{\widetilde{\mathrm{LCB}}}
\newcommand{\Lctil}{\widetilde{\mathcal{L}}}
\newcommand{\Loss}{\mathrm{Loss}}

% NoisyAdaptiveGT

\newcommand{\nMIi}{n_{\mathrm{MI,1}}}
\newcommand{\nMIii}{n_{\mathrm{MI,2}}}
\newcommand{\nConc}{n_{\mathrm{Conc}}}
\newcommand{\nIndiv}{n_{\mathrm{Indiv}}}
\newcommand{\nHalving}{n_{\mathrm{Halving}}}
\newcommand{\kmax}{k_{\mathrm{max}}}
\newcommand{\ptil}{\widetilde{p}}
\newcommand{\elltil}{\widetilde{\ell}}
\newcommand{\Stil}{\widetilde{S}}
\newcommand{\ncheck}{\check{n}}

% SeparateGT

\newcommand{\cmean}{c_{\mathrm{mean}}}
\newcommand{\cvar}{c_{\mathrm{var}}}
\newcommand{\ccov}{c_{\mathrm{cov}}}
\newcommand{\cmax}{c_{\mathrm{max}}}

\newcommand{\dneg}{d_{\mathrm{neg}}}
\newcommand{\dpos}{d_{\mathrm{pos}}}
\newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Npos}{N_{\mathrm{pos}}}
\newcommand{\Nerr}{N_{\mathrm{err}}}
\newcommand{\alphaneg}{\alpha_{\mathrm{neg}}}
\newcommand{\alphapos}{\alpha_{\mathrm{pos}}}

\newcommand{\pej}{P_{\mathrm{e},j}}
\newcommand{\nusymm}{\nu_{\mathrm{symm}}}

% PooledData
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\CNrm}{\mathrm{CN}}

% ConverseGP
\newcommand{\vbar}{\overline{v}}

% GT_ICASSP

\newcommand{\pc}{P_{\mathrm{c}}}

% ActiveMRF

\newcommand{\lammin}{\lambda_{\mathrm{min}}}
\newcommand{\lammax}{\lambda_{\mathrm{max}}}
\newcommand{\missing}{\ast}
\newcommand{\pFAi}{p_{\mathrm{FA},i}}
\newcommand{\pMDi}{p_{\mathrm{MD},i}}
\newcommand{\bSigmatil}{\widetilde{\mathbf{\Sigma}}}
\newcommand{\mtil}{\widetilde{m}}
\newcommand{\Ptil}{\widetilde{P}}
\newcommand{\dmin}{d_{\mathrm{min}}}
\newcommand{\davg}{d_{\mathrm{avg}}}
\newcommand{\dmaxbar}{\overline{d}_{\mathrm{max}}}
\newcommand{\taumin}{\tau_{\mathrm{min}}}
\newcommand{\taumax}{\tau_{\mathrm{max}}}
\newcommand{\ntil}{\widetilde{n}}
\newcommand{\Ntil}{\widetilde{N}}
\newcommand{\Ncheck}{\check{N}}
\newcommand{\kbar}{\overbar{k}}

\newcommand{\mmin}{m_{\mathrm{min}}}
\newcommand{\mmax}{m_{\mathrm{max}}}

% PartialSBM
\newcommand{\ellv}{\boldsymbol{\ell}}
\newcommand{\Cieq}{C_{1,\mathrm{eq}}}
\newcommand{\Cidif}{C_{1,\mathrm{dif}}}
\newcommand{\Ctilde}{\tilde{C}}
\newcommand{\dbar}{\overline{d}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\ktilde}{\tilde{k}}
 
% GT_ISIT
\newcommand{\Veq}{V_{\mathrm{eq}}}
\newcommand{\Vdif}{V_{\mathrm{dif}}}
\newcommand{\Vveq}{\mathbf{V}_{\mathrm{eq}}}
\newcommand{\Vvdif}{\mathbf{V}_{\mathrm{dif}}}
\newcommand{\veq}{v_{\mathrm{eq}}}
\newcommand{\vdif}{v_{\mathrm{dif}}}

%
% MultiMRI
%
\newcommand{\bpsi}{\boldsymbol{\psi}}

%
% Group testing 
%
\newcommand{\Hg}{\mathrm{Hypergeometric}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\dTV}{d_{\mathrm{TV}}}

%
% Graphical model selection
%
\newcommand{\Gbar}{\overbar{G}}
\newcommand{\Mbar}{\overbar{M}}
\newcommand{\qmax}{q_{\mathrm{max}}}

%
% Community detection
%
\newcommand{\Bi}{\mathrm{Binomial}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ev}{\mathbf{E}}

%
% Support recovery
%
\newcommand{\Sbar}{\overbar{S}}
\newcommand{\sbar}{\overbar{s}}

%\newcommand{\Wdif}{W_{\mathrm{dif}}}
%\newcommand{\Weq}{W_{\mathrm{eq}}}
%\newcommand{\wdif}{w_{\mathrm{dif}}}
%\newcommand{\weq}{w_{\mathrm{eq}}}

\newcommand{\Sdif}{S_{\mathrm{dif}}}
\newcommand{\Seq}{S_{\mathrm{eq}}}
\newcommand{\sdif}{s_{\mathrm{dif}}}
\newcommand{\sdifbar}{\overbar{s}_{\mathrm{dif}}}
\newcommand{\seqbar}{\overbar{s}_{\mathrm{eq}}}
\newcommand{\seq}{s_{\mathrm{eq}}}
\newcommand{\sdifhat}{\hat{s}_{\mathrm{dif}}}
\newcommand{\sdifx}{\overbar{s} \backslash s}
\newcommand{\seqx}{\overbar{s} \cap s}

\newcommand{\Xvdif}{\mathbf{X}_{\overbar{s} \backslash s}}
\newcommand{\Xveq}{\mathbf{X}_{\overbar{s} \cap s}}
\newcommand{\Xvdifo}{\mathbf{X}_{s \backslash \overbar{s}}}
\newcommand{\xvdif}{\mathbf{x}_{\overbar{s} \backslash s}}
\newcommand{\xveq}{\mathbf{x}_{\overbar{s} \cap s}}
\newcommand{\xveqo}{\mathbf{x}_{s \backslash \overbar{s}}}

\newcommand{\Ord}{\mathcal{O}}
\newcommand{\Yctil}{\widetilde{\mathcal{Y}}}

\newcommand{\dmax}{d_{\mathrm{max}}}
\newcommand{\dH}{d_{\mathrm{H}}}

\newcommand{\jeq}{j_{\mathrm{eq}}}
\newcommand{\jdiff}{j_{\mathrm{dif}}}

\newcommand{\Zhat}{\hat{Z}}
\newcommand{\Zhatmax}{\hat{Z}_{\mathrm{max}}}
\newcommand{\zdiff}{z_{\mathrm{dif}}}
\newcommand{\zcomm}{z_{\mathrm{eq}}}

\newcommand{\bmin}{b_{\mathrm{min}}}
\newcommand{\Bmin}{\beta_{\mathrm{min}}}
\newcommand{\bmax}{b_{\mathrm{max}}}
\newcommand{\sigbeta}{\sigma_{\beta}}
\newcommand{\siglv}{\sigma_{\sdif}}
\newcommand{\Tr}{\mathrm{Tr}}

\newcommand{\sign}{\mathrm{sign}}
\newcommand{\SNRdB}{\mathrm{SNR}_{\mathrm{dB}}}

\newcommand{\Weq}{W_{\mathrm{eq}}}
\newcommand{\Wdif}{W_{\mathrm{dif}}}
\newcommand{\weq}{w_{\mathrm{eq}}}
\newcommand{\wdif}{w_{\mathrm{dif}}}
\newcommand{\feq}{f_{\mathrm{eq}}}
\newcommand{\fdif}{f_{\mathrm{dif}}}

\newcommand{\bgood}{b_{\mathrm{good}}}
\newcommand{\bbad}{b_{\mathrm{bad}}}

\newcommand{\btil}{\widetilde{b}}
\newcommand{\betatil}{\widetilde{\beta}}
\newcommand{\betatileq}{\widetilde{\beta}_{\mathrm{eq}}}
\newcommand{\betatildif}{\widetilde{\beta}_{\mathrm{dif}}}
\newcommand{\btileq}{\widetilde{b}_{\mathrm{eq}}}
\newcommand{\btildif}{\widetilde{b}_{\mathrm{dif}}}
\newcommand{\stileq}{\widetilde{s}_{\mathrm{eq}}}
\newcommand{\stildif}{\widetilde{s}_{\mathrm{dif}}}
\newcommand{\pieq}{\pi_{\mathrm{eq}}}
\newcommand{\pidif}{\pi_{\mathrm{dif}}}
\newcommand{\Sdifhat}{\hat{S}_{\mathrm{dif}}}

\newcommand{\Bcfano}{\mathcal{B}'_{\mathrm{Fano}}}

\newcommand{\Sceq}{\mathcal{S}_{\mathrm{eq}}}
\newcommand{\Scdif}{\mathcal{S}_{\mathrm{dif}}}
\newcommand{\Nc}{\mathcal{N}}

%
% From MultiMRI
%
\newcommand{\Pv}{\mathbf{P}}
\newcommand{\Wvtil}{\widetilde{\mathbf{W}}}
\newcommand{\wtil}{\widetilde{w}}
\newcommand{\xvhat}{\hat{\mathbf{x}}}

%
% From Expanders_FOCS
%
\newcommand{\Bernoulli}{\mathrm{Bernoulli}}
\newcommand{\Binomial}{\mathrm{Binomial}}
\newcommand{\imtil}{\tilde{\imath}}
\newcommand{\SNR}{\mathrm{SNR}}

%
% From PaperBI
%
\newcommand{\CLM}{C_{\mathrm{LM}}}
\newcommand{\CSC}{C_{\mathrm{SC}}}
\newcommand{\ISC}{I_{\mathrm{SC}}}
\newcommand{\CM}{C_{\mathrm{M}}}
\newcommand{\Qmin}{Q_{\mathrm{min}}}
\newcommand{\Phat}{\widehat{P}}

%
% From JournalSU
%
\newcommand{\pebar}{\overbar{P}_{\mathrm{e}}}
\newcommand{\petilde}{\tilde{p}_{\mathrm{e}}}
\newcommand{\pe}{P_{\mathrm{e}}}
\newcommand{\pen}{P_{\mathrm{e},n}}
\newcommand{\peQ}{P_{\mathrm{e},Q}} 
\newcommand{\pemax}{P_{\mathrm{e},\mathrm{max}}} 
\newcommand{\msg}{\mathsf{m}}

\newcommand{\Ez}{E_{0}}
\newcommand{\Er}{E_{\mathrm{r}}}
\newcommand{\Esp}{E_{\mathrm{sp}}}
\newcommand{\Eziid}{E_{0}^{\mathrm{iid}}}
\newcommand{\Ezcc}{E_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcc}{\hat{E}_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcost}{\hat{E}_{0}^{\mathrm{cost}}}
\newcommand{\Ezcost}{E_{0}^{\mathrm{cost}}}
\newcommand{\Ezcostprime}{E_{0}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eriid}{E_{\mathrm{r}}^{\mathrm{iid}}}
\newcommand{\Ercc}{E_{\mathrm{r}}^{\mathrm{cc}}}
\newcommand{\Erccprime}{E_{\mathrm{r},12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Ercost}{E_{\mathrm{r}}^{\mathrm{cost}}}
\newcommand{\Ercostprime}{E_{\mathrm{r}}^{\mathrm{cost}^{\prime}}}

\newcommand{\rcu}{\mathrm{rcu}}
\newcommand{\rcus}{\rcu_{s}}
\newcommand{\rcuss}{\rcu_{s}^{*}}
\newcommand{\rcusa}{\rcu_{s,a}^{*}}
\newcommand{\rcushat}{\widehat{\mathrm{rcu}}_{s}}
\newcommand{\rcusshat}{\widehat{\mathrm{rcu}}_{s}^{*}}
\newcommand{\alphasa}{\alpha^{\mathrm{iid}}}
\newcommand{\rcul}{\rcu_{\mathrm{L}}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\LM}{I_{\mathrm{LM}}}
\newcommand{\GMI}{I_{\mathrm{GMI}}}

\newcommand{\SetScc}{\mathcal{S}}
\newcommand{\SetSncc}{\mathcal{S}_{n}}
\newcommand{\SetSncost}{\mathcal{S}_{n}}
\newcommand{\SetSiid}{\mathcal{S}^{\mathrm{iid}}}
\newcommand{\SetScost}{\mathcal{S}}
\newcommand{\SetSniid}{\mathcal{S}_{n}^{\mathrm{iid}}}
\newcommand{\SetTcc}{\mathcal{T}}
\newcommand{\SetTiid}{\mathcal{T}^{\mathrm{iid}}}
\newcommand{\SetTcost}{\mathcal{T}}
\newcommand{\SetTncost}{\mathcal{T}_{n}}
\newcommand{\SetTncc}{\mathcal{T}_{n}}

\newcommand{\Miid}{M^{\mathrm{iid}}}
\newcommand{\Mcc}{M^{\mathrm{cc}}}
\newcommand{\Mcost}{M^{\mathrm{cost}}}
\newcommand{\Rcr}{R_{\mathrm{cr}}}
\newcommand{\Rcrs}{R_s^{\mathrm{cr}}}

\newcommand{\Fbar}{\overbar{F}}
\newcommand{\Funder}{\underline{F}}
\newcommand{\Gunder}{\underline{G}}
\newcommand{\PXv}{P_{\Xv}}
\newcommand{\qbar}{\overbar{q}}
\newcommand{\rbar}{\overbar{r}}
\newcommand{\rtilde}{\tilde{r}}
\newcommand{\atilde}{\tilde{a}}
\newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\Mtilde}{\mytildee{M}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Rtilde}{\mytildee{R}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Wvtilde}{\widetilde{\mathbf{W}}}
\newcommand{\hover}{\overbar{h}}
\newcommand{\ubar}{\overbar{u}}
\newcommand{\Ubar}{\overbar{U}}
\newcommand{\xbarbar}{\overbar{\overbar{x}}}
\newcommand{\Xbarbar}{\overbar{\overbar{X}}}
\newcommand{\xbar}{\overbar{x}}
\newcommand{\Xbar}{\overbar{X}}
\newcommand{\xtilde}{\widetilde{x}}
\newcommand{\Xtilde}{\mytilde{X}}
\newcommand{\ybar}{\overbar{y}}
\newcommand{\zbar}{\overbar{z}}
\newcommand{\Zbar}{\overbar{Z}}
\newcommand{\thetabar}{\overbar{\theta}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\Qv}{\mathbf{Q}}
\newcommand{\uvbar}{\overbar{\mathbf{u}}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\Uvbar}{\overbar{\mathbf{U}}}
\newcommand{\Uv}{\mathbf{U}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\Vv}{\mathbf{V}}
\newcommand{\vvbar}{\overbar{\mathbf{v}}}
\newcommand{\xvbarbar}{\overbar{\overbar{\mathbf{x}}}}
\newcommand{\xvbar}{\overbar{\mathbf{x}}}
\newcommand{\xvtilde}{\widetilde{\mathbf{x}}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\Xvbarbar}{\overbar{\overbar{\mathbf{X}}}}
\newcommand{\Xvbar}{\overbar{\mathbf{X}}}
\newcommand{\Xvtilde}{\mytilde{\mathbf{X}}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Yvtilde}{\widetilde{\mathbf{Y}}}
\newcommand{\Xv}{\mathbf{X}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\Yv}{\mathbf{Y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\Zv}{\mathbf{Z}}

\newcommand{\Yvs}{\mathbf{Y}_{\hspace*{-0.5ex}s}}
\newcommand{\Uvn}{\mathbf{U}_{\hspace*{-0.3ex}n}}
\newcommand{\Tvn}{\mathbf{T}_{\hspace*{-0.3ex}n}} 
\newcommand{\Vvi}{\mathbf{V}_{\hspace*{-0.3ex}1}} 
\newcommand{\Vvii}{\mathbf{V}_{\hspace*{-0.3ex}2}}
\newcommand{\Vvm}{\mathbf{V}_{\hspace*{-0.3ex}m}}
\newcommand{\Vvtilden}{\widetilde{\mathbf{V}}_{\hspace*{-0.3ex}n}}   
\newcommand{\QUn}{Q_{U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QXgUn}{Q_{X|U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QUXn}{Q_{UX\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\Yvi}{\mathbf{Y}_{\hspace*{-0.5ex}1}}
\newcommand{\Yvii}{\mathbf{Y}_{\hspace*{-0.5ex}2}}
\newcommand{\Yvu}{\mathbf{Y}_{\hspace*{-0.5ex}u}}

\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\ic}{\mathcal{i}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\Qsf}{\mathsf{Q}}

\newcommand{\al}{\{a_l\}}
\newcommand{\rl}{\{r_l\}}
\newcommand{\rbarl}{\{\overbar{r}_l\}}
\newcommand{\defeq}{\triangleq}
\newcommand{\deq}{\stackrel{d}{=}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\erfcxi}{\mathrm{erfcx}_{1}}
\newcommand{\erfcx}{\mathrm{erfcx}}
\newcommand{\erfc}{\mathrm{erfc}}
\newcommand{\supp}{\mathrm{supp}}

\newcommand{\alphanl}{\alpha^{\mathrm{nl}}_n}
\newcommand{\alphal}{\alpha^{\mathrm{l}}_n}
\newcommand{\betanl}{\beta^{\mathrm{nl}}_n}
\newcommand{\betal}{\beta^{\mathrm{l}}_n}

\newcommand{\Es}{E_{\mathrm{s}}}
\newcommand{\EJ}{E_{\mathrm{J}}}
\newcommand{\EJi}{E_{\mathrm{J},1}}
\newcommand{\EJii}{E_{\mathrm{J},2}}

\newcommand{\Vmin}{V_{\mathrm{min}}}
\newcommand{\Vmax}{V_{\mathrm{max}}}

%
% From PaperExpurgated
%

\newcommand{\rcux}{\mathrm{rcux}}

\newcommand{\Eexiid}{E_{\mathrm{ex}}^{\mathrm{iid}}}
\newcommand{\Eexcc}{E_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexhatcc}{\hat{E}_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexcost}{E_{\mathrm{ex}}^{\mathrm{cost}}}
\newcommand{\Eexcostprime}{E_{\mathrm{ex}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Exiid}{E_{\mathrm{x}}^{\mathrm{iid}}}
\newcommand{\Excc}{E_{\mathrm{x}}^{\mathrm{cc}}}
\newcommand{\Excost}{E_{\mathrm{x}}^{\mathrm{cost}}}
\newcommand{\Excoststar}{E_{\mathrm{x}}^{\mathrm{cost}^{*}}}
\newcommand{\Excostprime}{E_{\mathrm{x}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eex}{E_{\mathrm{ex}}}
\newcommand{\Ex}{E_{\mathrm{x}}}

\newcommand{\Pxbicm}{P_{X}^{\rm bicm}}

\newcommand{\Av}{\mathbf{A}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\mbar}{\overbar{m}}
\newcommand{\tv}{\mathbf{t}}

\newcommand{\Lsf}{\mathsf{L}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\csf}{\mathsf{c}}
\newcommand{\Fsf}{\mathsf{F}}
\newcommand{\Tsf}{\mathsf{T}}

\newcommand{\brl}{\{\overbar{r}_l\}}

%
% From DocumentMU
%

\newcommand{\peobar}{\overbar{p}_{\mathrm{e},0}}
\newcommand{\peibar}{\overbar{p}_{\mathrm{e},1}}
\newcommand{\peiibar}{\overbar{p}_{\mathrm{e},2}}
\newcommand{\peiiibar}{\overbar{p}_{\mathrm{e},12}}
\newcommand{\peo}{P_{\mathrm{e},0}}
\newcommand{\pei}{P_{\mathrm{e},1}}
\newcommand{\peii}{P_{\mathrm{e},2}}
\newcommand{\peiii}{P_{\mathrm{e},12}}
\newcommand{\rcuo}{\mathrm{rcu}_{0}}
\newcommand{\rcui}{\mathrm{rcu}_{1}}
\newcommand{\rcuii}{\mathrm{rcu}_{2}}
\newcommand{\rcuiii}{\mathrm{rcu}_{12}}
\newcommand{\rcuiiiprime}{\mathrm{rcu}_{12}^{\prime}}
\newcommand{\rcuiiia}{\mathrm{rcu}_{12,1}}
\newcommand{\rcuiiib}{\mathrm{rcu}_{12,2}}

\newcommand{\Eiziid}{E_{0,1}^{\mathrm{iid}}}
\newcommand{\Eiiziid}{E_{0,2}^{\mathrm{iid}}}
\newcommand{\Eiiiziid}{E_{0,12}^{\mathrm{iid}}}
\newcommand{\Eiiiaziid}{E_{0,12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibziid}{E_{0,12,2}^{\mathrm{iid}}}
\newcommand{\Eozcc}{E_{0,0}^{\mathrm{cc}}}
\newcommand{\Eizcc}{E_{0,1}^{\mathrm{cc}}}
\newcommand{\Eiizcc}{E_{0,2}^{\mathrm{cc}}}
\newcommand{\Eiiizcc}{E_{0,12}^{\mathrm{cc}}}
\newcommand{\Eiiizccprime}{E_{0,12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eiiizccpprime}{E_{0,12}^{\mathrm{cc}^{\prime\prime}}}
\newcommand{\Eiiiazcc}{E_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibzcc}{E_{0,12,2}^{\mathrm{cc}}}
\newcommand{\Ehatiiiazcc}{\hat{E}_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eozcost}{E_{0,0}^{\mathrm{cost}}}
\newcommand{\Eizcost}{E_{0,1}^{\mathrm{cost}}}
\newcommand{\Eiizcost}{E_{0,2}^{\mathrm{cost}}}
\newcommand{\Eiiizcost}{E_{0,12}^{\mathrm{cost}}}
\newcommand{\Eiiiazcost}{E_{0,12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibzcost}{E_{0,12,2}^{\mathrm{cost}}}
\newcommand{\Eiiizaccts}{E_{0,12,1}^{\text{cc-ts}}}

\newcommand{\Eiriid}{E_{\mathrm{r},1}^{\mathrm{iid}}}
\newcommand{\Eiiriid}{E_{\mathrm{r},2}^{\mathrm{iid}}}
\newcommand{\Eiiiriid}{E_{\mathrm{r},12}^{\mathrm{iid}}}
\newcommand{\Eiiiariid}{E_{\mathrm{r},12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibriid}{E_{\mathrm{r},12,2}^{\mathrm{iid}}}
\newcommand{\Eorcc}{E_{\mathrm{r},0}^{\mathrm{cc}}}
\newcommand{\Eorccprime}{E_{\mathrm{r},0}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eircc}{E_{\mathrm{r},1}^{\mathrm{cc}}}
\newcommand{\Eiircc}{E_{\mathrm{r},2}^{\mathrm{cc}}}
\newcommand{\Eiiircc}{E_{\mathrm{r},12}^{\mathrm{cc}}}
\newcommand{\Eiiiarcc}{E_{\mathrm{r},12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibrcc}{E_{\mathrm{r},12,2}^{\mathrm{cc}}}
\newcommand{\Eorcost}{E_{\mathrm{r},0}^{\mathrm{cost}}}
\newcommand{\Eircost}{E_{\mathrm{r},1}^{\mathrm{cost}}}
\newcommand{\Eiircost}{E_{\mathrm{r},2}^{\mathrm{cost}}}
\newcommand{\Eiiircost}{E_{\mathrm{r},12}^{\mathrm{cost}}}
\newcommand{\Eiiiarcost}{E_{\mathrm{r},12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibrcost}{E_{\mathrm{r},12,2}^{\mathrm{cost}}}
\newcommand{\Eiiirtilde}{\widetilde{E}_{\mathrm{r,12}}}
\newcommand{\Eiiirccts}{E_{\mathrm{r},12}^{\text{cc-ts}}}

\newcommand{\Wsu}{W^{\prime}}
\newcommand{\qsu}{q^{\prime}}
\newcommand{\RegLM}{\mathcal{R}_{\mathrm{LM}}}
\newcommand{\RegLMex}{\mathcal{R}_{\mathrm{ex}}}

\newcommand{\SetSccts}{\mathcal{S}^{\mathrm{ts}}}
\newcommand{\SetTocc}{\mathcal{T}_0}
\newcommand{\SetToncc}{\mathcal{T}_{0,n}}
\newcommand{\SetTicc}{\mathcal{T}_{1}}
\newcommand{\SetTiicc}{\mathcal{T}_{2}}
\newcommand{\SetTiiicc}{\mathcal{T}_{12}}
\newcommand{\SetTiiincc}{\mathcal{T}_{12,n}}
\newcommand{\SetTnucc}{\mathcal{T}_{\nu}}
\newcommand{\SetTnuccex}{\mathcal{T}_{\nu}^{\mathrm{ex}}}
\newcommand{\SetTiccex}{\mathcal{T}_{1}^{\mathrm{ex}}}
\newcommand{\SetTiiccex}{\mathcal{T}_{2}^{\mathrm{ex}}}
\newcommand{\SetTiiiccex}{\mathcal{T}_{12}^{\mathrm{ex}}}
\newcommand{\SetTiccts}{\mathcal{T}_{1}^{\mathrm{ts}}}
\newcommand{\SetTiiccts}{\mathcal{T}_{2}^{\mathrm{ts}}}
\newcommand{\SetTiiiccts}{\mathcal{T}_{12}^{\mathrm{ts}}}

\newcommand{\qv}{\mathbf{q}}
\newcommand{\Wv}{\mathbf{W}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Vc}{\mathcal{V}}

\newcommand{\Rsc}{R^{\mathrm{sc}}}
\newcommand{\Rmac}{R^{\mathrm{ex}}}
\newcommand{\Rosc}{R_{0}^{\mathrm{sc}}}
\newcommand{\Risc}{R_{1}^{\mathrm{sc}}}
\newcommand{\Rimac}{R_{1}^{\mathrm{ex}}}
\newcommand{\Riimac}{R_{2}^{\mathrm{ex}}}
\newcommand{\Usc}{U^{\mathrm{sc}}}
\newcommand{\Ucsc}{\mathcal{U}^{\mathrm{sc}}}
\newcommand{\Ximac}{X_{1}^{\mathrm{ex}}}
\newcommand{\Xcimac}{\mathcal{X}_{1}^{\mathrm{ex}}}
\newcommand{\Xiimac}{X_{2}^{\mathrm{ex}}}
\newcommand{\Xciimac}{\mathcal{X}_{2}^{\mathrm{ex}}}

\newcommand{\PrML}{\PP^{(\mathrm{ML})}}
\newcommand{\PrS}{\PP^{(\mathrm{S})}}
\newcommand{\PrGenie}{\PP^{(\mathrm{Genie})}}

%
% From MAC2OR
%
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Iv}{\mathbf{I}}
\newcommand{\iv}{\mathbf{i}}
\newcommand{\Fv}{\mathbf{F}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\Mv}{\mathbf{M}}
\newcommand{\Jv}{\mathbf{J}}
\newcommand{\Kv}{\mathbf{K}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\Lv}{\mathbf{L}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\Sv}{\mathbf{S}}
\newcommand{\Tv}{\mathbf{T}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\Qinv}{\mathsf{Q}_{\mathrm{inv}}}

%
% From RefinementCC
%
\newcommand{\Wocc}{\mathcal{W}_{0}^{\mathrm{cc}}}
\newcommand{\Wosymm}{\mathcal{W}_{0}^{\mathrm{symm}}}
\newcommand{\Wsymm}{\mathcal{W}^{\mathrm{symm}}}
\newcommand{\Qocc}{\mathcal{Q}_{0}^{\mathrm{cc}}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\Ezxcc}{E_{0,x}^{\mathrm{cc}}}
\newcommand{\Ezxicc}{E_{0,x_{i}}^{\mathrm{cc}}}
\newcommand{\Rcrsa}{R_{s,a}^{\mathrm{cr}}}
\newcommand{\mineq}{m_{\mathrm{ineq}}}
\newcommand{\meq}{m_{\mathrm{eq}}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\ferm}{f_{\mathrm{erm}}}
\newcommand{\dVC}{d_{\mathrm{VC}}}
\newcommand{\Rchat}{\hat{\Rc}}
\newcommand{\Dtrain}{\Dc_{\mathrm{train}}}
\newcommand{\Dval}{\Dc_{\mathrm{val}}}
\newcommand{\Dtest}{\Dc_{\mathrm{test}}}
\newcommand{\Fall}{\Fc_{\mathrm{all}}}
\newcommand{\fopt}{f_{\mathrm{opt}}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\BIC}{\mathrm{BIC}}
\newcommand{\AIC}{\mathrm{AIC}}

\newcommand{\Bs}{\mathsf{B}}
\newcommand{\Oc}{\mathcal{O}}

\newcommand{\rwst}{\mathcal{E}_{\rm wst}^k(T)}
\newcommand{\ravg}{\mathcal{E}_{\rm avg}^k(T)}
\newcommand{\ravgsig}{\mathcal{E}_{\rm avg}^k(T,\sigma)}

\newcommand{\rwstmat}{\mathcal{E}_{\rm wst}^{\rm M}(T)}
\newcommand{\ravgmat}{\mathcal{E}_{\rm avg}^{\rm M}(T)}
\newcommand{\ravgsigmat}{\mathcal{E}_{\rm avg}^{\rm M}(T,\sigma)}

\newcommand{\rwstse}{\mathcal{E}_{\rm wst}^{\rm SE}(T)}
\newcommand{\ravgse}{\mathcal{E}_{\rm avg}^{\rm SE}(T)}
\newcommand{\ravgsigse}{\mathcal{E}_{\rm avg}^{\rm SE}(T,\sigma)}

\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\fhatsig}{\hat{f}_{\sigma}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Ihatsig}{\hat{I}_{\sigma}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Fbump}{\Fc_{\mathrm{bump}}}
\newcommand{\sob}{W_2^s}
\newcommand{\mat}{\Hc_{\rm M}}
\newcommand{\se}{\Hc_{\rm SE}}
\newcommand{\matsub}{\overline{\Hc}_{\rm M}}
\newcommand{\Hk}{\Hc_{k}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\ahat}{\hat{a}}
\newcommand{\NNd}{\mathbb{N}_{0}^{d}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\Lk}{L_k}
\newcommand{\knu}{k_{\rm M}}
\newcommand{\kse}{k_{\rm SE}}
\newcommand{\bthetahat}{\hat{\boldsymbol{\theta}}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\Upsilonhat}{\hat{\Upsilon}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\khat}{\hat{k}}
\newcommand{\Sigmahat}{\hat{\Sigma}}
\newcommand{\Hchat}{\hat{\mathcal{H}}}

\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\num}{\nu^{-}}
\newcommand{\nup}{\nu^{+}}

==> On Average-Case Error Bounds for Kernel-Based Bayesian Quadrature/se.tex <==
% \begin{thm}\label{thm:noiseless_lower}
%     {\em (Average-Case Noiseless SE Lower Bound)}
%     Consider our problem setup with constant parameters $(B,d,l,T)$.  Then, there exists a constant $C_l>0$ such that for any algorithm (possibly adaptive and/or randomized) for estimating $I(f)$ with $f\in \se$, the average-case error is at least:
%         \begin{equation}\label{eq:se_lb_nosig}
%             \ravgse = \Omega\big(e^{-C_l T^{\frac{2}{d}}} T^{-1} \big).
%         \end{equation}
%     Moreover, this lower bound holds even under the fixed weight function $p(\xv) = 1$.
% \end{thm}

\begin{thm} \label{thm:wst_se_nosig}
    {\em (Worst-Case Noiseless SE Upper Bound)} For $f$ lies in SE RKHS with $\|f\|_{\se}\le B$, then, any linear algorithm that uses the linear combination of noiseless function evaluations satisfies the following regrets: 
    \begin{enumerate}
        \item If the algorithm is tensor-product based Gauss-Hermite rule, then
        \begin{equation}
            \rwstse \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}},
        \end{equation}
        where $C_{gh} = B\big(\frac{e}{l^2}\big)^{\frac{d}{2}T^{\frac{1}{d}}}$.
        \item If the algorithm simply combines $\sum_{t=1}^{T} w_t f(\xv_t)$ for arbitrary $\{\xv_t\}_{t=1}^{T}$, with $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$, then:
        \begin{equation}
            \rwstse \le (C_l+1) C_{gh} T^{-\frac{1}{2}T^{\frac{1}{d}}},
        \end{equation}
        where $C_l:=\sqrt{\big(\frac{\pi}{6}\big)^d + o(1)}$.
    \end{enumerate}
\end{thm}

The above results indicate that Gauss-Hermite rules are not necessary in solving noiseless SE kernel quadrature, at least not in a bounded domain, since the error only differs by a constant factor.

The RKHS function class induced by SE kernel $\kse(\xv,\xv')=\exp\big(-\frac{\|\xv-\xv'\|^2}{2 l^2}\big)$ can be defined by
\begin{equation}
    \se = \Big\{f(\xv)=\sum_{\balpha\in\NNd} \theta_{\balpha} e_{\balpha}(\xv), \|f\|_{\se}^2:=\sum_{\balpha\in\NNd} \theta_{\balpha}^2 < \infty \Big\}, \label{eq:se_rkhs}
\end{equation}
where $\NN_0:=\NN\cup\{0\}$, and $\big\{e_{\balpha}(\xv) = \prod_{i=1}^{d} \frac{1}{l^{\balpha_i}\sqrt{\balpha_i !}} \xv_i^{\balpha_i} \exp\big(-\frac{\xv_i^2}{2l^2}\big)\big\}_{\balpha\in\NNd}$ forms an orthonormal
basis for $\se$.  The details of this SE RKHS function class can be found in \cite{Ste06} and \cite{Min10}.  By denoting $\balpha ! = \prod_{i=1}^{d} \balpha_i !$ and $\xv^{\balpha}  = \prod_{i=1}^{d} \xv_i^{\balpha_i}$, we can simplify the notion as 
\begin{equation}
    e_{\balpha}(\xv) = \frac{1}{l^{|\balpha|}\sqrt{\balpha !}} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big) = \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big),
\end{equation}
with $\mu_{\balpha} := \frac{1}{l^{|\balpha|}\sqrt{\balpha !}}$.



\section{Proof for Theorem \ref{thm:noiseless_lower} (Average-case SE Lower Bound)}\label{app:se_avg_lb}
% \subsection{Function Class Construction}
Instead of specifying the function class in the case of the SE kernel directly, we consider the bump function $\Phi(\bxi)=\exp(\frac{-1}{1-\|\bxi\|^2})\openone\{\|\bxi\|<1\}$ in the frequency domain.  Since $\Phi(\bxi)$ is infinitely differentiable, its inverse Fourier transform, $\phi(\xv)$, decays to zero as $\|\xv\|\rightarrow\infty$, at a rate faster than any finite power of $\|\xv\|^{-1}$.  Then, there exists a point $\bzeta=[\zeta,\ldots,\zeta]$ such that $\phi(\bzeta) \le \frac{1}{d\zeta^{n}}$ for $n$ sufficiently large.  We choose $\psi(\xv)=\frac{\epsilon}{\phi(\bzero)}\phi(\frac{\xv\zeta}{\omega})$ in the similar fashion as of $g(\xv)$ in the previous section, where $\omega$ is the diameter of the gird.  Let $\psi_1(\xv),\ldots,\psi_M(\xv)$ denote the shifted version of $\psi(\xv)$ which centered at the $M$ grids respectively.  

% Before preceding, the following lemma is useful for functions $\{\psi_i(\xv)\}$.
% \begin{lem} \label{lem:func_sum_bound}
%     {\em (\citep[Lemma 7]{Sca17a})}
%     The functions $\{\psi_j(\xv)\}$ established as above are such that the quantities $\vbar_i^j:=\max_{\xv\in D_i} |\psi_j(\xv)|$ satisfy $\sum_{j=1}^{M} (\vbar_i^j)^2 = O(\epsilon^2)$.
% \end{lem}

For functions of the form $\rho(\xv):=\sum_{i=1}^{M}\delta_i\psi_i(\xv)$, letting $I_i:=\int_{\xv\in D_i}\rho(\xv)d\xv$ denote the integral of $\rho(\xv)$ in cell $i$, then for $\delta_i=1$, $I_i$ is at least:
\begin{align}
    I_i &= \int_{\xv\in D_i}\rho(\xv)d\xv \nonumber\\
    &= \int_{\xv\in D_i}\sum_{j=1}^{M} \delta_j \psi_j(\xv) d\xv \nonumber\\
    &\ge \int_{\xv\in D_i} \psi_i(\xv) d\xv - \sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv. \label{eq:se_inti_lower1}
\end{align}
The first integral in the above equation is the area of the dominate bump of $\psi_i$, which is at least $\Omega(\omega^d \epsilon)$.  It now remains to determine the magnitude of $I_i':=\sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv$:
\begin{align}
    I_i' &= \sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv \nonumber\\
    &= O\big((M-1) w^d |\psi(\bw)| \big)  \nonumber\\
    &= O\Big( M w^d \frac{\epsilon}{\phi(\bzero)}|\phi(\bzeta)| \Big)\nonumber\\
    &= O\Big( \frac{\epsilon}{\phi(\bzero) d\zeta^n} \Big)\nonumber,
\end{align}
where we have used $M=\lfloor \frac{1}{\omega}\rfloor^d$.  It is easy to choose constants $n=c'n'$ such that $\zeta^{c'}>\omega^{-1}$, and $n'>d$, so that $\zeta^n = \zeta^{c'n'} > \omega^{-d}$.  From function construction perspective, for our current choice of $\zeta$ and $n$, each of the $\psi_i(\xv)$ is now principally ``well-separated''.  Therefore $I_i'= O(\omega^d \epsilon)$, which can be absorbed into the first term of \eqref{eq:se_inti_lower1}, and obtain
\begin{equation}\label{eq:se_inti_lower}
    I_i = \Omega\Big(\frac{\epsilon}{M}\Big).
\end{equation}
% Note also that if we only consider the dominate bump of cell $i$, $\psi_i(\xv)$, the integral of cell $i$ will be at least $\Omega(\omega^d\epsilon)$.  Combining this with \eqref{eq:cellint_upper}, we find that $I_i^2 = \Theta(\omega^{d} \epsilon^2)$
To control the RKHS norm of $\rho(\xv)$, we may use the following well-known lemma.

\begin{lem}\label{lem:rkhs_fourier}
 Consider an RKHS $\Hc$ for functions on $\RR^d$, corresponding to a translation invariant kernel $k(\tau)$, and let $K(\bxi)$ be the $d$-dimensional Fourier transform of $k(\tau)$. Then for any $f\in\Hc$ with Fourier transform $\fhat(\bxi)$, we have
 \begin{equation} \label{eq:rkhs_norm}
 \|f\|_{\Hc}^2 = \int K(\bxi)^{-1} |\fhat(\bxi)|^2 d\bxi,
 \end{equation}
 and the Fourier transform of $f$ given by
 \begin{equation*}
 \fhat(\bxi)=(2\pi)^{-d/2}\int f(\xv)e^{-j\langle \bxi,\xv \rangle}d\xv
 \end{equation*}
\end{lem}
In our case, the Fourier transform of the SE kernel is 
\begin{equation}
 K(\bxi) = (2\pi l^2)^{d/2}e^{-2\pi^2 l^2\|\bxi\|^2}, \label{eq:se_fourier}
\end{equation}
and the Fourier transform of $\rho(\xv)$ can be interpreted as
\begin{align}
    \rhohat(\bxi) &=(2\pi)^{-d/2}\int_{\xv\in D} \sum_{i=1}^{M}\delta_i \psi_i(\xv)e^{-j\langle\bxi,\xv\rangle}d\xv \nonumber\\
    &=(2\pi)^{-d/2}\int_{\xv\in D} \sum_{i=1}^{M}\delta_i \psi(\xv-\sv_i)e^{-j\langle\bxi,\xv\rangle}d\xv \label{eq:rho_fourier_1}\\
    &=(2\pi)^{-d/2}\sum_{i=1}^{M}\delta_i \int_{\xv\in D}\psi(\xv-\sv_i)e^{-j\langle\bxi,\xv\rangle}d\xv \nonumber\\
    &= \frac{\omega^d \epsilon}{(2\pi)^{d/2}\zeta^d\phi(\bzero)} \sum_{i=1}^{M} \delta_i e^{-j\langle\bxi,\sv_i\rangle} \Phi\Big(\frac{\omega}{\zeta}\bxi\Big) \label{eq:rho_fourier}
\end{align}
In the equations above: $\sv_i$ in \eqref{eq:rho_fourier_1} is a $d$-dimensional shifting vector for function $\psi_i(\xv)$ with each dimension taking value from $\{\omega, 2\omega,\ldots, \lfloor\frac{1}{\omega}\rfloor\omega\}$; \eqref{eq:rho_fourier} uses the fact that the $d$-dimensional Fourier transform of $af(\frac{\xv-\cv}{b})$ is $e^{-j\langle\bxi, \cv\rangle}ab^d F(\bxi b)$.

Now, recalling the definition of the RKHS norm in \eqref{eq:rkhs_norm}, and combining \eqref{eq:se_fourier} and \eqref{eq:rho_fourier}, the RKHS norm of $\rho(\xv)$ in terms of the SE kernel is given by
\begin{align}
 \|\rho(\xv)\|_{\se}^2 &= \frac{\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\frac{\bxi\omega}{\zeta}\|_2\le 1} \Big|\sum_{i=1}^{M} \delta_i e^{-j\langle\bxi,\sv_i\rangle} \Phi\Big(\frac{\omega}{\zeta}\bxi\Big)\Big|^2 e^{2\pi^2 l^2 \|\bxi\|_2^2} d\bxi \nonumber\\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\frac{\bxi\omega}{\zeta}\|_2\le 1} \exp\Big(2\pi^2 l^2 \|\bxi\|_2^2 - \frac{2}{1-\|\frac{\omega\bxi}{\zeta}\|_2^2}\Big) d\bxi \nonumber\\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\bxi\|_2\le \frac{\zeta}{\omega}} \exp\big(2\pi^2 l^2 \|\bxi\|_2^2\big) d\bxi \nonumber \\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} V\Big(\frac{\zeta}{\omega}\Big) \exp\Big(\frac{2\pi^2 l^2 \zeta^2}{\omega^2}\Big) \label{eq:ball_volume_1} \\
 &\le \frac{ M^2 \omega^{d} \epsilon^2 \pi^{d/2}}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^d\phi(\bzero)^2\Gamma(\frac{d}{2}-1)} \exp\Big(\frac{2\pi^2 l^2 \zeta^2}{\omega^2}\Big) \label{eq:ball_volume_2} \\
 &=O\Big(M \epsilon^2 e^{2\pi^2 l^2 \zeta^2 M^{\frac{2}{d}}}\Big), \label{eq:rho_se_norm_upper_square}
\end{align}
where \eqref{eq:ball_volume_1} follows by upper bounding $\|\bxi\|_2^2\le \zeta^2\omega^{-2}$, and defining $V(\zeta\omega^{-1})$ to be the volume of a ball of radius $\zeta\omega^{-1}$ in $d$ dimensions: $V(\zeta\omega^{-1}) := \frac{\pi^{d/2}}{\Gamma(\frac{d}{2}-1)}(\zeta\omega^{-1})^d$, which immediately yeilds \eqref{eq:ball_volume_2}.  \eqref{eq:rho_se_norm_upper_square} again uses $M=\lfloor\frac{1}{\omega}\rfloor^d$.

Equating \eqref{eq:rho_se_norm_upper_square} with $B^2$ (so that $\|\rho(\xv)\|_{\se}\le B$), we have that 
\begin{equation}\label{eq:eps_M_se}
    \epsilon = \Theta\bigg(\frac{B}{\sqrt{M}e^{C_l' M^{\frac{2}{d}}}}\bigg), \quad C_l':=\pi^2 l^2 \zeta^2.
\end{equation}

For completion of the average-case proof, we will make use of a probabilistic result known as Khinchin’s inequality.
\begin{lem}\label{lem:khin}
    {\em (Khinchin’s Inequality)}
    Let $\delta_i$ be i.i.d distributed random variables with $\delta_i=\pm 1$ with equal probability, then 
    \begin{equation*}
        \EE\bigg[\Big|\sum_{i=1}^T c_i \delta_i\Big|\bigg] \ge \sqrt{\sum_{i=1}^{T} c_i^2}.
    \end{equation*}
\end{lem}
In our case, similar to the proof in Appendix \ref{app:mat_lower}, let $c_i=I_i$, and consider $T=\frac{M}{2}$, the expected error is then
\begin{equation*}
    \ravgse = \EE\bigg[\Big|\sum_{i=1}^{M/2} I_i \delta_i\Big|\bigg] \ge \sqrt{\sum_{i=1}^{M/2} I_i^2} = \Omega\Big(\frac{\epsilon}{\sqrt{M}}\Big) = \Omega\big(e^{-C_l T^{\frac{2}{d}}} T^{-1} \big),
\end{equation*}
with $C_l :=\pi^2 l^2 \zeta^2 2^{\frac{2}{d}}$.



% Since any function in SE RKHS can be written as an infinite series, recall the definition in \eqref{eq:se_rkhs}, any finite combination of those series also belongs to $\se$.  In this sense, for a multidimensional index $\balpha = [\alpha,\ldots,\alpha]$, we consider the following $g(\xv)\in\se$ 
% \begin{equation*}
%     g(\xv) = \frac{B}{M} \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2 }{2l^2}\Big), \quad \xv \succ \bzero\footnote{This is an element-wise inequality.}.
% \end{equation*}
% This function has an infinitely supported bump for $\xv\succ \bzero$, where the peak value $h^*$ depends on the value of $\alpha$.  In fact, we can take the first-order derivative of $g(\xv)$ along a single dimension, and get
% \begin{equation*}
%     \frac{g'(x) M}{B\mu_{\alpha}} = \alpha x^{\alpha-1} \exp\Big(-\frac{x^2 }{2l^2}\Big) - \frac{x^{\alpha+1}}{l^2} \exp\Big(-\frac{x^2 }{2l^2}\Big).
% \end{equation*}
% Letting $h'(x) = 0$, we see that $h^*$ is taken at $\bw'=[w',\ldots,w']$ with $w'= l\sqrt{\alpha}$, and 
% \begin{align*}
%     h^* &= h(\bw') \\
%     &= \frac{B}{M} \mu_{\balpha} \big(l\sqrt{\alpha}\big)^{d\alpha} e^{-\frac{d\alpha}{2}} \\
%     &= \frac{B}{M} .
% \end{align*}
% The function value at $\bzeta=C_{\zeta}\bzeta$ is
% \begin{equation*}
%     h(\bzeta) = \Big(\frac{C_{\zeta} l'\sqrt{\alpha}}{e^{C_{\zeta}^2/2}}\Big)^{d\alpha},
% \end{equation*}
% where for suitably chosen $l'$ and $C_{\zeta}$, $h(\bzeta)\to 0$.  We call $\zeta = C_{\zeta}l'$ the ``width'' of function $h$.  Note that we do not mean that the bump function is finitely supported, but doing so would allow us to focus on the most informative part of the function.  For $\xv \prec \bzero$, we make the function symmetric by letting $h(\xv)=h(-\xv)$, so that the function has two bumps in $\RR^d$, within the region $[-\zeta,\zeta]^d$.

% For our domain $D=[0,1]^d$, we rescale $h(\xv)$ into $g(\xv)\in \se$ and truncate it by $D$, so that the width becomes $w\in(0,1)$ and height becomes $\epsilon$:
% \begin{equation}\label{eq:se_g_1}
%     g(\xv) = \frac{\epsilon}{h^*} h\Big(\frac{\xv\zeta}{w}\Big) = \frac{\epsilon \zeta^{d\alpha}}{h^* w^{d\alpha}}  \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big), \quad l:= \frac{l' w}{\zeta}.
% \end{equation}
% We can construct $M=\lfloor \frac{1}{2w} \rfloor ^d$ of such $g(\xv)$ in the domain $D=[0,1]^d$, by shifting the dual-bump of $g(\xv)$ (within $[-w,w]^d$) into these $M$ grids, denoted by $g_i(\xv), i\in\{1,\ldots,M\}$.  The function $f$ we are interested is now of the form $f(\xv) = \sum_{i=1}^{M} \delta_i g_i(\xv)$, where $\delta_i\in\{+1,-1\}$ with equiprobability.  The RKHS norm of $f$ is given by the definition in \eqref{eq:se_rkhs},
% \begin{equation*}
%     \|f\|_{\se} \le M\|g\|_{\se} = \frac{\epsilon \zeta^{d\alpha}}{h^* w^{d\alpha+d} 2^d \mu_{\balpha}}.
% \end{equation*}
% Thus, $\|f\|_{\se}$ is bounded by $B$ by a choice of $\epsilon$ satisfying
% \begin{align}
%     \epsilon &= \frac{B h^* w^{d\alpha +d} 2^d\mu_{\balpha}}{\zeta^{d\alpha}} 
%     % & = \Theta (\frac{B (l'\sqrt{\alpha})^{d\alpha} w^{d(\alpha+1)} \sqrt{e}^{d\alpha}}{(\sqrt{e}^{d\alpha}) (l\sqrt) } ))
% \end{align}


% Substituting this back into \eqref{eq:se_g_1}, $g(\xv)$ can be simplified into
% \begin{equation}\label{eq:se_g}
%     g(\xv)=B (2w)^{d} \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big).
% \end{equation}

% From \eqref{eq:se_g}, we see that the integration of $g(\xv)$ in $[0,w]^d$, is at least 
% \begin{equation*}
%     B w^{d} 2^d\mu_{\balpha}e^{-\frac{1}{2l^2}} \int_{\xv\in[0,w]^d} \xv^{\balpha} d\xv = \frac{B w^{d(\alpha+1)} 2^d\mu_{\balpha}e^{-\frac{1}{2l^2}}}{(\alpha+1)^d},
% \end{equation*}
% since $\int_{\xv\in[0,w]^d} \xv^{\balpha} d\xv = \frac{w^{d\alpha}}{(\alpha+1)^d}$

% Let 
% \begin{equation*}
%     I_i = \int_{\xv\in D_i} f(\xv) d\xv =  \sum_{j=1}^M \delta_i \int_{\xv\in D_i} g_j(\xv) d\xv
% \end{equation*}
% be the integral of $f$ in region $i$.  Suppose $\delta_i=1$ at region $i$, therefore, the lower bound for $I_i$ is
% \begin{align*}
%     I_i &\ge \int_{\xv\in D_i} g_i(\xv) d\xv - \sum_{j\neq i}^M \int_{\xv\in D_i} g_j(\xv) d\xv \\
%     &=  \int_{\xv\in D_i} g_i(\xv) d\xv - \int_{\xv\notin D_i} g_i(\xv) d\xv \\
%     &= 2\int_{\xv\in [0,w]^d} g(\xv) d\xv - \int_{\xv\in [w,1]^d} g(\xv) d\xv \\
%     &\ge \Omega\big(w^d g^*) - B w^d \mu_{\balpha}  \int_{\xv\in [w,1]^d} \xv^{\balpha} d\xv  \\
%     &= \Omega\big(w^{3d} \mu_{\balpha}) - B w^d \mu_{\balpha} \frac{1-w^{d\alpha}}{(\alpha+1)^d} \\
%     &\approx \Omega\big(w^{3d} \mu_{\balpha}),
% \end{align*}
% where we have used the fact that $g(\xv)$ decays to $0$ after $[w,\ldots,w]$, this can also be seen by considering large $\alpha$ and $d$ in the second-last inequality.

% Finally, we are able to use the same technique as we have done in Appendix \ref{app:mat_lower}, by considering $T=\Theta(M)$ and $\alpha=T^{\frac{1}{d}}$.  Therefore, we obtain
% \begin{equation*}
%     \rwstse = \Omega(M I_i) = \Omega(T^{-\frac{1}{2}} \alpha^{-d\alpha/2}) = \Omega(T^{-\frac{1}{2}T^{\frac{1}{d}}-\frac{1}{2}}).
% \end{equation*}


\section{Proof for Theorem \ref{thm:wst_se_nosig} (Worst-case Noiseless SE Upper Bound)} \label{app:wst_se_nosig}

\subsection{Proof for Gauss-Hermite Rules}
Consider the $1$-D case, let $\tau_{\alpha}(x)=x^{\alpha} \exp(-\frac{x^2}{2l^2})$, the integral of $\tau_{\alpha}(x)$ is then defined in terms of the integral of the polynomial $x^{\alpha}$ with Gaussian weighting function $\exp(-\frac{x^2}{2l^2})$.  A well-known solution to such integrand is the Gauss-Hermite rule for its exactness when solving polynomials, see for example \cite{Bar78}.  Such case also holds for multivariate integration if we make use of tensor product based Gauss-Hermite rules.  Formally, for dimension $i$, the Gauss-Hermite rule is exact for $I(x^{\balpha_i}\exp(-\frac{x^2}{2l^2}))$ with $\balpha_i/2$ query points (for derivation simplicity, we will use $\balpha_i$ instead of $\balpha_i/2$ since we are accounting for the upper bound and it will only affect the final results up to a constant factor).  By the arithmetic-geometric inequality, for any tensor product based Gauss-Hermite rule with a budget of $T:=\prod_{i=1}^{d}\balpha_i$ queries, we must have $|\balpha|\ge d T^{1/d}:=N$.  With this in mind, for $f\in\se$, the worst case error can be bounded in the following sense:
\begin{align}
    |I(f) - \Ihat(f)| &= \Big|\int_{\xv\in D} \sum_{\balpha\in\NNd}\theta_{\balpha}e_{\balpha}(\xv) d\xv - \Ihat\Big| \nonumber\\
    &\le \Big| \sum_{|\balpha|=N}^{\infty} \int_{\xv\in D}\theta_{\balpha}e_{\balpha}(\xv) d\xv \Big| \label{eq:se_worst_align_1}\\
    &\le \sup_{\xv\in D} \Big| \sum_{|\balpha|=N}^{\infty}  \theta_{\balpha}e_{\balpha}(\xv) d\xv \Big| \label{eq:se_worst_align_2}\\
    &\le \sup_{\xv\in D} \sqrt{\sum_{|\balpha|=N}^{\infty} \theta_{\balpha}^2} \cdot \sqrt{\sum_{|\balpha|=N}^{\infty} e_{\balpha}^2(\xv)} \label{eq:se_worst_align_3}\\
    &\le \sup_{\xv\in D} B \sqrt{\sum_{|\balpha|=N}^{\infty} e_{\balpha}^2(\xv)} \label{eq:se_worst_align_4}\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{|\balpha|=N}^{\infty} \frac{1}{l^{2|\balpha|}\balpha !} \xv^{2\balpha} \exp\big(-\frac{\|\xv\|^2}{l^2}\big)} \nonumber\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{k=N}^{\infty} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \sum_{|\balpha|=k} \frac{1}{l^{2k}\balpha !} \xv^{2\balpha} } \nonumber\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{k=N}^{\infty} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \frac{1}{k!} \sum_{|\balpha|=k} \frac{k!}{\balpha_1 !\cdots \balpha_d !}\big(\frac{\xv_1^2}{l^2}\big)^{\balpha_1}\cdots\big(\frac{\xv_d^2}{l^2}\big)^{\balpha_d} }  \nonumber \\
    &= \sup_{\xv\in D} B \sqrt{\exp\big(-\frac{\|\xv\|^2}{l^2}\big)\sum_{k=N}^{\infty}  \frac{1}{k!} \big(\frac{\xv_1^2+\ldots+\xv_d^2}{l^2}\big)^k} \label{eq:se_worst_align_5}\\
    &\le \sup_{\xv\in D} B \sqrt{\exp\big(-\frac{\|\xv\|^2}{l^2}\big) \frac{\|\xv\|^{2N}}{l^{2N}N!}\exp\big(\frac{\|\xv\|^2}{l^2}\big)} \label{eq:se_worst_align_6}\\
    &\le \sup_{\xv\in D} B \sqrt{\big(\frac{ed}{l^2 N}\big)^N} \label{eq:se_worst_align_7}
    % &= O\Big(\big(\frac{e}{N}\big)^{\frac{N}{2}}\Big). \label{eq:se_error_worst}
\end{align}
In the above equations:
\begin{itemize}
    \item \eqref{eq:se_worst_align_1} is since tensor product based Gauss-Hermite rules are exact for all $\theta_{\balpha}e_{\balpha}$ with $|\balpha|\le N$, thus the error is upper bounded by the residual;
    \item \eqref{eq:se_worst_align_2} is since $D=[0,1]^d$ and \eqref{eq:se_worst_align_3} follows from Holder's inequality with the counting measure;
    \item \eqref{eq:se_worst_align_4} is because we are only considering RKHS functions with smoothness $B$, i.e., $\sum_{|\balpha|=N}^{\infty}\theta_{\balpha}^2 < \sum_{\balpha\in\NNd}\theta_{\balpha}^2 = B^2$;
    \item \eqref{eq:se_worst_align_5} follows since the multinomial theorem;
    \item \eqref{eq:se_worst_align_6} uses the fact that $\sum_{n=N}^{\infty}\frac{x^n}{n!}\le \frac{x^N}{N!}e^{y}$, where $0<y\le x$;
    \item \eqref{eq:se_worst_align_7} is simplified due to Stirling's formula, $n!\sim\big(\frac{n}{e}\big)^n$, and $\|\xv\|^2\le d$
\end{itemize}

Recalling that $N=dT^{\frac{1}{d}}$, we obtain
\begin{equation*}
    \rwstse \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}}, \quad C_{gh} := B\Big(\frac{e}{l^2}\Big)^{\frac{d}{2}T^{\frac{1}{d}}}
\end{equation*}

\subsection{Proof for Regular Linear Algorithms}
Since normal linear algorithms cannot guarantee that the first $N:=d T^{\frac{1}{d}}$ series to be exactly solved like Gauss-Hermite rules, the error incurred by such algorithms are two-folds: The error for approximating the first $N$ series and the residual.  In this case, we consider $f\in\se$ in the following form,
\begin{equation*}
    f(\xv) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv^{\balpha},
\end{equation*}
with RKHS norm
\begin{equation} \label{eq:se_f_rkhs}
    \|f\|_{\se}^2 = \sum_{|\balpha|=0}^{N}\frac{\theta_{\balpha}^2}{\mu_{\balpha}^2} \le B^2.
\end{equation}
Let the quadrature rule be
\begin{equation*}
    \Ihat(f) = \sum_{t=1}^{T} w_t f(\xv_t),
\end{equation*}
and regularized by $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$.  Being in the worst-case setting, the maximum $\balpha^*$ that satisfies $|\balpha^*|=N$ is taken at $\balpha^*=[\frac{N}{d},\ldots,\frac{N}{d}]$.  Thus, we derive
\begin{align}
    |I(f) - \Ihat(f)| &= \bigg|\int_D \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv^{\balpha} d\xv - \sum_{t=1}^{T} w_t \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv_t^{\balpha} \bigg| \nonumber\\
    &\le \bigg| \sum_{|\balpha|=0}^{N} \theta_{\balpha} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv - \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)\Big) \bigg| \nonumber\\
    &\le \sqrt{\sum_{|\balpha|=0}^{N} \theta_{\balpha}^2} \sqrt{\sum_{|\balpha|=0}^{N} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv - \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)\Big)^2}  \label{eq:se_linear_int_upper_1} \\
    &\le B\mu_{\balpha^*} \sqrt{\sum_{|\balpha|=0}^{N} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \Big)^2 + \sum_{|\balpha|=0}^{N} \Big( \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \Big)^2} \label{eq:se_linear_int_upper_2}\\
    &\le B\sqrt{\Big(\frac{1}{l^{\frac{2N}{d}} (\frac{N}{d})!}\Big)^d} \sqrt{\sum_{|\balpha|=0}^{N} \prod_{i=1}^{d} \frac{1}{(\balpha_i+1)^2} + \sum_{|\balpha|=0}^{N} \sum_{t=1}^{T}w_t^2 \sum_{t=1}^{T} \xv_t^{2\balpha}\exp\big(-\frac{\|\xv_t\|^2}{l^2}\big) } \label{eq:se_linear_int_upper_3}\\
    &\le B\sqrt{\big(\frac{ed}{l^2 N}\big)^N} \sqrt{\Big(\sum_{k=1}^{N+1}\frac{1}{k^2}\Big)^d  + \Big(\frac{N}{d}\Big)^d o\Big(\frac{1}{T}\Big) }, \label{eq:se_linear_int_upper_4}
\end{align}
where 
\begin{itemize}
    \item \eqref{eq:se_linear_int_upper_1} follows by Cauchy-Schwarz inequality, and consequently, \eqref{eq:se_linear_int_upper_2} uses \eqref{eq:se_f_rkhs} and the fact that $\mu_{\balpha}$ is a decreasing sequence;
    \item The first square root term in \eqref{eq:se_linear_int_upper_3} substitutes the value of $\mu_{\balpha^*}$ for $\balpha^*=[\frac{N}{d},\ldots,\frac{N}{d}]$;  The first term in the second square root of \eqref{eq:se_linear_int_upper_3} is since $D=[0,1]^d$, so that $\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \le \int_D \xv^{\balpha} d\xv \le \prod_{i=1}^{d} \frac{1}{(\balpha_i+1)^2}$;  The second term in the second square root of \eqref{eq:se_linear_int_upper_3} again uses Cauchy-Schwarz inequality;
    \item \eqref{eq:se_linear_int_upper_4} is simply since $\max_{\xv\in D} \xv^{2\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \le 1$ and $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$.
\end{itemize}

Recalling $N=dT^{\frac{1}{d}}$ in \eqref{eq:se_linear_int_upper_4}, we can continue to wirte:
\begin{equation*}\label{eq:se_linear_int_upper}
    |I(f) - \Ihat(f)| \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}} \sqrt{\big(\frac{\pi}{6}\big)^d + o(1)} = C_l C_{gh} T^{-\frac{1}{2}T^{\frac{1}{d}}}, \quad C_l:=\sqrt{\big(\frac{\pi}{6}\big)^d + o(1)},
\end{equation*}
where we have used the fact that $\sum_{n=1}^{\infty}\frac{1}{n^2}=\frac{\pi}{6}$.  Finally, the proof is done for any $f\in\se$ with $\|f\|_{\se}\le B$, by amounting the residual error proved in the previous section.

% Denoting the worst case error to be $\epsilon$ and re-arranging \eqref{eq:se_error_worst} gives us that
% \begin{equation*}
%     N = O\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big),
% \end{equation*}
% and recalling $N=dT^{\frac{1}{d}}$, we obtain
% \begin{equation*}
%     T = O\bigg(\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big)^d\bigg). \label{eq:se_T_worst}
% \end{equation*}

% \section{Proof of SE Lower Bound}
% Following the idea of \cite{Kuo17}, given $T=N-1$ arbitrary inputs $\{x_1,\ldots,x_T\}$ from $D=[0,1]$, we can choose real numbers $\{\theta_1,\ldots,\theta_N\}$, such that 
% \begin{equation}
%     \sum_{m=1}^{N}\theta_m x_t^m = 0, \quad \forall t=1,2,\ldots,N-1. \label{eq:se_lower_linear}
% \end{equation}
%   Since the linear system has more unknowns ($N$) than the number of conditions ($N-1$), a non-trivial solution of \eqref{eq:se_lower_linear} certainly exists.  Thus, by re-scaling, there exists a solution such that
% \begin{equation}
%     \max_{1\le i\le N} |\theta_i|=1=\theta_k, \quad 1\le k\le N. \label{eq:theta_condition}
% \end{equation}
% We now define a function in the form:
% \begin{equation}
%     f(x) = \exp(-\frac{x^2}{2l^2}) \sum_{m=1}^{N}\theta_m x^m, \label{eq:se_lower_f}
% \end{equation}
% so that $f\in \se$, and most importantly, $f(x_t)=0$ for all $i=1,\ldots,N-1$, thus any quadrature rule based on linear combinations of these $N-1$ function values will return $0$.  Hence, the error of integrating $f(x)$ is equivalent to
% \begin{align}
%     \Big|\int_D f(x)dx -0 \Big| &= \Big|\int_D \exp(-\frac{x^2}{2l^2}) \sum_{m=1}^{N}\theta_m x^m dx \Big| \nonumber \\
%     &= \Big|\sum_{m=1}^{N} \theta_m \int_0^1 \exp(-\frac{x^2}{2l^2}) x^m dx \Big|. \label{eq:se_int_lower}
% \end{align}
% We argue that \eqref{eq:se_int_lower} cannot be $0$, since together with \eqref{eq:se_lower_linear}, we now have a linear system with same number of conditions and unknowns, thus $\theta$ is either unique or not existing.  This contradicts our assumption on the inputs and $\theta$, given that $\theta$ satisfies \eqref{eq:theta_condition}, we can perturb the inputs so that \eqref{eq:theta_condition} is no longer satisfied.  Therefore, $\big|\int_D f(x)dx\big|\in(0,\sum_{m=1}^N \frac{1}{m+1}]$, which can be regarded as a constant.

% an equivalent expression of $\rwstmat$ is 
% \begin{equation}
%     \sup_{p\in\Pc, f\in\Hc}\frac{|I-\Ihat|}{\|f\|_{\se}} = \sup_{p\in\Pc, f\in\Hc}\frac{1}{\|f\|_{\se}}. \label{eq:worst_error_equiv}
% \end{equation}

% Also, for $f$ defined in \eqref{eq:se_lower_f}, its RKHS norm is at most
% \begin{align}
%     \|f\|_{\se} &\le \sum_{m=1}^{N} |\theta_m| \|\tau_k(x)\tau_m(x)\|_{\se} \nonumber\\
%     &\le \sum_{m=1}^{N}  \|\tau_k(x)\tau_m(x)\|_{\se} \nonumber\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} \tau_m(x) \tau_k(x) \tau_j(x) dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand1}\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} x^{m+k} \exp(-\frac{3x^2}{4l^2}) x^{j} \exp(-\frac{3x^2}{4l^2})dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand2}\\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} \tau'_{m+k}(x) \tau'_j(x) dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand3}\\
%     &= \sum_{m=1}^N \frac{1}{\sqrt{\mu_{m+k}}} \label{eq:se_rkhs_expand4}\\
%     &\le \frac{N}{\sqrt{\mu_{2N}}}. \label{eq:se_rkhs_expand}
% \end{align}
% In the above equations:
% \begin{itemize}
%     \item \eqref{eq:se_rkhs_expand1} follows from the definition of RKHS norm, $\|f\|_{\se}^2 = \sum_{i\ge 0} \frac{\langle f, \tau_{i}\rangle_{L^2}^2}{\mu_i}$, see for example;
%     \item \eqref{eq:se_rkhs_expand2} is by expanding each $\tau(x)$ function and re-arranging;
%     \item $\tau'_{\alpha}(x) = x^{\alpha}\exp(-\frac{3x^2}{4l^2})$ in \eqref{eq:se_rkhs_expand3} can be regarded as the eigenfunction of the modified SE kernel $k'(x,x')=\exp(-\frac{3|x-x'|^2}{4l^2})$.  Therefore, $\langle \tau'_i, \tau'_j\rangle_{L^2} = 1$ for $i=j$, and $0$ otherwise, which yields \eqref{eq:se_rkhs_expand4};
%     \item \eqref{eq:se_rkhs_expand} is since $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence, i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{2N}$.
% \end{itemize}

% Moreover, recall the definition of the SE RKHS norm in \eqref{eq:se_rkhs}, the RKHS norm of $f$ defined in \eqref{eq:se_lower_f} can be bounded by
% \begin{align}
%     \|f\|_{\se}^2 = \sum_{m=1}^N \frac{\theta_m^2}{\mu_m} \le \frac{N}{\mu_N}, \label{eq:se_f_rkhs}
% \end{align}
% since $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence (i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{N}$).

% Combining \eqref{eq:se_f_rkhs} with \eqref{eq:se_int_lower}, the worst case error is at least 
% \begin{equation*}
%     \frac{\Big|\int_D f(x)dx - 0 \Big|}{\|f\|_{\se}} = \Omega\Big(\sqrt{\frac{\mu_{N}}{N}}\Big) = \Omega\Big(\frac{1}{\sqrt{N} l^{N} \sqrt{N!}}\Big) = \Omega\Big(\frac{1}{\sqrt{N}}\big(\frac{e}{N}\big)^{\frac{N}{2}} \Big).
% \end{equation*}
% Rearranging yields that
% \begin{equation*}
%     T=N-1=\Omega\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big).
% \end{equation*}


% \begin{lem} \label{lem:sig_interp_norm_upper}
%     The RKHS norm and the sampling norm regarding the kernel interpolant of the the noise $\varepsilon_1$, $\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1$, is upper bounded by
%     \begin{align}
%         \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se} &\le \frac{\|\varepsilon_1\| \sqrt{\lambda_{\min}(\Kv_T)}}{\lambda_{\min}(\Kv_T) + \lambda} , \label{eq:sig_interp_upper} \\
%         \big\|\big(\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \big)_X \big\|_{\infty} &\le \sqrt{T}\kappa C_F
%     \end{align}
%     where $\lambda_{\min}(\Kv_T)$ denotes the minimum eigenvalue of the kernel interpolant matrix $\Kv_T$, $\kappa = \sup_{\xv,\yv} \kse(\xv,\yv)$, and $C_F$ is the constant that guarantees $\|A\|_F \le C_F \|A\|_2 $.
% \end{lem}

% \begin{proof}
%     The proof simply follows from the reproducing property,
%     \begin{align}
%         \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se}^2 &= \varepsilon_1^T (\Kv_T^T +\lambda \Iv)^{-1} \Kv_T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \nonumber\\
%         &\le \|\varepsilon_1\|^2 \|(\Kv_T^T +\lambda \Iv)^{-1} \Kv_T (\Kv_T +\lambda \Iv)^{-1} \|_2 \nonumber\\
%         &\le \|\varepsilon_1\|^2  \|(\Kv_T +\lambda \Iv)^{-1}\|_2^2 \| \Kv_T\|_2 \label{eq:sig_interp_upper_1}\\
%         &\le \|\varepsilon_1\|^2 \frac{\lambda_{\min}(\Kv_T)}{\big( \lambda_{\min}(\Kv_T) + \lambda \big)^2} \label{eq:sig_interp_upper_2} ,
%     \end{align}
%     where $\|A\|_2$ for a matrix $A$ denotes the spectral norm, $\sup_{\xv\neq \bzero} \frac{\xv^T A \xv}{\|\xv\|^2}$; \eqref{eq:sig_interp_upper_1} uses the fact that $\|AB\|_2\le \|A\|_2\|B\|_2$ and $\Kv_T$ is symmetric; \eqref{eq:sig_interp_upper_2} is by the Rayleigh-Ritz theorem \cite{Hor12}.

%     \begin{align}
%         \big\|\big(\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \big)_X \big\|_{\infty}^2 &\le \sup_{\xv\in D}   \Big(\sum_{i=1}^T  \kse(\xv_t,\xv_i)  (\Kv_T +\lambda \Iv)^{-1}_{i,j} \sum_{j=1}^T \epsilon_j \Big)^2\\
%         &\le \Big(\sup_{\xv\in D, \xv_t\in X} \sum_{i=1}^T  \kse(\xv,\xv_i)^2 \Big)\sum_{i=1}^T\sum_{j=1}^T \big((\Kv_T +\lambda \Iv)^{-1}_{i,j}\big)^2  \sum_{j=1}^T \epsilon_j^2 \\
%         &\le T\kappa^2 \cdot \| (\Kv_T +\lambda \Iv)^{-1}\|_F^2 \cdot \|\varepsilon_1\|^2 \\
%         &\le T\kappa^2 C_F^2 \big( \lambda_{\min}(\Kv_T) + \lambda \big)^{-2} \|\varepsilon_1\|^2,
%     \end{align}
% \end{proof}

% Using Theorem \ref{thm:se_sampling_ineq}, and by triangle inequality, we have
% \begin{align}
%     \|f-\mu_T\|_{\se} \le \|f-\mu_T\|_{\se} + \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se}
% \end{align}

% Using Theorem \ref{thm:se_sampling_ineq}, for $f\in \se$, we derive
% \begin{align}
%     \|f - \mu_T\|_{L^2} &\le \exp\Big(\frac{C\log h_X}{h_X}\Big) \|f-\mu_T\|_{\se} + \exp\Big(\frac{\Ctil}{h_X}\Big) \|(f-\mu_T)_{X}\| \\
%     &\le \exp\Big(\frac{C\log h_X}{h_X}\Big) (\|f\|_{\se} + \|\mu_T\|_{\se}) +  \exp\Big(\frac{\Ctil}{h_X}\Big) \|(f-\mu_T)_{X}\| \\
%     &= O\bigg(\exp\Big(\frac{C\log h_X}{h_X}\Big)(\lambda^{-1}\|\varepsilon_1\| + B) + \exp\Big(\frac{\Ctil}{h_X}\Big) (\|\varepsilon_1\| + \lambda B) \bigg) \\
%     &= O\bigg( \exp\Big(\frac{C\log h_X}{h_X}\Big) + \exp\Big(\frac{\Ctil}{h_X}\Big)\lambda + \Big(\exp\Big(\frac{C\log h_X}{h_X}\Big)\lambda^{-1} + \exp\Big(\frac{\Ctil}{h_X}\Big)\Big) \|\varepsilon_1\|  \bigg)
% \end{align}


% In this section, we show how to obtain the noisy $L^2$ upper bound based on several properties in \cite{Bac17}, which are summarized in the following two lemmas.
% \begin{lem} \label{lem:int_sig_nosig}
%     {\em (Quadrature Noisy-noiseless relationship)}
%     Let $f$ be any function in $\se$, then for any algorithm that uses the linear combinations, $\Ihatsig =\sum_{t=1}^{T} \beta_t (f(\xv_t)+\epsilon_t)$ or $\Ihat =\sum_{t=1}^{T} \beta_t f(\xv_t)$, respectively of noisy or noiseless function evaluations, then we have the following relationship between the averaged integration error and the noiseless integration error:
%     \begin{equation}
%         \sup_{f\in \se} \EE[|I-\Ihatsig|^2] \le \sup_{f\in \se}2|I-\Ihat|^2 + 2\sum_{t=1}^{T}\beta_t^2 \EE[\|\varepsilon_1\|^2]. \label{eq:noisy_int_eq}
%     \end{equation}
% \end{lem}
% \begin{proof}
%     We note that $\EE[\cdot]$ in this section explicitly denotes the expectation taking with respect to $\varepsilon_1=\{\epsilon_1,\ldots,\epsilon_{T}\}$.  Then, we can use Cauchy-Schwarz inequality to obtain:
%     \begin{align*}
%         \EE\bigg[\Big|I-\sum_{t=1}^{T} \beta_t (f(\xv_t)+\epsilon_t)\Big|^2\bigg] &\le 2\Big|I-\sum_{t=1}^{T}\beta_t f(\xv_t) \Big|^2 + 2 \EE\bigg[\Big|\sum_{t=1}^{T} \beta_t \epsilon_t\Big|^2\bigg] \\
%         &\le 2|I-\Ihat|^2 +  2\EE\bigg[\sum_{t=1}^{T}\beta_t^2  \sum_{t=1}^{T}\epsilon_t^2\bigg]\\
%         &=  2|I-\Ihat|^2 + 2\sum_{t=1}^{T}\beta_t^2 \EE[\|\varepsilon_1\|^2].
%     \end{align*}
%     By taking the supreme over $f$ on both sides gives the proof.
% \end{proof}

% Before proceeding, we introduce a couple of lemmas in matrix analysis to help proving our upper bound.
% \begin{lem} \label{lem:mat_inv_diff}
%     {\em (\citep[Sec 5.8]{Hor12})}
%     Let $\|\cdot\|$ be a given matrix norm, for two nonsingular matrices $A$ and $B$, denote $\Delta = A-B$.  Given the assumption that $\|\Delta A^{-1}\|\le 1$, we have,
%     \begin{equation}
%         \|A^{-1} - B^{-1}\| \le \frac{\|A^{-1}\|^2\|\Delta\|}{1- \|A^{-1}\Delta\|}.
%     \end{equation}
% \end{lem}

% \begin{lem} \label{lem:mat_norm_bound}
%     {\em (\citep[Sec 5.8]{Hor12})}
%     Let $\|\cdot\|$ be a given matrix norm, for two real and symmetric matrices $A$ and $B$, we have,
%     \begin{equation}
%         \|(A+B)^{-1}\| \le \|A^{-1}\|.
%     \end{equation}
% \end{lem}

% Let $\phi(\xv)=\exp(-\frac{\|\xv\|^2}{2l^2})[\mu_{\bzero}\xv^{\bzero},\ldots,\mu_{\balpha}\xv^{\balpha},\ldots]^T$ be the infinite dimensional feature mapping of the SE kernel, which can be expanded as:
%  \begin{equation}
%         \exp\Big(-\frac{\|\xv-\yv\|^2}{2l^2}\Big) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\yv\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha}^2 \xv^{\balpha}\yv^{\balpha} = \phi(\xv)^T\phi(\yv). \label{eq:kse_expand}
%     \end{equation}
% Then, we have the following Theorem.
% \begin{thm} \label{thm:se_l2_upper_nosig}
%     {\em (Noisy $L^2$ Upper bound -- SE kernel)}
%     Let $f(\xv) = \int_D g(\yv)\kse(\xv,\yv)d\yv $ be any function lies in $\se$, where $g(\xv)\in L^2(D)$ and $\|g\|_{L^2}\le 1$, so that the RKHS norm of $f$ is less than $1$.  Denote 
%     $$
%         \fhat(\xv)= \kv_T(\xv)^T \Kv_T^{-1} \yv_T
%     $$ 
%     as the noiseless estimation of $f$, and 
%     $$
%         \fhatsig(\xv)= \kv_T(\xv)^T \Kv_T^{-1} (\yv_T+\varepsilon_1)
%     $$
%     as the noisy estimation of $f$.  Then, the error of estimating the noisy $L^2$-distance on $[0,1]^d$ is upper bounded by:
%     \begin{equation}
%         \EE\big[ \|f-\fhatsig\|_{L^2} \big] \le \|f-\fhat\|_{L^2} + O\Big(T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \label{eq:se_l2_upper_sig}
%     \end{equation}
% \end{thm}

% \begin{proof}
    % Consider the following expansion:
    % \begin{equation}
    %     \exp\big(\frac{\|\xv-\xv_t\|^2}{2l^2}\big) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha}^2 \xv_t^{\balpha}\xv^{\balpha}.
    % \end{equation}
    % We first observe that $f(\xv_t)=\psi(\xv_t)^T (\sqrt{\mu}\theta)$:
    % \begin{equation*}
    %     \psi(\xv_t)^T (\sqrt{\mu}\theta) = \exp(-\frac{\|\xv_t\|^2}{2l^2})\sum_{\balpha\in\NNd}\theta_{\balpha}\mu_{\balpha}\xv_t^{\alpha} = f(\xv_t).
    % \end{equation*}
    % By denoting $\bthetahat := \Phi^{-1} \yv_T$, we can expand $\fhat$ as
    % \begin{equation*}
    %     \fhat(\xv) = \exp(-\frac{\|\xv\|^2}{2l^2})\sum_{\balpha\in\NNd} \bthetahat_{\balpha}\mu_{\balpha} \xv^{\balpha}.
    % \end{equation*}
    % Then, the $L^2$ distance between $f$ and $\fhat$ is
    % \begin{align*}
    %     \|f-\fhat\|_{L^2}^2 &= \int_D \Big( \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} (\theta_{\balpha} -  \thetahat_{\balpha}) \Big)^2 d\xv \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\theta_{\balpha} - \thetahat_{\balpha}) (\theta_{\bgamma} - \thetahat_{\bgamma}) \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv.
    % \end{align*}
    % \begin{align}
    %     \fhat(\xv) &= \sum_{t=1}^{T} \beta_t \psi(\xv_t)^T \psi(\xv)\\
    %     &= \sum_{t=1}^{T/2}\beta_t \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha} \xv_t^{\balpha}\xv^{\balpha} \nonumber\\
    %     &= \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} \sum_{t=1}^{T/2} \beta_t \xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)
    % \end{align}
    % We can expand $\fhat$ as:
    % \begin{align}
    %     \fhat(\xv) &=  \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{t=1}^{T/2}\beta_t  \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \theta_{\balpha} \mu_{\balpha} \xv_t^{\balpha} \nonumber \\
    %     &= \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \sum_{t=1}^{T/2} \beta_t \xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)
    % \end{align}
    % Denoting $\Upsilon_{\balpha}:= \sum_{t=1}^{T/2}\beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)$, the $L^2$ distance between $f$ and $\fhat$ is then
    % \begin{align}
    %     \|f-\fhat\|_{L^2}^2 &= \int_D \bigg( \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} \Big(\theta_{\balpha} - \sum_{t=1}^{T/2} \beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \Big)  \bigg)^2 d\xv \nonumber\\
    %     &= \int_D \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \Big(\sum_{\balpha\in\NNd} \mu_{\balpha} \xv^{\balpha} (\theta_{\balpha} - \Upsilon_{\balpha}) \Big)^2 d\xv \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\theta_{\balpha} - \Upsilon_{\balpha}) (\theta_{\bgamma} - \Upsilon_{\bgamma}) \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv. \label{eq:se_l2_expand}
    % \end{align}
    % Denoting $\Lambda_{\balpha} := \int_D \xv^{\alpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv$, the error of estimating the integration is
    % Denoting $\Upsilon_{\balpha} := \int_D \xv^{\alpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv$, and $\Upsilonhat_{\balpha} := \sum_{t=1}^{T/2}\beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)$, the error of integration can be calculated in the similar fashion:
    % \begin{align}
    %     |I - \Ihat|^2 &= \bigg( \int_D \exp(-\frac{\|\xv\|^2}{2l^2})\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv^{\balpha} d\xv -  \sum_{t=1}^{T/2}\beta_t \exp(-\frac{\|\xv_t\|^2}{2l^2})\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv_t^{\balpha} \bigg)^2 \nonumber\\
    %     &= \Big(\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} (\Upsilon_{\balpha} - \Upsilonhat_{\bgamma} )  \Big)^2 \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\Upsilon_{\balpha} - \Upsilonhat_{\balpha}) (\Upsilon_{\bgamma} - \Upsilonhat_{\bgamma}) \theta_{\balpha}\theta_{\gamma}. \label{eq:se_int_expand}
    % \end{align}
    % Now, by setting $\theta_{\balpha} = \Lambda_{\balpha}$, it can be seen that the only difference between \eqref{eq:se_l2_expand} and \eqref{eq:se_int_expand} is $\Lambda_{\balpha}\Lambda_{\bgamma}$ v.s. $\int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv$.  We can further compare these two by noting that $D=[0,1]^d$:
    % \begin{equation*}
    %     \int_D \xv^{\balpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \le \int_D\xv^{\balpha} d\xv = \prod_{i=1}^d \frac{1}{\balpha_i+1}.
    % \end{equation*}
    % Hence we have
    % \begin{equation}
    %     \Lambda_{\balpha}\Lambda_{\bgamma} \le \prod_{i=1}^d \frac{1}{(\balpha_i+1)(\bgamma_i+1)} \le \prod_{i=1}^d \frac{1}{\balpha_i+\bgamma_i+1}, \label{eq:l2_residual}
    % \end{equation}
    % and
    % \begin{equation}
    %     \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv \le \prod_{i=1}^d \frac{1}{\balpha_i+\bgamma_i+1}. \label{eq:int_residual}
    % \end{equation}
    % We have now proved that the supremacy between $\|f-\fhat\|_{L^2}^2$ and $|I - \Ihat|^2$ are equivalent, the rest of the proof is to show that setting $\theta_{\balpha} = \Lambda_{\balpha}$ dose not violate the smoothness of the function:
    % \begin{equation*}
    %     \sum_{\balpha\in\NNd} \theta_{\balpha}^2 \le \sum_{\balpha\in\NNd} \prod_{i=1}^d \frac{1}{(\balpha_i+1)^2} = \prod_{i=1}^d \sum_{\balpha_i \ge 2} \frac{1}{\balpha_i^2} \le \Big(\frac{\pi^2}{6}-1\Big)^d := B,
    % \end{equation*}
    % where we have used the fact that $\sum_{n\ge 1} \frac{1}{n^2} = \frac{\pi^2}{6}$.
    % Let 
    % $$
    %     \Phi = [\phi(\xv_1),\ldots,\phi(\xv_T)]^T \in \RR^{T\times\infty}
    % $$
    % be the feature matrix with infinite number of columns, then we have the following properties,
    % \begin{align*}
    %     \Kv_T &= \Phi \Phi^T, \\
    %     \kv_T(\xv) &= \Phi \phi(\xv), \\
    %     \yv_T &= \Phi \btheta.
    % \end{align*}
    % Under the setting that $T\to \infty$, together we can derive
    % \begin{align}
    %     f(\xv) &= \phi(\xv)^T \btheta \nonumber\\
    %     & = (\Phi^{-1} \kv_T(\xv))^T (\Phi^{-1} \yv_T) \nonumber\\
    %     & = \kv_T(\xv)^T (\Phi\Phi^T)^{-1} \yv_T \nonumber\\
    %     & = \kv_T(\xv)^T \Kv_T^{-1} \yv_T. \label{eq:fse_equal}
    % \end{align}
    % For $\lambda$ being small enough, such that $\lambda \|\Kv_T^{-1}\|\le 1$ satisfies for an appropriate matrix norm,  we have the following Neumann series
    % \begin{align*}
    %     (\Kv_T + \lambda \Iv_T)^{-1} &= \Kv_T^{-1}(\lambda \Kv_T^{-1} + \Iv_T)^{-1} \\
    %     &= \Kv_T^{-1} -\lambda \Kv_T^{-2} + \lambda^2\Kv_T^{-3} - \ldots
    % \end{align*}
    % % By truncating the rest, $(\Kv_T + \lambda \Iv_T)^{-1}$ can be approximated by $\Kv_T^{-1} -\lambda \Kv_T^{-2} $.
    % On the one hand, by Cauchy-Schwartz inequality, we have
    % \begin{align*}
    %     f(\xv)^2 &= \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \Big(\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv^{\balpha} \Big)^2 \\
    %     &\le \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \sum_{\balpha\in\NNd}\mu_{\balpha}^2 \xv^{2\balpha} \\
    %     &= \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \exp\Big(\frac{\|\xv\|^2}{l^2}\Big) \\
    %     &= \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \\
    %     &\le B^2,
    % \end{align*}
    % so that the $L^2$-norm of $f$ is also bounded by $B$ since our domain is $[0,1]^d$.  On the other hand, recall \eqref{eq:fse_equal}, and again by Cauchy-Schwartz inequality, we write
    % \begin{align*}
    %     \|f(\xv)\|_{L^2} &= \Big\| \kv_T(\xv)^T \Kv_T^{-1} \yv_T \Big\|_{L^2} \\
    %     &\le \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \big\|\Kv_T^{-1} \big\|_F \cdot \|\yv_T\| \\
    %     &\le \sqrt{T} \max_{\xv^*\in\{\xv_1,\ldots,\xv_T\}} \big|f(\xv^*)\big| \sqrt{T \int_D \exp\Big(-\frac{\|\xv-\xv^*\|^2}{l^2}\Big) d\xv} \cdot \big\|\Kv_T^{-1} \big\|_F \\
    %     &\le TB\big\|\Kv_T^{-1} \big\|_F,
    % \end{align*}
    % where the last step is since $\max_{\xv\in D} |f(\xv)| \le B$ and $\max_{\xv^*} \int_D \exp\big(-\frac{\|\xv-\xv^*\|^2}{l^2}\big) d\xv \le 1$.  Equating the last equation with $B$, we can see that
    % \begin{equation}
    %     \big\|\Kv_T^{-1} \big\|_F  = \Theta\Big(\frac{1}{T}\Big). \label{eq:kernel_matnorm_upper}
    % \end{equation}
    % Therefore,
%     First, by triangle inequality, it is easy to observe that
%     \begin{equation}
%         \|f-\fhatsig\|_{L^2} \le \|f-\fhat\|_{L^2} + \|\fhat-\fhatsig\|_{L^2}.
%     \end{equation}
%     Thus, we aim to deal with these two terms separately. $\fhat$ can be explicitly written as the following:
%     \begin{equation*}
%         \fhat = \sum_{t=1}^{T} \beta_t \kse(\xv,\xv_t), \quad \text{where } (\beta_1,\ldots,\beta_T)^T = \Kv_T^{-1} \yv.
%     \end{equation*}

%     \begin{align}
%         \|\fhat - \fhatsig\|_{L^2} &= \Big\|\kv_T(\xv)^T \Kv_T^{-1} \yv_T -  \kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} \yv_T \Big\|_{L^2} \nonumber \\
%         &=\Big\|\kv_T(\xv)^T (\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}) \yv_T\Big\|_{L^2} \nonumber\\
%         &\le \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \Big\|\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}\Big\|_F \cdot \|\yv_T\| \nonumber\\
%         &\le O\bigg(T  \Big\|\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}\Big\|_F\bigg) \nonumber\\
%         &\le O\bigg( \frac{T\|\Kv_T^{-1}\|_F^2 \|\lambda \Iv_T\|_F}{1- \|\Kv_T^{-1}\lambda \Iv_T\|_F}\bigg) \label{eq:se_l2_upper_nosig_1} \\
%         &\le O\bigg( \frac{\|\Kv_T^{-1}\|_F^2}{1- \lambda\|\Kv_T^{-1}\|_F} \lambda T^{\frac{3}{2}}\bigg) \\
%         &\le O\Big(\frac{\lambda}{\sqrt{T}}\Big), \label{eq:se_l2_upper_nosig_2}
%     \end{align}
%     where \eqref{eq:se_l2_upper_nosig_1} -- \eqref{eq:se_l2_upper_nosig_2} has used Lemma \ref{lem:mat_inv_diff} and \eqref{eq:kernel_matnorm_upper}, and the fact that $\|\Iv_T\|_F = \sqrt{T}$, $\lambda\|\Kv_T^{-1}\|_F \ll 1$.
% \end{proof}

% \begin{cor} \label{cor:se_l2_upper_sig}
%     {\em (Noisy $L^2$ upper bound -- SE kernel)}
%     Under the setup of Theorem \ref{thm:se_l2_upper_nosig}, with only $\yv_T$ replaced by the noisy version.  Then, the error of estimating the noisy $L^2$-distance on $[0,1]^d$ is upper bounded by:
%     \begin{equation}
%        \EE[\|f-\mu_T\|_{L^2}] = O\Big( \lambda T^{-\frac{1}{2}} + T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \label{eq:se_l2_upper_sig}
%     \end{equation}
% \end{cor}
% \begin{proof}
%     Using Lemma \ref{lem:mat_norm_bound}, and the proof in Theorem \ref{thm:se_l2_upper_nosig}, it follows that
%     \begin{align}
%         \EE[\|f-\mu_T\|_{L^2}] &= \EE\bigg[\Big\|\kv_T(\xv)^T \Kv_T^{-1} \yv_T -  \kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} (\yv_T + \varepsilon_1)\Big\|_{L^2} \bigg] \nonumber\\
%         &\le \|f-\fhat\|_{L^2} + \EE\bigg[ \Big\|\kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} \varepsilon_1\Big\|_{L^2} \bigg] \nonumber\\
%         &\le \|f-\fhat\|_{L^2} +  \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \big\|\Kv_T^{-1} \big\|_F \cdot \EE[\|\varepsilon_1\|] \label{eq:se_l2_upper_sig_1}\\
%         &= O\Big(\lambda T^{-\frac{1}{2}} + T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \nonumber
%     \end{align}
% \end{proof}


% \begin{proof}
%     Since we have shown the supremacy of $\EE[|I-\Ihatsig|^2]$ in Lemma \ref{lem:int_sig_nosig}, we are left to show the supremacy of $\EE[\|f-\fhatsig\|_{L^2}^2]$:
%     \begin{align*}
%         \EE[\|f-\fhatsig\|_{L^2}^2] &= \EE\bigg[\Big\| f-\fhat - \sum_{t=1}^{T/2}\beta_t\epsilon_t  \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd}\frac{\xv^{\balpha}}{\theta_{\balpha}} \Big\|_{L^2}^2\bigg] \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\EE\bigg[\Big|\sum_{t=1}^{T/2}\beta_t\epsilon_t \Big|^2 \bigg] \Big\|\exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd}\frac{\xv^{\balpha}}{\theta_{\balpha}} \Big\|_{L^2}^2 \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\sum_{t=1}^{T/2}\beta_t^2 \EE[\|\varepsilon_1\|^2] \sum_{\balpha}\sum_{\bgamma} \frac{\int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv}{\Lambda_{\balpha}\Lambda_{\bgamma}} \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\sum_{t=1}^{T/2}\beta_t^2 \EE[\|\varepsilon_1\|^2] ,
%     \end{align*}
%     where the last inequality follows since \eqref{eq:int_residual} and $\Lambda_{\balpha}\Lambda_{\bgamma} \ge $
% \end{proof}

% Combining \eqref{eq:noisy_int_eq}, \eqref{eq:int_l2_nosig} and \eqref{eq:int_l2_sig} in these two lemmas, it is easy to see that 
% \begin{equation}
%     \sup_{\|f\|_{\se}\le 1}\EE[\|f-\fhat\|_{L^2}^2] \le \Big( \sup_{p\in\Pc,\|f\|_{\se}\le 1}|I-\Ihat| +  \sqrt{\sum_{t=1}^{T/2}\alpha_i^2} \EE[\|\varepsilon_1\|_2]\Big)^2 + \sum_{t=1}^{T/2}\alpha_i^2 \var[\|\varepsilon_1\|_2]. \label{eq:l2_se_sig}
% \end{equation}


% The first term in the above equation includes the worst-case noiseless integration error, $\rwstse$, which we can recall Theorem \ref{thm:noiseless_upper} part 3.  Therefore, it remains to bound $\sqrt{\sum_{t=1}^{T/2}\alpha_i^2}$.  In \cite{Bac17}, $\alpha_i$ is treated as the fraction of $\frac{\beta_i}{q(\xv_i)^{1/2}}$, where $\|\beta\|_2^2\le \frac{8}{T}$, and $q(\xv_i)$ is regarded as the {\em importance weight}, so that $\{\xv_1,\ldots,\xv_{T/2}\}$ are now sampled i.i.d from the density $q$.  Most importantly, the optimized distribution $q(\xv)\propto \sum_{m\ge 1} \frac{\mu_m}{\mu_m+\lambda}e_m(\xv)^2$, is uniform (which is a constant) on $[0,1]^d$, given the fact that the eigen-functions of the SE kernel integral operator can be expressed as the $d$-th order tensor product of the uni-dimensional Fourier basis.  For more details, one may refer to \citep[Section 4.4]{Bac17}.  Therefore, we are ready to obtain 
% \begin{equation*}
%     \sum_{t=1}^{T/2}\alpha_i^2 = \sum_{t=1}^{T/2}\frac{\beta_i^2}{q(\xv_i)} = O(\|\beta\|_2^2) = O\Big(\frac{1}{T}\Big).
% \end{equation*}
% To make the proof complete, we need to show that $\mu_{T/2}(\xv)$ is one kind of $\fhat$, indeed, $\mu_{T/2}(\xv) = \sum_{t=1}^{T/2} [(\Sigma + \lambda I)^{-1}\yv_{T/2})]_i \cdot k(\xv,\xv_i)$.  The proof is then finished by substituting the bound of $\rwstse$ and  $\sum_{t=1}^{T/2}\alpha_i^2 $ into \eqref{eq:l2_se_sig}.
% \section{Lower Bound on SE Kernel When $d=1$} \label{app:se_lower}
% For each $\btheta\in\{0,1\}^N$, we define $f_{\btheta}\in\Fc(B)$ (with the kernel being the SE kernel) as
% \begin{equation}
%     f_{\btheta}(x) = B\sqrt{\frac{\mu_N}{N}} \sum_{i=0}^{N-1} \btheta(i) \tau_i(x),
% \end{equation}
% where $\mu_N=\frac{1}{l^{2N} N!}$ and $\tau_i(\xv)=x^i\exp(-\frac{x^2}{2l^2})$.  It can be verified that $f$ belongs to $\Fc(B)$:
% \begin{equation*}
%     \|f\|_{\se}^2 = \frac{B^2\mu_N}{N}\sum_{i=1}^{N}\frac{\theta^2}{\mu_k} \le \frac{B^2\mu_N}{N}\sum_{i=1}^{N}\frac{\theta^2}{\mu_N} \le B^2.
% \end{equation*}

% It is worth noting that the decreasing sequence $\mu_0\ge\mu_1\ge\ldots\ge 0$ and the corresponding functions $\{\tau_i(x)\}_{i=0}^{\infty}$ forms an eigen system of the following integral operator $(\Lk f)(\xv) : L^2(D)\rightarrow L^2(D)$:
% \begin{equation*}
%     (\Lk f)(\xv) = \int_D k(\xv, \yv) f(\yv) d\yv = \langle k(\xv,\cdot), f \rangle_{L^2},
% \end{equation*}
% which applying to the eigenfunctions, we have
% \begin{equation*}
%     (\Lk \tau_{\balpha})(\xv) = \mu_{\balpha} \tau_{\balpha}(\xv).
% \end{equation*}
% Then, the spectral theorem implies that the SE kernel can be decomposed into:
% \begin{equation*}
%     k(\xv,\yv) = \sum_{\balpha\in\NNd} \mu_{\balpha} \tau_{\balpha}(\xv) \tau_{\balpha}(\yv).
% \end{equation*}
% Moreover, it turns out that the square root of the operator, $\Lk^{1/2}$, is an isometric embedding of $L^2\rightarrow\se$.  Specifically, for $f,g\in L^2(D)$, we have
% \begin{equation*}
%     \langle\Lk^{1/2}f, \Lk^{1/2}g\rangle_{\se} = \langle f, g\rangle_{L^2}.
% \end{equation*}
% Similarly, for kernel $k(\xv,\yv)$, we have
% \begin{equation*}
%     k(\xv,\yv) = \langle k(\xv,\cdot), k(\yv,\cdot)\rangle_{\se} = \langle\Lk^{1/2}\psi(\xv,\cdot), \Lk^{1/2}\psi(\xv,\cdot)\rangle_{\se} =\langle \psi(\xv,\cdot), \psi(\yv,\cdot)\rangle_{L^2},
% \end{equation*}
% where $\psi(\xv,\yv)$ can be decomposed into:
% \begin{equation*}
%     \psi(\xv,\yv) = \sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv) \tau_{\balpha}(\yv).
% \end{equation*}


% \begin{thm} \label{thm:se_lower_worst}
%     {\em (SE kernel worst-case lower bound)} 
%     For a family of functions $\{\psi_1(\xv),\ldots,\psi_T(\xv)\}\in L^2(D)$ satisfying the following conditions
%     \begin{itemize}
%         \item[(i)] $\frac{1}{T}\sum_{i=1}^{T}\|\psi_i(\xv)\|_{L^2} \le \tr(L)$
%         \item[(ii)] $\sup_{f\in\Fc}\inf_{\sum_{i=1}^{T}\beta_i^2\le \frac{1}{T}} \|f-\sum_{i=1}^{T}\beta_i\psi_i\|_{L^2} \le \epsilon$ 
%     \end{itemize}
%     Then,
%     \begin{equation*}
%         T = \Omega\bigg(\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big)^d\bigg).
%     \end{equation*}
% \end{thm}

% Using Varshamov-Gilbert’s lemma, there exists a family of $\{\btheta_j\}_{j\in\Jc}$, such that for $j\neq j'\in\Jc$, $\|\btheta_j - \btheta_{j'}\|^2 \ge \frac{N}{4}$, and consequently, $\|f_{\btheta_j} - f_{\btheta_{j'}}\|_{L^2} = \frac{B^2\mu_N}{N} \|\btheta_j - \btheta_{j'}\|^2 \ge \frac{B^2\mu_N}{4}$.  

% For algorithms linearly combining the evaluations $\{f(\xv_1),\ldots f(\xv_T)\}$, the mean absolute error can be expressed using the reproducing property:
% \begin{align*}
%     \Big| \int_D f(\xv) d\xv - \sum_{i=1}^{T} \beta_i f(\xv_i) \Big| &= \Big| \langle f,   \int_D k(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i k(\xv_i,\cdot) \rangle_{\se} \Big|\\
%     &\le \|f\|_{\se} \cdot \Big\|\int_D k(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i k(\xv_i,\cdot) \Big\|_{\se} \\
%     &\le B \Big\|\int_D \psi(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i \psi(\xv_i,\cdot) \Big\|_{L^2}  \\
%     &= B \Big\|\int_D \sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv) \tau_{\balpha}(\cdot) d\xv - \sum_{i=1}^{T} \beta_i \sum_{\balpha\in\NNd}\sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv_i) \tau_{\balpha}(\cdot) \Big\|_{L^2} \\
%     &= B \Big\|\sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} \\
%     &= B \Big\|\sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} \\
%     &\le B \sum_{\balpha\in\NNd} \Big\|\sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} 
% \end{align*}




% We note that $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence, i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{2N}$.

% From the definition of RKHS norm, $\|f\|_{\se}^2 = \sum_{i\ge 0} \frac{\langle f, \tau_{i}\rangle_{L^2}^2}{\mu_i}$, it can be verified that $f$ belongs to $\Fc(B)$:
% \begin{align*}
%     \|f\|_{\se}^2 = \frac{B^2\mu_{2N}}{N} \Big(\frac{\theta_k^2 }{\mu_{2k}}+ \sum_{m\in M}\frac{\theta_m^2}{\mu_{2m-1}} \Big) = \frac{B^2}{N} \Big(\frac{\mu_{2N}}{\mu_{2k}}\theta_k^2 + \sum_{m\in M}\frac{\mu_{2N}}{\mu_{2m-1}} \theta_m^2 \Big) \le B^2,
% \end{align*}
% where the first equality is since $\langle \tau_i,\tau_i\rangle_{L^2} = 1$ whereas $\langle \tau_i,\tau_j\rangle_{L^2} = 0$ for $i\neq j$.

% On the other hand, we have
% \begin{equation*}
%     \int_{-1}^1 f(x) dx = \frac{B\sqrt{\mu_{2N}}}{\sqrt{N}} \int_{-1}^{1} \Big(\theta_k \tau_{2k}(x) +\sum_{m\in M} \theta_m \tau_{2m-1}(x) \Big) dx = \frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \theta_{k} \int_{0}^1 \tau_{2k}(x) dx,
% \end{equation*}
% since $\{\tau_{2m-1}\}$ are odd functions and $\tau_{2k}$ is even.  Therefore, the worst case error is at least 
% \begin{align*}
%     |I(f) - 0| &= \Big|\frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \theta_k \int_0^1 x^{2k} \exp(-\frac{x^2}{2l^2})dx  \Big|\\
%     &\ge \frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \int_0^1 x^{2N} \exp(-\frac{x^2}{2l^2})dx \\
%     &\ge \frac{2B}{\sqrt{N}l^{2N} \sqrt{2N!} } \exp(-\frac{1}{2l^2})\int_{0}^{1} x^{2N} dx\\
%     &= \Omega\Big(\frac{1}{N\sqrt{N}\sqrt{2N!}} \Big) \\
%     &= \Omega\Big(\frac{1}{N\sqrt{N}}\big(\frac{e}{2N}\big)^{N} \Big).
% \end{align*}

==> se.tex <==
% \begin{thm}\label{thm:noiseless_lower}
%     {\em (Average-Case Noiseless SE Lower Bound)}
%     Consider our problem setup with constant parameters $(B,d,l,T)$.  Then, there exists a constant $C_l>0$ such that for any algorithm (possibly adaptive and/or randomized) for estimating $I(f)$ with $f\in \se$, the average-case error is at least:
%         \begin{equation}\label{eq:se_lb_nosig}
%             \ravgse = \Omega\big(e^{-C_l T^{\frac{2}{d}}} T^{-1} \big).
%         \end{equation}
%     Moreover, this lower bound holds even under the fixed weight function $p(\xv) = 1$.
% \end{thm}

\begin{thm} \label{thm:wst_se_nosig}
    {\em (Worst-Case Noiseless SE Upper Bound)} For $f$ lies in SE RKHS with $\|f\|_{\se}\le B$, then, any linear algorithm that uses the linear combination of noiseless function evaluations satisfies the following regrets: 
    \begin{enumerate}
        \item If the algorithm is tensor-product based Gauss-Hermite rule, then
        \begin{equation}
            \rwstse \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}},
        \end{equation}
        where $C_{gh} = B\big(\frac{e}{l^2}\big)^{\frac{d}{2}T^{\frac{1}{d}}}$.
        \item If the algorithm simply combines $\sum_{t=1}^{T} w_t f(\xv_t)$ for arbitrary $\{\xv_t\}_{t=1}^{T}$, with $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$, then:
        \begin{equation}
            \rwstse \le (C_l+1) C_{gh} T^{-\frac{1}{2}T^{\frac{1}{d}}},
        \end{equation}
        where $C_l:=\sqrt{\big(\frac{\pi}{6}\big)^d + o(1)}$.
    \end{enumerate}
\end{thm}

The above results indicate that Gauss-Hermite rules are not necessary in solving noiseless SE kernel quadrature, at least not in a bounded domain, since the error only differs by a constant factor.

The RKHS function class induced by SE kernel $\kse(\xv,\xv')=\exp\big(-\frac{\|\xv-\xv'\|^2}{2 l^2}\big)$ can be defined by
\begin{equation}
    \se = \Big\{f(\xv)=\sum_{\balpha\in\NNd} \theta_{\balpha} e_{\balpha}(\xv), \|f\|_{\se}^2:=\sum_{\balpha\in\NNd} \theta_{\balpha}^2 < \infty \Big\}, \label{eq:se_rkhs}
\end{equation}
where $\NN_0:=\NN\cup\{0\}$, and $\big\{e_{\balpha}(\xv) = \prod_{i=1}^{d} \frac{1}{l^{\balpha_i}\sqrt{\balpha_i !}} \xv_i^{\balpha_i} \exp\big(-\frac{\xv_i^2}{2l^2}\big)\big\}_{\balpha\in\NNd}$ forms an orthonormal
basis for $\se$.  The details of this SE RKHS function class can be found in \cite{Ste06} and \cite{Min10}.  By denoting $\balpha ! = \prod_{i=1}^{d} \balpha_i !$ and $\xv^{\balpha}  = \prod_{i=1}^{d} \xv_i^{\balpha_i}$, we can simplify the notion as 
\begin{equation}
    e_{\balpha}(\xv) = \frac{1}{l^{|\balpha|}\sqrt{\balpha !}} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big) = \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big),
\end{equation}
with $\mu_{\balpha} := \frac{1}{l^{|\balpha|}\sqrt{\balpha !}}$.



\section{Proof for Theorem \ref{thm:noiseless_lower} (Average-case SE Lower Bound)}\label{app:se_avg_lb}
% \subsection{Function Class Construction}
Instead of specifying the function class in the case of the SE kernel directly, we consider the bump function $\Phi(\bxi)=\exp(\frac{-1}{1-\|\bxi\|^2})\openone\{\|\bxi\|<1\}$ in the frequency domain.  Since $\Phi(\bxi)$ is infinitely differentiable, its inverse Fourier transform, $\phi(\xv)$, decays to zero as $\|\xv\|\rightarrow\infty$, at a rate faster than any finite power of $\|\xv\|^{-1}$.  Then, there exists a point $\bzeta=[\zeta,\ldots,\zeta]$ such that $\phi(\bzeta) \le \frac{1}{d\zeta^{n}}$ for $n$ sufficiently large.  We choose $\psi(\xv)=\frac{\epsilon}{\phi(\bzero)}\phi(\frac{\xv\zeta}{\omega})$ in the similar fashion as of $g(\xv)$ in the previous section, where $\omega$ is the diameter of the gird.  Let $\psi_1(\xv),\ldots,\psi_M(\xv)$ denote the shifted version of $\psi(\xv)$ which centered at the $M$ grids respectively.  

% Before preceding, the following lemma is useful for functions $\{\psi_i(\xv)\}$.
% \begin{lem} \label{lem:func_sum_bound}
%     {\em (\citep[Lemma 7]{Sca17a})}
%     The functions $\{\psi_j(\xv)\}$ established as above are such that the quantities $\vbar_i^j:=\max_{\xv\in D_i} |\psi_j(\xv)|$ satisfy $\sum_{j=1}^{M} (\vbar_i^j)^2 = O(\epsilon^2)$.
% \end{lem}

For functions of the form $\rho(\xv):=\sum_{i=1}^{M}\delta_i\psi_i(\xv)$, letting $I_i:=\int_{\xv\in D_i}\rho(\xv)d\xv$ denote the integral of $\rho(\xv)$ in cell $i$, then for $\delta_i=1$, $I_i$ is at least:
\begin{align}
    I_i &= \int_{\xv\in D_i}\rho(\xv)d\xv \nonumber\\
    &= \int_{\xv\in D_i}\sum_{j=1}^{M} \delta_j \psi_j(\xv) d\xv \nonumber\\
    &\ge \int_{\xv\in D_i} \psi_i(\xv) d\xv - \sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv. \label{eq:se_inti_lower1}
\end{align}
The first integral in the above equation is the area of the dominate bump of $\psi_i$, which is at least $\Omega(\omega^d \epsilon)$.  It now remains to determine the magnitude of $I_i':=\sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv$:
\begin{align}
    I_i' &= \sum_{j\neq i}^{M}\int_{\xv\in D_i}|\psi_j(\xv)| d\xv \nonumber\\
    &= O\big((M-1) w^d |\psi(\bw)| \big)  \nonumber\\
    &= O\Big( M w^d \frac{\epsilon}{\phi(\bzero)}|\phi(\bzeta)| \Big)\nonumber\\
    &= O\Big( \frac{\epsilon}{\phi(\bzero) d\zeta^n} \Big)\nonumber,
\end{align}
where we have used $M=\lfloor \frac{1}{\omega}\rfloor^d$.  It is easy to choose constants $n=c'n'$ such that $\zeta^{c'}>\omega^{-1}$, and $n'>d$, so that $\zeta^n = \zeta^{c'n'} > \omega^{-d}$.  From function construction perspective, for our current choice of $\zeta$ and $n$, each of the $\psi_i(\xv)$ is now principally ``well-separated''.  Therefore $I_i'= O(\omega^d \epsilon)$, which can be absorbed into the first term of \eqref{eq:se_inti_lower1}, and obtain
\begin{equation}\label{eq:se_inti_lower}
    I_i = \Omega\Big(\frac{\epsilon}{M}\Big).
\end{equation}
% Note also that if we only consider the dominate bump of cell $i$, $\psi_i(\xv)$, the integral of cell $i$ will be at least $\Omega(\omega^d\epsilon)$.  Combining this with \eqref{eq:cellint_upper}, we find that $I_i^2 = \Theta(\omega^{d} \epsilon^2)$
To control the RKHS norm of $\rho(\xv)$, we may use the following well-known lemma.

\begin{lem}\label{lem:rkhs_fourier}
 Consider an RKHS $\Hc$ for functions on $\RR^d$, corresponding to a translation invariant kernel $k(\tau)$, and let $K(\bxi)$ be the $d$-dimensional Fourier transform of $k(\tau)$. Then for any $f\in\Hc$ with Fourier transform $\fhat(\bxi)$, we have
 \begin{equation} \label{eq:rkhs_norm}
 \|f\|_{\Hc}^2 = \int K(\bxi)^{-1} |\fhat(\bxi)|^2 d\bxi,
 \end{equation}
 and the Fourier transform of $f$ given by
 \begin{equation*}
 \fhat(\bxi)=(2\pi)^{-d/2}\int f(\xv)e^{-j\langle \bxi,\xv \rangle}d\xv
 \end{equation*}
\end{lem}
In our case, the Fourier transform of the SE kernel is 
\begin{equation}
 K(\bxi) = (2\pi l^2)^{d/2}e^{-2\pi^2 l^2\|\bxi\|^2}, \label{eq:se_fourier}
\end{equation}
and the Fourier transform of $\rho(\xv)$ can be interpreted as
\begin{align}
    \rhohat(\bxi) &=(2\pi)^{-d/2}\int_{\xv\in D} \sum_{i=1}^{M}\delta_i \psi_i(\xv)e^{-j\langle\bxi,\xv\rangle}d\xv \nonumber\\
    &=(2\pi)^{-d/2}\int_{\xv\in D} \sum_{i=1}^{M}\delta_i \psi(\xv-\sv_i)e^{-j\langle\bxi,\xv\rangle}d\xv \label{eq:rho_fourier_1}\\
    &=(2\pi)^{-d/2}\sum_{i=1}^{M}\delta_i \int_{\xv\in D}\psi(\xv-\sv_i)e^{-j\langle\bxi,\xv\rangle}d\xv \nonumber\\
    &= \frac{\omega^d \epsilon}{(2\pi)^{d/2}\zeta^d\phi(\bzero)} \sum_{i=1}^{M} \delta_i e^{-j\langle\bxi,\sv_i\rangle} \Phi\Big(\frac{\omega}{\zeta}\bxi\Big) \label{eq:rho_fourier}
\end{align}
In the equations above: $\sv_i$ in \eqref{eq:rho_fourier_1} is a $d$-dimensional shifting vector for function $\psi_i(\xv)$ with each dimension taking value from $\{\omega, 2\omega,\ldots, \lfloor\frac{1}{\omega}\rfloor\omega\}$; \eqref{eq:rho_fourier} uses the fact that the $d$-dimensional Fourier transform of $af(\frac{\xv-\cv}{b})$ is $e^{-j\langle\bxi, \cv\rangle}ab^d F(\bxi b)$.

Now, recalling the definition of the RKHS norm in \eqref{eq:rkhs_norm}, and combining \eqref{eq:se_fourier} and \eqref{eq:rho_fourier}, the RKHS norm of $\rho(\xv)$ in terms of the SE kernel is given by
\begin{align}
 \|\rho(\xv)\|_{\se}^2 &= \frac{\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\frac{\bxi\omega}{\zeta}\|_2\le 1} \Big|\sum_{i=1}^{M} \delta_i e^{-j\langle\bxi,\sv_i\rangle} \Phi\Big(\frac{\omega}{\zeta}\bxi\Big)\Big|^2 e^{2\pi^2 l^2 \|\bxi\|_2^2} d\bxi \nonumber\\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\frac{\bxi\omega}{\zeta}\|_2\le 1} \exp\Big(2\pi^2 l^2 \|\bxi\|_2^2 - \frac{2}{1-\|\frac{\omega\bxi}{\zeta}\|_2^2}\Big) d\bxi \nonumber\\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} \int_{\|\bxi\|_2\le \frac{\zeta}{\omega}} \exp\big(2\pi^2 l^2 \|\bxi\|_2^2\big) d\bxi \nonumber \\
 &\le \frac{M^2\omega^{2d}   \epsilon^2}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^{2d}\phi(\bzero)^2} V\Big(\frac{\zeta}{\omega}\Big) \exp\Big(\frac{2\pi^2 l^2 \zeta^2}{\omega^2}\Big) \label{eq:ball_volume_1} \\
 &\le \frac{ M^2 \omega^{d} \epsilon^2 \pi^{d/2}}{(2\pi)^{d}(2\pi l^2)^{d/2}\zeta^d\phi(\bzero)^2\Gamma(\frac{d}{2}-1)} \exp\Big(\frac{2\pi^2 l^2 \zeta^2}{\omega^2}\Big) \label{eq:ball_volume_2} \\
 &=O\Big(M \epsilon^2 e^{2\pi^2 l^2 \zeta^2 M^{\frac{2}{d}}}\Big), \label{eq:rho_se_norm_upper_square}
\end{align}
where \eqref{eq:ball_volume_1} follows by upper bounding $\|\bxi\|_2^2\le \zeta^2\omega^{-2}$, and defining $V(\zeta\omega^{-1})$ to be the volume of a ball of radius $\zeta\omega^{-1}$ in $d$ dimensions: $V(\zeta\omega^{-1}) := \frac{\pi^{d/2}}{\Gamma(\frac{d}{2}-1)}(\zeta\omega^{-1})^d$, which immediately yeilds \eqref{eq:ball_volume_2}.  \eqref{eq:rho_se_norm_upper_square} again uses $M=\lfloor\frac{1}{\omega}\rfloor^d$.

Equating \eqref{eq:rho_se_norm_upper_square} with $B^2$ (so that $\|\rho(\xv)\|_{\se}\le B$), we have that 
\begin{equation}\label{eq:eps_M_se}
    \epsilon = \Theta\bigg(\frac{B}{\sqrt{M}e^{C_l' M^{\frac{2}{d}}}}\bigg), \quad C_l':=\pi^2 l^2 \zeta^2.
\end{equation}

For completion of the average-case proof, we will make use of a probabilistic result known as Khinchin’s inequality.
\begin{lem}\label{lem:khin}
    {\em (Khinchin’s Inequality)}
    Let $\delta_i$ be i.i.d distributed random variables with $\delta_i=\pm 1$ with equal probability, then 
    \begin{equation*}
        \EE\bigg[\Big|\sum_{i=1}^T c_i \delta_i\Big|\bigg] \ge \sqrt{\sum_{i=1}^{T} c_i^2}.
    \end{equation*}
\end{lem}
In our case, similar to the proof in Appendix \ref{app:mat_lower}, let $c_i=I_i$, and consider $T=\frac{M}{2}$, the expected error is then
\begin{equation*}
    \ravgse = \EE\bigg[\Big|\sum_{i=1}^{M/2} I_i \delta_i\Big|\bigg] \ge \sqrt{\sum_{i=1}^{M/2} I_i^2} = \Omega\Big(\frac{\epsilon}{\sqrt{M}}\Big) = \Omega\big(e^{-C_l T^{\frac{2}{d}}} T^{-1} \big),
\end{equation*}
with $C_l :=\pi^2 l^2 \zeta^2 2^{\frac{2}{d}}$.



% Since any function in SE RKHS can be written as an infinite series, recall the definition in \eqref{eq:se_rkhs}, any finite combination of those series also belongs to $\se$.  In this sense, for a multidimensional index $\balpha = [\alpha,\ldots,\alpha]$, we consider the following $g(\xv)\in\se$ 
% \begin{equation*}
%     g(\xv) = \frac{B}{M} \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2 }{2l^2}\Big), \quad \xv \succ \bzero\footnote{This is an element-wise inequality.}.
% \end{equation*}
% This function has an infinitely supported bump for $\xv\succ \bzero$, where the peak value $h^*$ depends on the value of $\alpha$.  In fact, we can take the first-order derivative of $g(\xv)$ along a single dimension, and get
% \begin{equation*}
%     \frac{g'(x) M}{B\mu_{\alpha}} = \alpha x^{\alpha-1} \exp\Big(-\frac{x^2 }{2l^2}\Big) - \frac{x^{\alpha+1}}{l^2} \exp\Big(-\frac{x^2 }{2l^2}\Big).
% \end{equation*}
% Letting $h'(x) = 0$, we see that $h^*$ is taken at $\bw'=[w',\ldots,w']$ with $w'= l\sqrt{\alpha}$, and 
% \begin{align*}
%     h^* &= h(\bw') \\
%     &= \frac{B}{M} \mu_{\balpha} \big(l\sqrt{\alpha}\big)^{d\alpha} e^{-\frac{d\alpha}{2}} \\
%     &= \frac{B}{M} .
% \end{align*}
% The function value at $\bzeta=C_{\zeta}\bzeta$ is
% \begin{equation*}
%     h(\bzeta) = \Big(\frac{C_{\zeta} l'\sqrt{\alpha}}{e^{C_{\zeta}^2/2}}\Big)^{d\alpha},
% \end{equation*}
% where for suitably chosen $l'$ and $C_{\zeta}$, $h(\bzeta)\to 0$.  We call $\zeta = C_{\zeta}l'$ the ``width'' of function $h$.  Note that we do not mean that the bump function is finitely supported, but doing so would allow us to focus on the most informative part of the function.  For $\xv \prec \bzero$, we make the function symmetric by letting $h(\xv)=h(-\xv)$, so that the function has two bumps in $\RR^d$, within the region $[-\zeta,\zeta]^d$.

% For our domain $D=[0,1]^d$, we rescale $h(\xv)$ into $g(\xv)\in \se$ and truncate it by $D$, so that the width becomes $w\in(0,1)$ and height becomes $\epsilon$:
% \begin{equation}\label{eq:se_g_1}
%     g(\xv) = \frac{\epsilon}{h^*} h\Big(\frac{\xv\zeta}{w}\Big) = \frac{\epsilon \zeta^{d\alpha}}{h^* w^{d\alpha}}  \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big), \quad l:= \frac{l' w}{\zeta}.
% \end{equation}
% We can construct $M=\lfloor \frac{1}{2w} \rfloor ^d$ of such $g(\xv)$ in the domain $D=[0,1]^d$, by shifting the dual-bump of $g(\xv)$ (within $[-w,w]^d$) into these $M$ grids, denoted by $g_i(\xv), i\in\{1,\ldots,M\}$.  The function $f$ we are interested is now of the form $f(\xv) = \sum_{i=1}^{M} \delta_i g_i(\xv)$, where $\delta_i\in\{+1,-1\}$ with equiprobability.  The RKHS norm of $f$ is given by the definition in \eqref{eq:se_rkhs},
% \begin{equation*}
%     \|f\|_{\se} \le M\|g\|_{\se} = \frac{\epsilon \zeta^{d\alpha}}{h^* w^{d\alpha+d} 2^d \mu_{\balpha}}.
% \end{equation*}
% Thus, $\|f\|_{\se}$ is bounded by $B$ by a choice of $\epsilon$ satisfying
% \begin{align}
%     \epsilon &= \frac{B h^* w^{d\alpha +d} 2^d\mu_{\balpha}}{\zeta^{d\alpha}} 
%     % & = \Theta (\frac{B (l'\sqrt{\alpha})^{d\alpha} w^{d(\alpha+1)} \sqrt{e}^{d\alpha}}{(\sqrt{e}^{d\alpha}) (l\sqrt) } ))
% \end{align}


% Substituting this back into \eqref{eq:se_g_1}, $g(\xv)$ can be simplified into
% \begin{equation}\label{eq:se_g}
%     g(\xv)=B (2w)^{d} \mu_{\balpha} \xv^{\balpha} \exp\Big(-\frac{\|\xv\|^2}{2l^2}\Big).
% \end{equation}

% From \eqref{eq:se_g}, we see that the integration of $g(\xv)$ in $[0,w]^d$, is at least 
% \begin{equation*}
%     B w^{d} 2^d\mu_{\balpha}e^{-\frac{1}{2l^2}} \int_{\xv\in[0,w]^d} \xv^{\balpha} d\xv = \frac{B w^{d(\alpha+1)} 2^d\mu_{\balpha}e^{-\frac{1}{2l^2}}}{(\alpha+1)^d},
% \end{equation*}
% since $\int_{\xv\in[0,w]^d} \xv^{\balpha} d\xv = \frac{w^{d\alpha}}{(\alpha+1)^d}$

% Let 
% \begin{equation*}
%     I_i = \int_{\xv\in D_i} f(\xv) d\xv =  \sum_{j=1}^M \delta_i \int_{\xv\in D_i} g_j(\xv) d\xv
% \end{equation*}
% be the integral of $f$ in region $i$.  Suppose $\delta_i=1$ at region $i$, therefore, the lower bound for $I_i$ is
% \begin{align*}
%     I_i &\ge \int_{\xv\in D_i} g_i(\xv) d\xv - \sum_{j\neq i}^M \int_{\xv\in D_i} g_j(\xv) d\xv \\
%     &=  \int_{\xv\in D_i} g_i(\xv) d\xv - \int_{\xv\notin D_i} g_i(\xv) d\xv \\
%     &= 2\int_{\xv\in [0,w]^d} g(\xv) d\xv - \int_{\xv\in [w,1]^d} g(\xv) d\xv \\
%     &\ge \Omega\big(w^d g^*) - B w^d \mu_{\balpha}  \int_{\xv\in [w,1]^d} \xv^{\balpha} d\xv  \\
%     &= \Omega\big(w^{3d} \mu_{\balpha}) - B w^d \mu_{\balpha} \frac{1-w^{d\alpha}}{(\alpha+1)^d} \\
%     &\approx \Omega\big(w^{3d} \mu_{\balpha}),
% \end{align*}
% where we have used the fact that $g(\xv)$ decays to $0$ after $[w,\ldots,w]$, this can also be seen by considering large $\alpha$ and $d$ in the second-last inequality.

% Finally, we are able to use the same technique as we have done in Appendix \ref{app:mat_lower}, by considering $T=\Theta(M)$ and $\alpha=T^{\frac{1}{d}}$.  Therefore, we obtain
% \begin{equation*}
%     \rwstse = \Omega(M I_i) = \Omega(T^{-\frac{1}{2}} \alpha^{-d\alpha/2}) = \Omega(T^{-\frac{1}{2}T^{\frac{1}{d}}-\frac{1}{2}}).
% \end{equation*}


\section{Proof for Theorem \ref{thm:wst_se_nosig} (Worst-case Noiseless SE Upper Bound)} \label{app:wst_se_nosig}

\subsection{Proof for Gauss-Hermite Rules}
Consider the $1$-D case, let $\tau_{\alpha}(x)=x^{\alpha} \exp(-\frac{x^2}{2l^2})$, the integral of $\tau_{\alpha}(x)$ is then defined in terms of the integral of the polynomial $x^{\alpha}$ with Gaussian weighting function $\exp(-\frac{x^2}{2l^2})$.  A well-known solution to such integrand is the Gauss-Hermite rule for its exactness when solving polynomials, see for example \cite{Bar78}.  Such case also holds for multivariate integration if we make use of tensor product based Gauss-Hermite rules.  Formally, for dimension $i$, the Gauss-Hermite rule is exact for $I(x^{\balpha_i}\exp(-\frac{x^2}{2l^2}))$ with $\balpha_i/2$ query points (for derivation simplicity, we will use $\balpha_i$ instead of $\balpha_i/2$ since we are accounting for the upper bound and it will only affect the final results up to a constant factor).  By the arithmetic-geometric inequality, for any tensor product based Gauss-Hermite rule with a budget of $T:=\prod_{i=1}^{d}\balpha_i$ queries, we must have $|\balpha|\ge d T^{1/d}:=N$.  With this in mind, for $f\in\se$, the worst case error can be bounded in the following sense:
\begin{align}
    |I(f) - \Ihat(f)| &= \Big|\int_{\xv\in D} \sum_{\balpha\in\NNd}\theta_{\balpha}e_{\balpha}(\xv) d\xv - \Ihat\Big| \nonumber\\
    &\le \Big| \sum_{|\balpha|=N}^{\infty} \int_{\xv\in D}\theta_{\balpha}e_{\balpha}(\xv) d\xv \Big| \label{eq:se_worst_align_1}\\
    &\le \sup_{\xv\in D} \Big| \sum_{|\balpha|=N}^{\infty}  \theta_{\balpha}e_{\balpha}(\xv) d\xv \Big| \label{eq:se_worst_align_2}\\
    &\le \sup_{\xv\in D} \sqrt{\sum_{|\balpha|=N}^{\infty} \theta_{\balpha}^2} \cdot \sqrt{\sum_{|\balpha|=N}^{\infty} e_{\balpha}^2(\xv)} \label{eq:se_worst_align_3}\\
    &\le \sup_{\xv\in D} B \sqrt{\sum_{|\balpha|=N}^{\infty} e_{\balpha}^2(\xv)} \label{eq:se_worst_align_4}\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{|\balpha|=N}^{\infty} \frac{1}{l^{2|\balpha|}\balpha !} \xv^{2\balpha} \exp\big(-\frac{\|\xv\|^2}{l^2}\big)} \nonumber\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{k=N}^{\infty} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \sum_{|\balpha|=k} \frac{1}{l^{2k}\balpha !} \xv^{2\balpha} } \nonumber\\
    &= \sup_{\xv\in D} B \sqrt{\sum_{k=N}^{\infty} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \frac{1}{k!} \sum_{|\balpha|=k} \frac{k!}{\balpha_1 !\cdots \balpha_d !}\big(\frac{\xv_1^2}{l^2}\big)^{\balpha_1}\cdots\big(\frac{\xv_d^2}{l^2}\big)^{\balpha_d} }  \nonumber \\
    &= \sup_{\xv\in D} B \sqrt{\exp\big(-\frac{\|\xv\|^2}{l^2}\big)\sum_{k=N}^{\infty}  \frac{1}{k!} \big(\frac{\xv_1^2+\ldots+\xv_d^2}{l^2}\big)^k} \label{eq:se_worst_align_5}\\
    &\le \sup_{\xv\in D} B \sqrt{\exp\big(-\frac{\|\xv\|^2}{l^2}\big) \frac{\|\xv\|^{2N}}{l^{2N}N!}\exp\big(\frac{\|\xv\|^2}{l^2}\big)} \label{eq:se_worst_align_6}\\
    &\le \sup_{\xv\in D} B \sqrt{\big(\frac{ed}{l^2 N}\big)^N} \label{eq:se_worst_align_7}
    % &= O\Big(\big(\frac{e}{N}\big)^{\frac{N}{2}}\Big). \label{eq:se_error_worst}
\end{align}
In the above equations:
\begin{itemize}
    \item \eqref{eq:se_worst_align_1} is since tensor product based Gauss-Hermite rules are exact for all $\theta_{\balpha}e_{\balpha}$ with $|\balpha|\le N$, thus the error is upper bounded by the residual;
    \item \eqref{eq:se_worst_align_2} is since $D=[0,1]^d$ and \eqref{eq:se_worst_align_3} follows from Holder's inequality with the counting measure;
    \item \eqref{eq:se_worst_align_4} is because we are only considering RKHS functions with smoothness $B$, i.e., $\sum_{|\balpha|=N}^{\infty}\theta_{\balpha}^2 < \sum_{\balpha\in\NNd}\theta_{\balpha}^2 = B^2$;
    \item \eqref{eq:se_worst_align_5} follows since the multinomial theorem;
    \item \eqref{eq:se_worst_align_6} uses the fact that $\sum_{n=N}^{\infty}\frac{x^n}{n!}\le \frac{x^N}{N!}e^{y}$, where $0<y\le x$;
    \item \eqref{eq:se_worst_align_7} is simplified due to Stirling's formula, $n!\sim\big(\frac{n}{e}\big)^n$, and $\|\xv\|^2\le d$
\end{itemize}

Recalling that $N=dT^{\frac{1}{d}}$, we obtain
\begin{equation*}
    \rwstse \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}}, \quad C_{gh} := B\Big(\frac{e}{l^2}\Big)^{\frac{d}{2}T^{\frac{1}{d}}}
\end{equation*}

\subsection{Proof for Regular Linear Algorithms}
Since normal linear algorithms cannot guarantee that the first $N:=d T^{\frac{1}{d}}$ series to be exactly solved like Gauss-Hermite rules, the error incurred by such algorithms are two-folds: The error for approximating the first $N$ series and the residual.  In this case, we consider $f\in\se$ in the following form,
\begin{equation*}
    f(\xv) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv^{\balpha},
\end{equation*}
with RKHS norm
\begin{equation} \label{eq:se_f_rkhs}
    \|f\|_{\se}^2 = \sum_{|\balpha|=0}^{N}\frac{\theta_{\balpha}^2}{\mu_{\balpha}^2} \le B^2.
\end{equation}
Let the quadrature rule be
\begin{equation*}
    \Ihat(f) = \sum_{t=1}^{T} w_t f(\xv_t),
\end{equation*}
and regularized by $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$.  Being in the worst-case setting, the maximum $\balpha^*$ that satisfies $|\balpha^*|=N$ is taken at $\balpha^*=[\frac{N}{d},\ldots,\frac{N}{d}]$.  Thus, we derive
\begin{align}
    |I(f) - \Ihat(f)| &= \bigg|\int_D \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv^{\balpha} d\xv - \sum_{t=1}^{T} w_t \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{|\balpha|=0}^{N} \theta_{\balpha}\xv_t^{\balpha} \bigg| \nonumber\\
    &\le \bigg| \sum_{|\balpha|=0}^{N} \theta_{\balpha} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv - \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)\Big) \bigg| \nonumber\\
    &\le \sqrt{\sum_{|\balpha|=0}^{N} \theta_{\balpha}^2} \sqrt{\sum_{|\balpha|=0}^{N} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv - \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)\Big)^2}  \label{eq:se_linear_int_upper_1} \\
    &\le B\mu_{\balpha^*} \sqrt{\sum_{|\balpha|=0}^{N} \Big(\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \Big)^2 + \sum_{|\balpha|=0}^{N} \Big( \sum_{t=1}^{T} w_t \xv_t^{\balpha} \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \Big)^2} \label{eq:se_linear_int_upper_2}\\
    &\le B\sqrt{\Big(\frac{1}{l^{\frac{2N}{d}} (\frac{N}{d})!}\Big)^d} \sqrt{\sum_{|\balpha|=0}^{N} \prod_{i=1}^{d} \frac{1}{(\balpha_i+1)^2} + \sum_{|\balpha|=0}^{N} \sum_{t=1}^{T}w_t^2 \sum_{t=1}^{T} \xv_t^{2\balpha}\exp\big(-\frac{\|\xv_t\|^2}{l^2}\big) } \label{eq:se_linear_int_upper_3}\\
    &\le B\sqrt{\big(\frac{ed}{l^2 N}\big)^N} \sqrt{\Big(\sum_{k=1}^{N+1}\frac{1}{k^2}\Big)^d  + \Big(\frac{N}{d}\Big)^d o\Big(\frac{1}{T}\Big) }, \label{eq:se_linear_int_upper_4}
\end{align}
where 
\begin{itemize}
    \item \eqref{eq:se_linear_int_upper_1} follows by Cauchy-Schwarz inequality, and consequently, \eqref{eq:se_linear_int_upper_2} uses \eqref{eq:se_f_rkhs} and the fact that $\mu_{\balpha}$ is a decreasing sequence;
    \item The first square root term in \eqref{eq:se_linear_int_upper_3} substitutes the value of $\mu_{\balpha^*}$ for $\balpha^*=[\frac{N}{d},\ldots,\frac{N}{d}]$;  The first term in the second square root of \eqref{eq:se_linear_int_upper_3} is since $D=[0,1]^d$, so that $\int_D \xv^{\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \le \int_D \xv^{\balpha} d\xv \le \prod_{i=1}^{d} \frac{1}{(\balpha_i+1)^2}$;  The second term in the second square root of \eqref{eq:se_linear_int_upper_3} again uses Cauchy-Schwarz inequality;
    \item \eqref{eq:se_linear_int_upper_4} is simply since $\max_{\xv\in D} \xv^{2\balpha} \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \le 1$ and $\sum_{t=1}^{T} w_t^2 = o(\frac{1}{T^2})$.
\end{itemize}

Recalling $N=dT^{\frac{1}{d}}$ in \eqref{eq:se_linear_int_upper_4}, we can continue to wirte:
\begin{equation*}\label{eq:se_linear_int_upper}
    |I(f) - \Ihat(f)| \le C_{gh}T^{-\frac{1}{2}T^{\frac{1}{d}}} \sqrt{\big(\frac{\pi}{6}\big)^d + o(1)} = C_l C_{gh} T^{-\frac{1}{2}T^{\frac{1}{d}}}, \quad C_l:=\sqrt{\big(\frac{\pi}{6}\big)^d + o(1)},
\end{equation*}
where we have used the fact that $\sum_{n=1}^{\infty}\frac{1}{n^2}=\frac{\pi}{6}$.  Finally, the proof is done for any $f\in\se$ with $\|f\|_{\se}\le B$, by amounting the residual error proved in the previous section.

% Denoting the worst case error to be $\epsilon$ and re-arranging \eqref{eq:se_error_worst} gives us that
% \begin{equation*}
%     N = O\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big),
% \end{equation*}
% and recalling $N=dT^{\frac{1}{d}}$, we obtain
% \begin{equation*}
%     T = O\bigg(\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big)^d\bigg). \label{eq:se_T_worst}
% \end{equation*}

% \section{Proof of SE Lower Bound}
% Following the idea of \cite{Kuo17}, given $T=N-1$ arbitrary inputs $\{x_1,\ldots,x_T\}$ from $D=[0,1]$, we can choose real numbers $\{\theta_1,\ldots,\theta_N\}$, such that 
% \begin{equation}
%     \sum_{m=1}^{N}\theta_m x_t^m = 0, \quad \forall t=1,2,\ldots,N-1. \label{eq:se_lower_linear}
% \end{equation}
%   Since the linear system has more unknowns ($N$) than the number of conditions ($N-1$), a non-trivial solution of \eqref{eq:se_lower_linear} certainly exists.  Thus, by re-scaling, there exists a solution such that
% \begin{equation}
%     \max_{1\le i\le N} |\theta_i|=1=\theta_k, \quad 1\le k\le N. \label{eq:theta_condition}
% \end{equation}
% We now define a function in the form:
% \begin{equation}
%     f(x) = \exp(-\frac{x^2}{2l^2}) \sum_{m=1}^{N}\theta_m x^m, \label{eq:se_lower_f}
% \end{equation}
% so that $f\in \se$, and most importantly, $f(x_t)=0$ for all $i=1,\ldots,N-1$, thus any quadrature rule based on linear combinations of these $N-1$ function values will return $0$.  Hence, the error of integrating $f(x)$ is equivalent to
% \begin{align}
%     \Big|\int_D f(x)dx -0 \Big| &= \Big|\int_D \exp(-\frac{x^2}{2l^2}) \sum_{m=1}^{N}\theta_m x^m dx \Big| \nonumber \\
%     &= \Big|\sum_{m=1}^{N} \theta_m \int_0^1 \exp(-\frac{x^2}{2l^2}) x^m dx \Big|. \label{eq:se_int_lower}
% \end{align}
% We argue that \eqref{eq:se_int_lower} cannot be $0$, since together with \eqref{eq:se_lower_linear}, we now have a linear system with same number of conditions and unknowns, thus $\theta$ is either unique or not existing.  This contradicts our assumption on the inputs and $\theta$, given that $\theta$ satisfies \eqref{eq:theta_condition}, we can perturb the inputs so that \eqref{eq:theta_condition} is no longer satisfied.  Therefore, $\big|\int_D f(x)dx\big|\in(0,\sum_{m=1}^N \frac{1}{m+1}]$, which can be regarded as a constant.

% an equivalent expression of $\rwstmat$ is 
% \begin{equation}
%     \sup_{p\in\Pc, f\in\Hc}\frac{|I-\Ihat|}{\|f\|_{\se}} = \sup_{p\in\Pc, f\in\Hc}\frac{1}{\|f\|_{\se}}. \label{eq:worst_error_equiv}
% \end{equation}

% Also, for $f$ defined in \eqref{eq:se_lower_f}, its RKHS norm is at most
% \begin{align}
%     \|f\|_{\se} &\le \sum_{m=1}^{N} |\theta_m| \|\tau_k(x)\tau_m(x)\|_{\se} \nonumber\\
%     &\le \sum_{m=1}^{N}  \|\tau_k(x)\tau_m(x)\|_{\se} \nonumber\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} \tau_m(x) \tau_k(x) \tau_j(x) dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand1}\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} x^{m+k} \exp(-\frac{3x^2}{4l^2}) x^{j} \exp(-\frac{3x^2}{4l^2})dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand2}\\\
%     &= \sum_{m=1}^N \bigg(\sum_{j\ge 0} \frac{1}{\mu_j} \Big(\int_{D} \tau'_{m+k}(x) \tau'_j(x) dx\Big)^2\bigg)^{1/2} \label{eq:se_rkhs_expand3}\\
%     &= \sum_{m=1}^N \frac{1}{\sqrt{\mu_{m+k}}} \label{eq:se_rkhs_expand4}\\
%     &\le \frac{N}{\sqrt{\mu_{2N}}}. \label{eq:se_rkhs_expand}
% \end{align}
% In the above equations:
% \begin{itemize}
%     \item \eqref{eq:se_rkhs_expand1} follows from the definition of RKHS norm, $\|f\|_{\se}^2 = \sum_{i\ge 0} \frac{\langle f, \tau_{i}\rangle_{L^2}^2}{\mu_i}$, see for example;
%     \item \eqref{eq:se_rkhs_expand2} is by expanding each $\tau(x)$ function and re-arranging;
%     \item $\tau'_{\alpha}(x) = x^{\alpha}\exp(-\frac{3x^2}{4l^2})$ in \eqref{eq:se_rkhs_expand3} can be regarded as the eigenfunction of the modified SE kernel $k'(x,x')=\exp(-\frac{3|x-x'|^2}{4l^2})$.  Therefore, $\langle \tau'_i, \tau'_j\rangle_{L^2} = 1$ for $i=j$, and $0$ otherwise, which yields \eqref{eq:se_rkhs_expand4};
%     \item \eqref{eq:se_rkhs_expand} is since $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence, i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{2N}$.
% \end{itemize}

% Moreover, recall the definition of the SE RKHS norm in \eqref{eq:se_rkhs}, the RKHS norm of $f$ defined in \eqref{eq:se_lower_f} can be bounded by
% \begin{align}
%     \|f\|_{\se}^2 = \sum_{m=1}^N \frac{\theta_m^2}{\mu_m} \le \frac{N}{\mu_N}, \label{eq:se_f_rkhs}
% \end{align}
% since $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence (i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{N}$).

% Combining \eqref{eq:se_f_rkhs} with \eqref{eq:se_int_lower}, the worst case error is at least 
% \begin{equation*}
%     \frac{\Big|\int_D f(x)dx - 0 \Big|}{\|f\|_{\se}} = \Omega\Big(\sqrt{\frac{\mu_{N}}{N}}\Big) = \Omega\Big(\frac{1}{\sqrt{N} l^{N} \sqrt{N!}}\Big) = \Omega\Big(\frac{1}{\sqrt{N}}\big(\frac{e}{N}\big)^{\frac{N}{2}} \Big).
% \end{equation*}
% Rearranging yields that
% \begin{equation*}
%     T=N-1=\Omega\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big).
% \end{equation*}


% \begin{lem} \label{lem:sig_interp_norm_upper}
%     The RKHS norm and the sampling norm regarding the kernel interpolant of the the noise $\varepsilon_1$, $\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1$, is upper bounded by
%     \begin{align}
%         \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se} &\le \frac{\|\varepsilon_1\| \sqrt{\lambda_{\min}(\Kv_T)}}{\lambda_{\min}(\Kv_T) + \lambda} , \label{eq:sig_interp_upper} \\
%         \big\|\big(\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \big)_X \big\|_{\infty} &\le \sqrt{T}\kappa C_F
%     \end{align}
%     where $\lambda_{\min}(\Kv_T)$ denotes the minimum eigenvalue of the kernel interpolant matrix $\Kv_T$, $\kappa = \sup_{\xv,\yv} \kse(\xv,\yv)$, and $C_F$ is the constant that guarantees $\|A\|_F \le C_F \|A\|_2 $.
% \end{lem}

% \begin{proof}
%     The proof simply follows from the reproducing property,
%     \begin{align}
%         \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se}^2 &= \varepsilon_1^T (\Kv_T^T +\lambda \Iv)^{-1} \Kv_T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \nonumber\\
%         &\le \|\varepsilon_1\|^2 \|(\Kv_T^T +\lambda \Iv)^{-1} \Kv_T (\Kv_T +\lambda \Iv)^{-1} \|_2 \nonumber\\
%         &\le \|\varepsilon_1\|^2  \|(\Kv_T +\lambda \Iv)^{-1}\|_2^2 \| \Kv_T\|_2 \label{eq:sig_interp_upper_1}\\
%         &\le \|\varepsilon_1\|^2 \frac{\lambda_{\min}(\Kv_T)}{\big( \lambda_{\min}(\Kv_T) + \lambda \big)^2} \label{eq:sig_interp_upper_2} ,
%     \end{align}
%     where $\|A\|_2$ for a matrix $A$ denotes the spectral norm, $\sup_{\xv\neq \bzero} \frac{\xv^T A \xv}{\|\xv\|^2}$; \eqref{eq:sig_interp_upper_1} uses the fact that $\|AB\|_2\le \|A\|_2\|B\|_2$ and $\Kv_T$ is symmetric; \eqref{eq:sig_interp_upper_2} is by the Rayleigh-Ritz theorem \cite{Hor12}.

%     \begin{align}
%         \big\|\big(\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \big)_X \big\|_{\infty}^2 &\le \sup_{\xv\in D}   \Big(\sum_{i=1}^T  \kse(\xv_t,\xv_i)  (\Kv_T +\lambda \Iv)^{-1}_{i,j} \sum_{j=1}^T \epsilon_j \Big)^2\\
%         &\le \Big(\sup_{\xv\in D, \xv_t\in X} \sum_{i=1}^T  \kse(\xv,\xv_i)^2 \Big)\sum_{i=1}^T\sum_{j=1}^T \big((\Kv_T +\lambda \Iv)^{-1}_{i,j}\big)^2  \sum_{j=1}^T \epsilon_j^2 \\
%         &\le T\kappa^2 \cdot \| (\Kv_T +\lambda \Iv)^{-1}\|_F^2 \cdot \|\varepsilon_1\|^2 \\
%         &\le T\kappa^2 C_F^2 \big( \lambda_{\min}(\Kv_T) + \lambda \big)^{-2} \|\varepsilon_1\|^2,
%     \end{align}
% \end{proof}

% Using Theorem \ref{thm:se_sampling_ineq}, and by triangle inequality, we have
% \begin{align}
%     \|f-\mu_T\|_{\se} \le \|f-\mu_T\|_{\se} + \|\kv_T(\xv)^T (\Kv_T +\lambda \Iv)^{-1} \varepsilon_1 \|_{\se}
% \end{align}

% Using Theorem \ref{thm:se_sampling_ineq}, for $f\in \se$, we derive
% \begin{align}
%     \|f - \mu_T\|_{L^2} &\le \exp\Big(\frac{C\log h_X}{h_X}\Big) \|f-\mu_T\|_{\se} + \exp\Big(\frac{\Ctil}{h_X}\Big) \|(f-\mu_T)_{X}\| \\
%     &\le \exp\Big(\frac{C\log h_X}{h_X}\Big) (\|f\|_{\se} + \|\mu_T\|_{\se}) +  \exp\Big(\frac{\Ctil}{h_X}\Big) \|(f-\mu_T)_{X}\| \\
%     &= O\bigg(\exp\Big(\frac{C\log h_X}{h_X}\Big)(\lambda^{-1}\|\varepsilon_1\| + B) + \exp\Big(\frac{\Ctil}{h_X}\Big) (\|\varepsilon_1\| + \lambda B) \bigg) \\
%     &= O\bigg( \exp\Big(\frac{C\log h_X}{h_X}\Big) + \exp\Big(\frac{\Ctil}{h_X}\Big)\lambda + \Big(\exp\Big(\frac{C\log h_X}{h_X}\Big)\lambda^{-1} + \exp\Big(\frac{\Ctil}{h_X}\Big)\Big) \|\varepsilon_1\|  \bigg)
% \end{align}


% In this section, we show how to obtain the noisy $L^2$ upper bound based on several properties in \cite{Bac17}, which are summarized in the following two lemmas.
% \begin{lem} \label{lem:int_sig_nosig}
%     {\em (Quadrature Noisy-noiseless relationship)}
%     Let $f$ be any function in $\se$, then for any algorithm that uses the linear combinations, $\Ihatsig =\sum_{t=1}^{T} \beta_t (f(\xv_t)+\epsilon_t)$ or $\Ihat =\sum_{t=1}^{T} \beta_t f(\xv_t)$, respectively of noisy or noiseless function evaluations, then we have the following relationship between the averaged integration error and the noiseless integration error:
%     \begin{equation}
%         \sup_{f\in \se} \EE[|I-\Ihatsig|^2] \le \sup_{f\in \se}2|I-\Ihat|^2 + 2\sum_{t=1}^{T}\beta_t^2 \EE[\|\varepsilon_1\|^2]. \label{eq:noisy_int_eq}
%     \end{equation}
% \end{lem}
% \begin{proof}
%     We note that $\EE[\cdot]$ in this section explicitly denotes the expectation taking with respect to $\varepsilon_1=\{\epsilon_1,\ldots,\epsilon_{T}\}$.  Then, we can use Cauchy-Schwarz inequality to obtain:
%     \begin{align*}
%         \EE\bigg[\Big|I-\sum_{t=1}^{T} \beta_t (f(\xv_t)+\epsilon_t)\Big|^2\bigg] &\le 2\Big|I-\sum_{t=1}^{T}\beta_t f(\xv_t) \Big|^2 + 2 \EE\bigg[\Big|\sum_{t=1}^{T} \beta_t \epsilon_t\Big|^2\bigg] \\
%         &\le 2|I-\Ihat|^2 +  2\EE\bigg[\sum_{t=1}^{T}\beta_t^2  \sum_{t=1}^{T}\epsilon_t^2\bigg]\\
%         &=  2|I-\Ihat|^2 + 2\sum_{t=1}^{T}\beta_t^2 \EE[\|\varepsilon_1\|^2].
%     \end{align*}
%     By taking the supreme over $f$ on both sides gives the proof.
% \end{proof}

% Before proceeding, we introduce a couple of lemmas in matrix analysis to help proving our upper bound.
% \begin{lem} \label{lem:mat_inv_diff}
%     {\em (\citep[Sec 5.8]{Hor12})}
%     Let $\|\cdot\|$ be a given matrix norm, for two nonsingular matrices $A$ and $B$, denote $\Delta = A-B$.  Given the assumption that $\|\Delta A^{-1}\|\le 1$, we have,
%     \begin{equation}
%         \|A^{-1} - B^{-1}\| \le \frac{\|A^{-1}\|^2\|\Delta\|}{1- \|A^{-1}\Delta\|}.
%     \end{equation}
% \end{lem}

% \begin{lem} \label{lem:mat_norm_bound}
%     {\em (\citep[Sec 5.8]{Hor12})}
%     Let $\|\cdot\|$ be a given matrix norm, for two real and symmetric matrices $A$ and $B$, we have,
%     \begin{equation}
%         \|(A+B)^{-1}\| \le \|A^{-1}\|.
%     \end{equation}
% \end{lem}

% Let $\phi(\xv)=\exp(-\frac{\|\xv\|^2}{2l^2})[\mu_{\bzero}\xv^{\bzero},\ldots,\mu_{\balpha}\xv^{\balpha},\ldots]^T$ be the infinite dimensional feature mapping of the SE kernel, which can be expanded as:
%  \begin{equation}
%         \exp\Big(-\frac{\|\xv-\yv\|^2}{2l^2}\Big) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\yv\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha}^2 \xv^{\balpha}\yv^{\balpha} = \phi(\xv)^T\phi(\yv). \label{eq:kse_expand}
%     \end{equation}
% Then, we have the following Theorem.
% \begin{thm} \label{thm:se_l2_upper_nosig}
%     {\em (Noisy $L^2$ Upper bound -- SE kernel)}
%     Let $f(\xv) = \int_D g(\yv)\kse(\xv,\yv)d\yv $ be any function lies in $\se$, where $g(\xv)\in L^2(D)$ and $\|g\|_{L^2}\le 1$, so that the RKHS norm of $f$ is less than $1$.  Denote 
%     $$
%         \fhat(\xv)= \kv_T(\xv)^T \Kv_T^{-1} \yv_T
%     $$ 
%     as the noiseless estimation of $f$, and 
%     $$
%         \fhatsig(\xv)= \kv_T(\xv)^T \Kv_T^{-1} (\yv_T+\varepsilon_1)
%     $$
%     as the noisy estimation of $f$.  Then, the error of estimating the noisy $L^2$-distance on $[0,1]^d$ is upper bounded by:
%     \begin{equation}
%         \EE\big[ \|f-\fhatsig\|_{L^2} \big] \le \|f-\fhat\|_{L^2} + O\Big(T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \label{eq:se_l2_upper_sig}
%     \end{equation}
% \end{thm}

% \begin{proof}
    % Consider the following expansion:
    % \begin{equation}
    %     \exp\big(\frac{\|\xv-\xv_t\|^2}{2l^2}\big) = \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha}^2 \xv_t^{\balpha}\xv^{\balpha}.
    % \end{equation}
    % We first observe that $f(\xv_t)=\psi(\xv_t)^T (\sqrt{\mu}\theta)$:
    % \begin{equation*}
    %     \psi(\xv_t)^T (\sqrt{\mu}\theta) = \exp(-\frac{\|\xv_t\|^2}{2l^2})\sum_{\balpha\in\NNd}\theta_{\balpha}\mu_{\balpha}\xv_t^{\alpha} = f(\xv_t).
    % \end{equation*}
    % By denoting $\bthetahat := \Phi^{-1} \yv_T$, we can expand $\fhat$ as
    % \begin{equation*}
    %     \fhat(\xv) = \exp(-\frac{\|\xv\|^2}{2l^2})\sum_{\balpha\in\NNd} \bthetahat_{\balpha}\mu_{\balpha} \xv^{\balpha}.
    % \end{equation*}
    % Then, the $L^2$ distance between $f$ and $\fhat$ is
    % \begin{align*}
    %     \|f-\fhat\|_{L^2}^2 &= \int_D \Big( \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} (\theta_{\balpha} -  \thetahat_{\balpha}) \Big)^2 d\xv \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\theta_{\balpha} - \thetahat_{\balpha}) (\theta_{\bgamma} - \thetahat_{\bgamma}) \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv.
    % \end{align*}
    % \begin{align}
    %     \fhat(\xv) &= \sum_{t=1}^{T} \beta_t \psi(\xv_t)^T \psi(\xv)\\
    %     &= \sum_{t=1}^{T/2}\beta_t \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \mu_{\balpha} \xv_t^{\balpha}\xv^{\balpha} \nonumber\\
    %     &= \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} \sum_{t=1}^{T/2} \beta_t \xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)
    % \end{align}
    % We can expand $\fhat$ as:
    % \begin{align}
    %     \fhat(\xv) &=  \exp\big(-\frac{\|\xv\|^2}{2l^2}\big) \sum_{t=1}^{T/2}\beta_t  \exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \sum_{\balpha\in\NNd} \theta_{\balpha} \mu_{\balpha} \xv_t^{\balpha} \nonumber \\
    %     &= \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \sum_{t=1}^{T/2} \beta_t \xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)
    % \end{align}
    % Denoting $\Upsilon_{\balpha}:= \sum_{t=1}^{T/2}\beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)$, the $L^2$ distance between $f$ and $\fhat$ is then
    % \begin{align}
    %     \|f-\fhat\|_{L^2}^2 &= \int_D \bigg( \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd} \mu_{\balpha}\xv^{\balpha} \Big(\theta_{\balpha} - \sum_{t=1}^{T/2} \beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big) \Big)  \bigg)^2 d\xv \nonumber\\
    %     &= \int_D \exp\big(-\frac{\|\xv\|^2}{l^2}\big) \Big(\sum_{\balpha\in\NNd} \mu_{\balpha} \xv^{\balpha} (\theta_{\balpha} - \Upsilon_{\balpha}) \Big)^2 d\xv \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\theta_{\balpha} - \Upsilon_{\balpha}) (\theta_{\bgamma} - \Upsilon_{\bgamma}) \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv. \label{eq:se_l2_expand}
    % \end{align}
    % Denoting $\Lambda_{\balpha} := \int_D \xv^{\alpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv$, the error of estimating the integration is
    % Denoting $\Upsilon_{\balpha} := \int_D \xv^{\alpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv$, and $\Upsilonhat_{\balpha} := \sum_{t=1}^{T/2}\beta_t\xv_t^{\balpha}\exp\big(-\frac{\|\xv_t\|^2}{2l^2}\big)$, the error of integration can be calculated in the similar fashion:
    % \begin{align}
    %     |I - \Ihat|^2 &= \bigg( \int_D \exp(-\frac{\|\xv\|^2}{2l^2})\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv^{\balpha} d\xv -  \sum_{t=1}^{T/2}\beta_t \exp(-\frac{\|\xv_t\|^2}{2l^2})\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv_t^{\balpha} \bigg)^2 \nonumber\\
    %     &= \Big(\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} (\Upsilon_{\balpha} - \Upsilonhat_{\bgamma} )  \Big)^2 \nonumber\\
    %     &= \sum_{\balpha\in\NNd} \sum_{\bgamma\in\NNd} \mu_{\balpha}\mu_{\bgamma} (\Upsilon_{\balpha} - \Upsilonhat_{\balpha}) (\Upsilon_{\bgamma} - \Upsilonhat_{\bgamma}) \theta_{\balpha}\theta_{\gamma}. \label{eq:se_int_expand}
    % \end{align}
    % Now, by setting $\theta_{\balpha} = \Lambda_{\balpha}$, it can be seen that the only difference between \eqref{eq:se_l2_expand} and \eqref{eq:se_int_expand} is $\Lambda_{\balpha}\Lambda_{\bgamma}$ v.s. $\int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv$.  We can further compare these two by noting that $D=[0,1]^d$:
    % \begin{equation*}
    %     \int_D \xv^{\balpha}\exp\big(-\frac{\|\xv\|^2}{2l^2}\big) d\xv \le \int_D\xv^{\balpha} d\xv = \prod_{i=1}^d \frac{1}{\balpha_i+1}.
    % \end{equation*}
    % Hence we have
    % \begin{equation}
    %     \Lambda_{\balpha}\Lambda_{\bgamma} \le \prod_{i=1}^d \frac{1}{(\balpha_i+1)(\bgamma_i+1)} \le \prod_{i=1}^d \frac{1}{\balpha_i+\bgamma_i+1}, \label{eq:l2_residual}
    % \end{equation}
    % and
    % \begin{equation}
    %     \int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv \le \prod_{i=1}^d \frac{1}{\balpha_i+\bgamma_i+1}. \label{eq:int_residual}
    % \end{equation}
    % We have now proved that the supremacy between $\|f-\fhat\|_{L^2}^2$ and $|I - \Ihat|^2$ are equivalent, the rest of the proof is to show that setting $\theta_{\balpha} = \Lambda_{\balpha}$ dose not violate the smoothness of the function:
    % \begin{equation*}
    %     \sum_{\balpha\in\NNd} \theta_{\balpha}^2 \le \sum_{\balpha\in\NNd} \prod_{i=1}^d \frac{1}{(\balpha_i+1)^2} = \prod_{i=1}^d \sum_{\balpha_i \ge 2} \frac{1}{\balpha_i^2} \le \Big(\frac{\pi^2}{6}-1\Big)^d := B,
    % \end{equation*}
    % where we have used the fact that $\sum_{n\ge 1} \frac{1}{n^2} = \frac{\pi^2}{6}$.
    % Let 
    % $$
    %     \Phi = [\phi(\xv_1),\ldots,\phi(\xv_T)]^T \in \RR^{T\times\infty}
    % $$
    % be the feature matrix with infinite number of columns, then we have the following properties,
    % \begin{align*}
    %     \Kv_T &= \Phi \Phi^T, \\
    %     \kv_T(\xv) &= \Phi \phi(\xv), \\
    %     \yv_T &= \Phi \btheta.
    % \end{align*}
    % Under the setting that $T\to \infty$, together we can derive
    % \begin{align}
    %     f(\xv) &= \phi(\xv)^T \btheta \nonumber\\
    %     & = (\Phi^{-1} \kv_T(\xv))^T (\Phi^{-1} \yv_T) \nonumber\\
    %     & = \kv_T(\xv)^T (\Phi\Phi^T)^{-1} \yv_T \nonumber\\
    %     & = \kv_T(\xv)^T \Kv_T^{-1} \yv_T. \label{eq:fse_equal}
    % \end{align}
    % For $\lambda$ being small enough, such that $\lambda \|\Kv_T^{-1}\|\le 1$ satisfies for an appropriate matrix norm,  we have the following Neumann series
    % \begin{align*}
    %     (\Kv_T + \lambda \Iv_T)^{-1} &= \Kv_T^{-1}(\lambda \Kv_T^{-1} + \Iv_T)^{-1} \\
    %     &= \Kv_T^{-1} -\lambda \Kv_T^{-2} + \lambda^2\Kv_T^{-3} - \ldots
    % \end{align*}
    % % By truncating the rest, $(\Kv_T + \lambda \Iv_T)^{-1}$ can be approximated by $\Kv_T^{-1} -\lambda \Kv_T^{-2} $.
    % On the one hand, by Cauchy-Schwartz inequality, we have
    % \begin{align*}
    %     f(\xv)^2 &= \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \Big(\sum_{\balpha\in\NNd} \theta_{\balpha}\mu_{\balpha} \xv^{\balpha} \Big)^2 \\
    %     &\le \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \sum_{\balpha\in\NNd}\mu_{\balpha}^2 \xv^{2\balpha} \\
    %     &= \exp\Big(-\frac{\|\xv\|^2}{l^2}\Big) \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \exp\Big(\frac{\|\xv\|^2}{l^2}\Big) \\
    %     &= \sum_{\balpha\in\NNd}\theta_{\balpha}^2 \\
    %     &\le B^2,
    % \end{align*}
    % so that the $L^2$-norm of $f$ is also bounded by $B$ since our domain is $[0,1]^d$.  On the other hand, recall \eqref{eq:fse_equal}, and again by Cauchy-Schwartz inequality, we write
    % \begin{align*}
    %     \|f(\xv)\|_{L^2} &= \Big\| \kv_T(\xv)^T \Kv_T^{-1} \yv_T \Big\|_{L^2} \\
    %     &\le \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \big\|\Kv_T^{-1} \big\|_F \cdot \|\yv_T\| \\
    %     &\le \sqrt{T} \max_{\xv^*\in\{\xv_1,\ldots,\xv_T\}} \big|f(\xv^*)\big| \sqrt{T \int_D \exp\Big(-\frac{\|\xv-\xv^*\|^2}{l^2}\Big) d\xv} \cdot \big\|\Kv_T^{-1} \big\|_F \\
    %     &\le TB\big\|\Kv_T^{-1} \big\|_F,
    % \end{align*}
    % where the last step is since $\max_{\xv\in D} |f(\xv)| \le B$ and $\max_{\xv^*} \int_D \exp\big(-\frac{\|\xv-\xv^*\|^2}{l^2}\big) d\xv \le 1$.  Equating the last equation with $B$, we can see that
    % \begin{equation}
    %     \big\|\Kv_T^{-1} \big\|_F  = \Theta\Big(\frac{1}{T}\Big). \label{eq:kernel_matnorm_upper}
    % \end{equation}
    % Therefore,
%     First, by triangle inequality, it is easy to observe that
%     \begin{equation}
%         \|f-\fhatsig\|_{L^2} \le \|f-\fhat\|_{L^2} + \|\fhat-\fhatsig\|_{L^2}.
%     \end{equation}
%     Thus, we aim to deal with these two terms separately. $\fhat$ can be explicitly written as the following:
%     \begin{equation*}
%         \fhat = \sum_{t=1}^{T} \beta_t \kse(\xv,\xv_t), \quad \text{where } (\beta_1,\ldots,\beta_T)^T = \Kv_T^{-1} \yv.
%     \end{equation*}

%     \begin{align}
%         \|\fhat - \fhatsig\|_{L^2} &= \Big\|\kv_T(\xv)^T \Kv_T^{-1} \yv_T -  \kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} \yv_T \Big\|_{L^2} \nonumber \\
%         &=\Big\|\kv_T(\xv)^T (\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}) \yv_T\Big\|_{L^2} \nonumber\\
%         &\le \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \Big\|\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}\Big\|_F \cdot \|\yv_T\| \nonumber\\
%         &\le O\bigg(T  \Big\|\Kv_T^{-1} - \big(\Kv_T + \lambda \Iv_T \big)^{-1}\Big\|_F\bigg) \nonumber\\
%         &\le O\bigg( \frac{T\|\Kv_T^{-1}\|_F^2 \|\lambda \Iv_T\|_F}{1- \|\Kv_T^{-1}\lambda \Iv_T\|_F}\bigg) \label{eq:se_l2_upper_nosig_1} \\
%         &\le O\bigg( \frac{\|\Kv_T^{-1}\|_F^2}{1- \lambda\|\Kv_T^{-1}\|_F} \lambda T^{\frac{3}{2}}\bigg) \\
%         &\le O\Big(\frac{\lambda}{\sqrt{T}}\Big), \label{eq:se_l2_upper_nosig_2}
%     \end{align}
%     where \eqref{eq:se_l2_upper_nosig_1} -- \eqref{eq:se_l2_upper_nosig_2} has used Lemma \ref{lem:mat_inv_diff} and \eqref{eq:kernel_matnorm_upper}, and the fact that $\|\Iv_T\|_F = \sqrt{T}$, $\lambda\|\Kv_T^{-1}\|_F \ll 1$.
% \end{proof}

% \begin{cor} \label{cor:se_l2_upper_sig}
%     {\em (Noisy $L^2$ upper bound -- SE kernel)}
%     Under the setup of Theorem \ref{thm:se_l2_upper_nosig}, with only $\yv_T$ replaced by the noisy version.  Then, the error of estimating the noisy $L^2$-distance on $[0,1]^d$ is upper bounded by:
%     \begin{equation}
%        \EE[\|f-\mu_T\|_{L^2}] = O\Big( \lambda T^{-\frac{1}{2}} + T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \label{eq:se_l2_upper_sig}
%     \end{equation}
% \end{cor}
% \begin{proof}
%     Using Lemma \ref{lem:mat_norm_bound}, and the proof in Theorem \ref{thm:se_l2_upper_nosig}, it follows that
%     \begin{align}
%         \EE[\|f-\mu_T\|_{L^2}] &= \EE\bigg[\Big\|\kv_T(\xv)^T \Kv_T^{-1} \yv_T -  \kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} (\yv_T + \varepsilon_1)\Big\|_{L^2} \bigg] \nonumber\\
%         &\le \|f-\fhat\|_{L^2} + \EE\bigg[ \Big\|\kv_T(\xv)^T\big(\Kv_T + \lambda \Iv_T \big)^{-1} \varepsilon_1\Big\|_{L^2} \bigg] \nonumber\\
%         &\le \|f-\fhat\|_{L^2} +  \sqrt{\sum_{t=1}^T \big\|\kse(\xv,\xv_t)\big\|_{L^2}^2} \cdot \big\|\Kv_T^{-1} \big\|_F \cdot \EE[\|\varepsilon_1\|] \label{eq:se_l2_upper_sig_1}\\
%         &= O\Big(\lambda T^{-\frac{1}{2}} + T^{-\frac{1}{2}} \EE[\|\varepsilon_1\|] \Big). \nonumber
%     \end{align}
% \end{proof}


% \begin{proof}
%     Since we have shown the supremacy of $\EE[|I-\Ihatsig|^2]$ in Lemma \ref{lem:int_sig_nosig}, we are left to show the supremacy of $\EE[\|f-\fhatsig\|_{L^2}^2]$:
%     \begin{align*}
%         \EE[\|f-\fhatsig\|_{L^2}^2] &= \EE\bigg[\Big\| f-\fhat - \sum_{t=1}^{T/2}\beta_t\epsilon_t  \exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd}\frac{\xv^{\balpha}}{\theta_{\balpha}} \Big\|_{L^2}^2\bigg] \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\EE\bigg[\Big|\sum_{t=1}^{T/2}\beta_t\epsilon_t \Big|^2 \bigg] \Big\|\exp\big(-\frac{\|\xv\|^2}{2l^2}\big)\sum_{\balpha\in\NNd}\frac{\xv^{\balpha}}{\theta_{\balpha}} \Big\|_{L^2}^2 \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\sum_{t=1}^{T/2}\beta_t^2 \EE[\|\varepsilon_1\|^2] \sum_{\balpha}\sum_{\bgamma} \frac{\int_D \xv^{\balpha+\bgamma} \exp\big(-\frac{\|\xv\|^2}{l^2}\big) d\xv}{\Lambda_{\balpha}\Lambda_{\bgamma}} \\
%         &\le 2\| f-\fhat\|_{L^2}^2 + 2\sum_{t=1}^{T/2}\beta_t^2 \EE[\|\varepsilon_1\|^2] ,
%     \end{align*}
%     where the last inequality follows since \eqref{eq:int_residual} and $\Lambda_{\balpha}\Lambda_{\bgamma} \ge $
% \end{proof}

% Combining \eqref{eq:noisy_int_eq}, \eqref{eq:int_l2_nosig} and \eqref{eq:int_l2_sig} in these two lemmas, it is easy to see that 
% \begin{equation}
%     \sup_{\|f\|_{\se}\le 1}\EE[\|f-\fhat\|_{L^2}^2] \le \Big( \sup_{p\in\Pc,\|f\|_{\se}\le 1}|I-\Ihat| +  \sqrt{\sum_{t=1}^{T/2}\alpha_i^2} \EE[\|\varepsilon_1\|_2]\Big)^2 + \sum_{t=1}^{T/2}\alpha_i^2 \var[\|\varepsilon_1\|_2]. \label{eq:l2_se_sig}
% \end{equation}


% The first term in the above equation includes the worst-case noiseless integration error, $\rwstse$, which we can recall Theorem \ref{thm:noiseless_upper} part 3.  Therefore, it remains to bound $\sqrt{\sum_{t=1}^{T/2}\alpha_i^2}$.  In \cite{Bac17}, $\alpha_i$ is treated as the fraction of $\frac{\beta_i}{q(\xv_i)^{1/2}}$, where $\|\beta\|_2^2\le \frac{8}{T}$, and $q(\xv_i)$ is regarded as the {\em importance weight}, so that $\{\xv_1,\ldots,\xv_{T/2}\}$ are now sampled i.i.d from the density $q$.  Most importantly, the optimized distribution $q(\xv)\propto \sum_{m\ge 1} \frac{\mu_m}{\mu_m+\lambda}e_m(\xv)^2$, is uniform (which is a constant) on $[0,1]^d$, given the fact that the eigen-functions of the SE kernel integral operator can be expressed as the $d$-th order tensor product of the uni-dimensional Fourier basis.  For more details, one may refer to \citep[Section 4.4]{Bac17}.  Therefore, we are ready to obtain 
% \begin{equation*}
%     \sum_{t=1}^{T/2}\alpha_i^2 = \sum_{t=1}^{T/2}\frac{\beta_i^2}{q(\xv_i)} = O(\|\beta\|_2^2) = O\Big(\frac{1}{T}\Big).
% \end{equation*}
% To make the proof complete, we need to show that $\mu_{T/2}(\xv)$ is one kind of $\fhat$, indeed, $\mu_{T/2}(\xv) = \sum_{t=1}^{T/2} [(\Sigma + \lambda I)^{-1}\yv_{T/2})]_i \cdot k(\xv,\xv_i)$.  The proof is then finished by substituting the bound of $\rwstse$ and  $\sum_{t=1}^{T/2}\alpha_i^2 $ into \eqref{eq:l2_se_sig}.
% \section{Lower Bound on SE Kernel When $d=1$} \label{app:se_lower}
% For each $\btheta\in\{0,1\}^N$, we define $f_{\btheta}\in\Fc(B)$ (with the kernel being the SE kernel) as
% \begin{equation}
%     f_{\btheta}(x) = B\sqrt{\frac{\mu_N}{N}} \sum_{i=0}^{N-1} \btheta(i) \tau_i(x),
% \end{equation}
% where $\mu_N=\frac{1}{l^{2N} N!}$ and $\tau_i(\xv)=x^i\exp(-\frac{x^2}{2l^2})$.  It can be verified that $f$ belongs to $\Fc(B)$:
% \begin{equation*}
%     \|f\|_{\se}^2 = \frac{B^2\mu_N}{N}\sum_{i=1}^{N}\frac{\theta^2}{\mu_k} \le \frac{B^2\mu_N}{N}\sum_{i=1}^{N}\frac{\theta^2}{\mu_N} \le B^2.
% \end{equation*}

% It is worth noting that the decreasing sequence $\mu_0\ge\mu_1\ge\ldots\ge 0$ and the corresponding functions $\{\tau_i(x)\}_{i=0}^{\infty}$ forms an eigen system of the following integral operator $(\Lk f)(\xv) : L^2(D)\rightarrow L^2(D)$:
% \begin{equation*}
%     (\Lk f)(\xv) = \int_D k(\xv, \yv) f(\yv) d\yv = \langle k(\xv,\cdot), f \rangle_{L^2},
% \end{equation*}
% which applying to the eigenfunctions, we have
% \begin{equation*}
%     (\Lk \tau_{\balpha})(\xv) = \mu_{\balpha} \tau_{\balpha}(\xv).
% \end{equation*}
% Then, the spectral theorem implies that the SE kernel can be decomposed into:
% \begin{equation*}
%     k(\xv,\yv) = \sum_{\balpha\in\NNd} \mu_{\balpha} \tau_{\balpha}(\xv) \tau_{\balpha}(\yv).
% \end{equation*}
% Moreover, it turns out that the square root of the operator, $\Lk^{1/2}$, is an isometric embedding of $L^2\rightarrow\se$.  Specifically, for $f,g\in L^2(D)$, we have
% \begin{equation*}
%     \langle\Lk^{1/2}f, \Lk^{1/2}g\rangle_{\se} = \langle f, g\rangle_{L^2}.
% \end{equation*}
% Similarly, for kernel $k(\xv,\yv)$, we have
% \begin{equation*}
%     k(\xv,\yv) = \langle k(\xv,\cdot), k(\yv,\cdot)\rangle_{\se} = \langle\Lk^{1/2}\psi(\xv,\cdot), \Lk^{1/2}\psi(\xv,\cdot)\rangle_{\se} =\langle \psi(\xv,\cdot), \psi(\yv,\cdot)\rangle_{L^2},
% \end{equation*}
% where $\psi(\xv,\yv)$ can be decomposed into:
% \begin{equation*}
%     \psi(\xv,\yv) = \sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv) \tau_{\balpha}(\yv).
% \end{equation*}


% \begin{thm} \label{thm:se_lower_worst}
%     {\em (SE kernel worst-case lower bound)} 
%     For a family of functions $\{\psi_1(\xv),\ldots,\psi_T(\xv)\}\in L^2(D)$ satisfying the following conditions
%     \begin{itemize}
%         \item[(i)] $\frac{1}{T}\sum_{i=1}^{T}\|\psi_i(\xv)\|_{L^2} \le \tr(L)$
%         \item[(ii)] $\sup_{f\in\Fc}\inf_{\sum_{i=1}^{T}\beta_i^2\le \frac{1}{T}} \|f-\sum_{i=1}^{T}\beta_i\psi_i\|_{L^2} \le \epsilon$ 
%     \end{itemize}
%     Then,
%     \begin{equation*}
%         T = \Omega\bigg(\Big(\frac{\log\frac{1}{\epsilon}}{\log\log\frac{1}{\epsilon}}\Big)^d\bigg).
%     \end{equation*}
% \end{thm}

% Using Varshamov-Gilbert’s lemma, there exists a family of $\{\btheta_j\}_{j\in\Jc}$, such that for $j\neq j'\in\Jc$, $\|\btheta_j - \btheta_{j'}\|^2 \ge \frac{N}{4}$, and consequently, $\|f_{\btheta_j} - f_{\btheta_{j'}}\|_{L^2} = \frac{B^2\mu_N}{N} \|\btheta_j - \btheta_{j'}\|^2 \ge \frac{B^2\mu_N}{4}$.  

% For algorithms linearly combining the evaluations $\{f(\xv_1),\ldots f(\xv_T)\}$, the mean absolute error can be expressed using the reproducing property:
% \begin{align*}
%     \Big| \int_D f(\xv) d\xv - \sum_{i=1}^{T} \beta_i f(\xv_i) \Big| &= \Big| \langle f,   \int_D k(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i k(\xv_i,\cdot) \rangle_{\se} \Big|\\
%     &\le \|f\|_{\se} \cdot \Big\|\int_D k(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i k(\xv_i,\cdot) \Big\|_{\se} \\
%     &\le B \Big\|\int_D \psi(\xv,\cdot) d\xv - \sum_{i=1}^{T} \beta_i \psi(\xv_i,\cdot) \Big\|_{L^2}  \\
%     &= B \Big\|\int_D \sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv) \tau_{\balpha}(\cdot) d\xv - \sum_{i=1}^{T} \beta_i \sum_{\balpha\in\NNd}\sqrt{\mu_{\balpha}} \tau_{\balpha}(\xv_i) \tau_{\balpha}(\cdot) \Big\|_{L^2} \\
%     &= B \Big\|\sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} \\
%     &= B \Big\|\sum_{\balpha\in\NNd} \sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} \\
%     &\le B \sum_{\balpha\in\NNd} \Big\|\sqrt{\mu_{\balpha}} \tau_{\balpha}(\cdot) \big( \int_D \tau_{\balpha}(\xv) d\xv -   \sum_{i=1}^{T} \beta_i\tau_{\balpha}(\xv_i) \big)  \Big\|_{L^2} 
% \end{align*}




% We note that $\mu_m=\frac{1}{l^{2m} m!}$ is a decreasing sequence, i.e., $\mu_1\ge\mu_2\ge\ldots\ge \mu_{2N}$.

% From the definition of RKHS norm, $\|f\|_{\se}^2 = \sum_{i\ge 0} \frac{\langle f, \tau_{i}\rangle_{L^2}^2}{\mu_i}$, it can be verified that $f$ belongs to $\Fc(B)$:
% \begin{align*}
%     \|f\|_{\se}^2 = \frac{B^2\mu_{2N}}{N} \Big(\frac{\theta_k^2 }{\mu_{2k}}+ \sum_{m\in M}\frac{\theta_m^2}{\mu_{2m-1}} \Big) = \frac{B^2}{N} \Big(\frac{\mu_{2N}}{\mu_{2k}}\theta_k^2 + \sum_{m\in M}\frac{\mu_{2N}}{\mu_{2m-1}} \theta_m^2 \Big) \le B^2,
% \end{align*}
% where the first equality is since $\langle \tau_i,\tau_i\rangle_{L^2} = 1$ whereas $\langle \tau_i,\tau_j\rangle_{L^2} = 0$ for $i\neq j$.

% On the other hand, we have
% \begin{equation*}
%     \int_{-1}^1 f(x) dx = \frac{B\sqrt{\mu_{2N}}}{\sqrt{N}} \int_{-1}^{1} \Big(\theta_k \tau_{2k}(x) +\sum_{m\in M} \theta_m \tau_{2m-1}(x) \Big) dx = \frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \theta_{k} \int_{0}^1 \tau_{2k}(x) dx,
% \end{equation*}
% since $\{\tau_{2m-1}\}$ are odd functions and $\tau_{2k}$ is even.  Therefore, the worst case error is at least 
% \begin{align*}
%     |I(f) - 0| &= \Big|\frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \theta_k \int_0^1 x^{2k} \exp(-\frac{x^2}{2l^2})dx  \Big|\\
%     &\ge \frac{2B\sqrt{\mu_{2N}}}{\sqrt{N}} \int_0^1 x^{2N} \exp(-\frac{x^2}{2l^2})dx \\
%     &\ge \frac{2B}{\sqrt{N}l^{2N} \sqrt{2N!} } \exp(-\frac{1}{2l^2})\int_{0}^{1} x^{2N} dx\\
%     &= \Omega\Big(\frac{1}{N\sqrt{N}\sqrt{2N!}} \Big) \\
%     &= \Omega\Big(\frac{1}{N\sqrt{N}}\big(\frac{e}{2N}\big)^{N} \Big).
% \end{align*}
